OMNI-EPIC: Open-endedness via Models of human Notions of Interestingness with Environments Programmed in Code

Open-ended and AI-generating algorithms aim to continuously generate and solve increasingly complex tasks indefinitely, offering a promising path toward more general intelligence. To accomplish this grand vision, learning must occur within a vast array of potential tasks. Existing approaches to automatically generating environments are constrained within manually predefined, often narrow distributions of environment, limiting their ability to create any learning environment. To address this limitation, we introduce a novel framework, OMNI-EPIC, that augments previous work in Open-endedness via Models of human Notions of Interestingness (OMNI) with Environments Programmed in Code (EPIC). OMNI-EPIC leverages foundation models to autonomously generate code specifying the next learnable (i.e., not too easy or difficult for the agent's current skill set) and interesting (e.g., worthwhile and novel) tasks. OMNI-EPIC generates both environments (e.g., an obstacle course) and reward functions (e.g., progress through the obstacle course quickly without touching red objects), enabling it, in principle, to create any simulatable learning task. We showcase the explosive creativity of OMNI-EPIC, which continuously innovates to suggest new, interesting learning challenges. We also highlight how OMNI-EPIC can adapt to reinforcement learning agents' learning progress, generating tasks that are of suitable difficulty. Overall, OMNI-EPIC can endlessly create learnable and interesting environments, further propelling the development of self-improving AI systems and AI-Generating Algorithms. Project website with videos: https://dub.sh/omniepic

==> env_codes/few_shot/few_shot_1.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env


class Env(R2D2Env):
    """
    Balance on a board placed on top of a rolling cylinder.

    Description:
    - A cylinder (radius 0.5 m and height 1 m) is placed on the ground and can roll along the y-axis.
    - A board (length 3 m, width 2 m and thickness 0.05 m) is placed on top of the cylinder.
    The robot is initialized on top of the board facing toward the positive x-axis.
    The task of the robot is to stand on the board and keep its balance on the board while the cylinder moves underneath.

    Success:
    The task is completed if the robot remains standing on the board for more than 10 s.

    Rewards:
    The robot is rewarded for remaining on the board.

    Termination:
    The task terminates if the robot falls of the board.
    """

    def __init__(self):
        super().__init__()

        # Init ground
        self.ground_size = [10., 10., 10.]
        self.ground_position = [0., 0., 0.]
        self.ground_id = self.create_box(mass=0., half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)

        # Init cylinder
        self.cylinder_radius = 0.5
        self.cylinder_height = 1.
        self.cylinder_position_init = [self.ground_position[0], self.ground_position[1], self.ground_position[2] + self.ground_size[2] / 2 + self.cylinder_radius]
        self.cylinder_orientation_init = self._p.getQuaternionFromEuler(eulerAngles=[0., np.pi / 2, 0.])  # roll along y-axis
        self.cylinder_id = self.create_cylinder(mass=10., radius=self.cylinder_radius, height=self.cylinder_height, position=self.cylinder_position_init, orientation=self.cylinder_orientation_init, color=[0., 0., 1., 1.]) 
        self._p.changeDynamics(bodyUniqueId=self.cylinder_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)

        # Init board
        self.board_size = [2., 3., 0.05]
        self.board_position_init = [self.cylinder_position_init[0], self.cylinder_position_init[1], self.cylinder_position_init[2] + self.cylinder_radius + self.board_size[2] / 2]  # Init board above cylinder
        self.board_id = self.create_box(mass=10., half_extents=[self.board_size[0] / 2, self.board_size[1] / 2, self.board_size[2] / 2], position=self.board_position_init, color=[1., 0., 0., 1.])
        self._p.changeDynamics(bodyUniqueId=self.board_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, orientation, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position, baseOrientation=orientation)

    def reset(self):
        observation = super().reset()

        # Reset time
        self.time = 0.

        # Reset cylinder position
        self._p.resetBasePositionAndOrientation(self.cylinder_id, self.cylinder_position_init, self.cylinder_orientation_init)

        # Reset board position
        self._p.resetBasePositionAndOrientation(self.board_id, self.board_position_init, [0., 0., 0., 1.])

        # Reset robot position
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.board_position_init[0], self.board_position_init[1], self.board_position_init[2] + self.board_size[2] / 2 + self.robot.links["base"].position_init[2]], self.robot.links["base"].orientation_init)

        return observation

    def step(self, action):
        observation, reward, terminated, truncated, info = super().step(action)

        # Increase time
        self.time += self.dt

        return observation, reward, terminated, truncated, info

    def get_task_rewards(self, action):
        # On board
        on_board = 1. if self.robot.links["base"].position[2] > self.board_position_init[2] + self.board_size[2] / 2 else -1.
        return {"on_board": on_board}

    def get_terminated(self, action):
        # Terminate if not on board
        is_on_board = self.robot.links["base"].position[2] > self.board_position_init[2] + self.board_size[2] / 2
        return not is_on_board

    def get_success(self):
        # Success if on board after 10. s
        on_board = self.time >= 10. and self.robot.links["base"].position[2] > self.board_position_init[2] + self.board_size[2] / 2
        return on_board
\end{lstlisting}


==> env_codes/long_run/long_run_103.tex <==
\begin{lstlisting}[language=Python]
import os
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Conveyor Belt Item Delivery

    Description:
    - The environment consists of two 5 m x 5 m platforms connected by a 5 m long conveyor belt. The conveyor belt moves from left to right at a speed of 0.5 m/s.
    - On the right platform, there are three target areas marked by 1 m x 1 m colored squares (red, green, blue). 
    - Also on the right platform, there is a dispenser that releases items onto the conveyor belt at random intervals between 2-5 seconds. The items are 0.5 m cubes colored either red, green, or blue.
    - The robot begins on the left platform. 

    Task:
    The robot must jump onto the conveyor belt, pick up the colored items, ride the conveyor to the right platform, and deliver each item to the target area matching its color. The robot should try to deliver as many items as possible to the correct targets within the time limit.

    After delivering an item, the robot must jump back onto the conveyor belt and return to the left platform before the next item is released. The robot should wait on the left platform for the next item.

    Rewards:
    - Provide a small reward for picking up an item from the conveyor belt.
    - Provide a large reward for delivering an item to the correct target area based on color.
    - Provide a small penalty for delivering an item to the wrong target area.
    - Provide a moderate penalty if the robot falls off the conveyor belt or platforms.

    Success Conditions:
    The task is considered complete if the robot successfully delivers at least 5 items to their correct target areas within the time limit.

    Time Limit:
    The robot has 3 minutes to deliver as many items as possible.

    Termination:
    The episode ends if the robot falls off the platforms or conveyor belt, or if the time limit is reached.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [5.0, 5.0, 0.5]
        self.conveyor_size = [5.0, 1.0, 0.2]
        self.conveyor_speed = 0.5
        self.item_size = [0.5, 0.5, 0.5]
        self.item_colors = [[1.0, 0.0, 0.0], [0.0, 1.0, 0.0], [0.0, 0.0, 1.0]]
        self.target_size = [1.0, 1.0, 0.01]
        self.target_positions = [[3.5, 1.5, 0.26], [3.5, 0.0, 0.26], [3.5, -1.5, 0.26]]
        self.dispenser_position = [-2.0, 0.0, 1.0]
        self.dispense_interval_range = [2.0, 5.0]
        self.left_platform_position = [-2.5, 0.0, 0.0]
        self.left_platform_id = self.create_box(0.0, [self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], self.left_platform_position, [0.8, 0.8, 0.8, 1.0])
        self.right_platform_position = [2.5, 0.0, 0.0]
        self.right_platform_id = self.create_box(0.0, [self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], self.right_platform_position, [0.8, 0.8, 0.8, 1.0])
        self.conveyor_position = [0.0, 0.0, self.platform_size[2] / 2 + self.conveyor_size[2] / 2]
        self.conveyor_id = self.create_box(0.0, [self.conveyor_size[0] / 2, self.conveyor_size[1] / 2, self.conveyor_size[2] / 2], self.conveyor_position, [0.3, 0.3, 0.3, 1.0])
        self.target_ids = []
        for position, color in zip(self.target_positions, self.item_colors):
            target_id = self.create_box(0.0, [self.target_size[0] / 2, self.target_size[1] / 2, self.target_size[2] / 2], position, color + [0.5])
            self.target_ids.append(target_id)
        self.item_ids = []
        self.robot_position_init = [self.left_platform_position[0], self.left_platform_position[1], self.platform_size[2] + self.robot.links['base'].position_init[2] + 0.1]
        self.time_limit = 3 * 60
        self.num_items_delivered = 0
        self.next_dispense_time = None

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self.num_items_delivered = 0
        self.next_dispense_time = self.time + np.random.uniform(*self.dispense_interval_range)
        for item_id in self.item_ids:
            self._p.removeBody(item_id)
        self.item_ids = []
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.conveyor_velocity = [self.conveyor_speed, 0.0, 0.0]
        for item_id in self.item_ids:
            item_position, _ = self._p.getBasePositionAndOrientation(item_id)
            self._p.resetBaseVelocity(item_id, self.conveyor_velocity, [0.0, 0.0, 0.0])
            if item_position[0] > self.right_platform_position[0] + self.platform_size[0] / 2:
                self._p.removeBody(item_id)
                self.item_ids.remove(item_id)
        if self.time >= self.next_dispense_time:
            self.next_dispense_time += np.random.uniform(*self.dispense_interval_range)
            color_index = np.random.randint(len(self.item_colors))
            item_id = self.create_box(1.0, [self.item_size[0] / 2, self.item_size[1] / 2, self.item_size[2] / 2], self.dispenser_position, self.item_colors[color_index] + [1.0])
            self.item_ids.append(item_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        pick_up_reward = 0.0
        if len(self._p.getContactPoints(bodyA=self.robot.robot_id, linkIndexA=-1)) > 0:
            for item_id in self.item_ids:
                if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=item_id, linkIndexA=-1)) > 0:
                    pick_up_reward = 1.0
                    break
        delivery_reward = 0.0
        wrong_delivery_penalty = 0.0
        for i, item_id in enumerate(self.item_ids):
            item_position, _ = self._p.getBasePositionAndOrientation(item_id)
            for j, target_id in enumerate(self.target_ids):
                if len(self._p.getContactPoints(bodyA=item_id, bodyB=target_id)) > 0:
                    if i == j:
                        delivery_reward = 10.0
                        self.num_items_delivered += 1
                    else:
                        wrong_delivery_penalty = -1.0
                    self._p.removeBody(item_id)
                    self.item_ids.remove(item_id)
                    break
        fall_off_penalty = 0.0
        robot_position = self.robot.links['base'].position
        if robot_position[2] < 0.0:
            fall_off_penalty = -5.0
        return {'pick_up_reward': pick_up_reward, 'delivery_reward': delivery_reward, 'wrong_delivery_penalty': wrong_delivery_penalty, 'fall_off_penalty': fall_off_penalty}

    def get_terminated(self, action):
        robot_position = self.robot.links['base'].position
        if robot_position[2] < 0.0:
            return True
        if self.time >= self.time_limit:
            return True
        return False

    def get_success(self):
        return self.num_items_delivered >= 5
\end{lstlisting}


==> env_codes/long_run/long_run_122.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Kick ball through moving gates to zones marked by moving targets.

    The environment consists of a large flat ground. A ball is placed 5 meters directly in front of the robot. After a delay of 1-2 seconds (randomized), the ball begins rolling straight ahead at a constant velocity of 1-2 m/s (randomized).

    Five vertical rectangular gates, each 3 meters tall and 1 meter wide, are placed at randomized positions between 5 to 25 meters in front of the ball's initial position, at randomized lateral offsets up to 5 meters on either side. The gates translate laterally with randomized constant velocities between 0.2-1 m/s, reversing direction each time they move 5 meters from their initial position. The gates' movement is triggered at the start of the episode.

    Five target zones are marked on the ground at randomized positions between 10 to 30 meters in front of the ball's initial position, at randomized lateral offsets up to 10 meters on either side. Each target zone is a circle with radius 2 meters. At the center of each target zone is a flat cylindrical marker, 2 meters in radius and 0.1 meters tall. The markers rotate in place with randomized constant angular velocities between 0.1-0.5 rad/s, switching between clockwise and counterclockwise rotation each time the ball passes through a gate. The markers' rotation is triggered at the start of the episode.

    The robot is initialized 3 meters behind the ball, facing the direction of the ball's initial velocity.

    The task is for the robot to kick the ball through each gate in order, aiming to get the ball to stop within the corresponding target zone after it passes through the gate. The robot should decide when and how to kick the ball based on the observed motion of the gates and markers.

    Passing through a gate awards 2 points if the ball subsequently stops in the correct target zone, and 1 point otherwise. The episode ends when the ball passes through all gates, or a maximum time limit is reached. The robot should aim to maximize its total score.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [100.0, 100.0, 0.1]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.ball_position_init = [0.0, 0.0, self.ground_size[2] / 2 + self.ball_radius]
        self.ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=self.ball_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.num_gates = 5
        self.gate_width = 1.0
        self.gate_height = 3.0
        self.gate_thickness = 0.1
        self.gate_ids = []
        self.gate_positions_init = []
        self.gate_velocities = []
        for _ in range(self.num_gates):
            gate_x = np.random.uniform(5.0, 25.0)
            gate_y = np.random.uniform(-5.0, 5.0)
            gate_position_init = [gate_x, gate_y, self.ground_size[2] / 2 + self.gate_height / 2]
            self.gate_positions_init.append(gate_position_init)
            gate_left_id = self.create_box(mass=0.0, half_extents=[self.gate_thickness / 2, self.gate_width / 2, self.gate_height / 2], position=[gate_position_init[0], gate_position_init[1] - self.gate_width / 2, gate_position_init[2]], color=[0.0, 0.0, 1.0, 1.0])
            gate_right_id = self.create_box(mass=0.0, half_extents=[self.gate_thickness / 2, self.gate_width / 2, self.gate_height / 2], position=[gate_position_init[0], gate_position_init[1] + self.gate_width / 2, gate_position_init[2]], color=[0.0, 0.0, 1.0, 1.0])
            self.gate_ids.append((gate_left_id, gate_right_id))
            gate_velocity = np.random.uniform(0.2, 1.0) * np.random.choice([-1.0, 1.0])
            self.gate_velocities.append(gate_velocity)
        self.num_targets = 5
        self.target_radius = 2.0
        self.target_height = 0.1
        self.target_ids = []
        self.target_positions_init = []
        self.target_angular_velocities = []
        for _ in range(self.num_targets):
            target_x = np.random.uniform(10.0, 30.0)
            target_y = np.random.uniform(-10.0, 10.0)
            target_position_init = [target_x, target_y, self.ground_size[2] / 2 + self.target_height / 2]
            self.target_positions_init.append(target_position_init)
            target_id = self.create_cylinder(mass=0.0, radius=self.target_radius, height=self.target_height, position=target_position_init, color=[0.0, 1.0, 0.0, 1.0])
            self.target_ids.append(target_id)
            target_angular_velocity = np.random.uniform(0.1, 0.5) * np.random.choice([-1.0, 1.0])
            self.target_angular_velocities.append(target_angular_velocity)
        self.robot_position_init = [self.ball_position_init[0] - 3.0, self.ball_position_init[1], self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])
        self.max_steps = 2000
        self.gate_counter = 0
        self.score = 0

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_object_velocity(self, object_id):
        return np.asarray(self._p.getBaseVelocity(object_id)[0])

    def reset(self):
        observation = super().reset()
        self.ball_velocity_init = [np.random.uniform(1.0, 2.0), 0.0, 0.0]
        self.ball_delay = np.random.uniform(1.0, 2.0)
        self._p.resetBasePositionAndOrientation(self.ball_id, self.ball_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBaseVelocity(self.ball_id, [0.0, 0.0, 0.0], [0.0, 0.0, 0.0])
        for i, (gate_left_id, gate_right_id) in enumerate(self.gate_ids):
            gate_position_init = self.gate_positions_init[i]
            self._p.resetBasePositionAndOrientation(gate_left_id, [gate_position_init[0], gate_position_init[1] - self.gate_width / 2, gate_position_init[2]], [0.0, 0.0, 0.0, 1.0])
            self._p.resetBasePositionAndOrientation(gate_right_id, [gate_position_init[0], gate_position_init[1] + self.gate_width / 2, gate_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        for i, target_id in enumerate(self.target_ids):
            target_position_init = self.target_positions_init[i]
            self._p.resetBasePositionAndOrientation(target_id, target_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        self.time = 0.0
        self.steps = 0
        self.gate_counter = 0
        self.score = 0
        return observation

    def step(self, action):
        self.ball_position = self.get_object_position(self.ball_id)
        self.ball_velocity = self.get_object_velocity(self.ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        self.steps += 1
        if self.time > self.ball_delay:
            self._p.resetBaseVelocity(self.ball_id, self.ball_velocity_init, [0.0, 0.0, 0.0])
        for i, (gate_left_id, gate_right_id) in enumerate(self.gate_ids):
            gate_position = self.get_object_position(gate_left_id)
            gate_velocity = self.gate_velocities[i]
            if abs(gate_position[1] - self.gate_positions_init[i][1]) > 5.0:
                gate_velocity *= -1.0
                self.gate_velocities[i] = gate_velocity
            new_gate_position = [gate_position[0], gate_position[1] + gate_velocity * self.dt, gate_position[2]]
            self._p.resetBasePositionAndOrientation(gate_left_id, [new_gate_position[0], new_gate_position[1] - self.gate_width / 2, new_gate_position[2]], [0.0, 0.0, 0.0, 1.0])
            self._p.resetBasePositionAndOrientation(gate_right_id, [new_gate_position[0], new_gate_position[1] + self.gate_width / 2, new_gate_position[2]], [0.0, 0.0, 0.0, 1.0])
        for i, target_id in enumerate(self.target_ids):
            target_position = self.get_object_position(target_id)
            target_angular_velocity = self.target_angular_velocities[i]
            target_orientation = self._p.getQuaternionFromEuler([0.0, 0.0, target_angular_velocity * self.time])
            self._p.resetBasePositionAndOrientation(target_id, target_position, target_orientation)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        gate_reward = 0.0
        if self.gate_counter < self.num_gates:
            gate_left_id, gate_right_id = self.gate_ids[self.gate_counter]
            if len(self._p.getContactPoints(bodyA=self.ball_id, bodyB=gate_left_id)) > 0 or len(self._p.getContactPoints(bodyA=self.ball_id, bodyB=gate_right_id)) > 0:
                self.gate_counter += 1
                if self.gate_counter < self.num_targets:
                    target_id = self.target_ids[self.gate_counter - 1]
                    if np.linalg.norm(self.get_object_position(self.ball_id)[:2] - self.get_object_position(target_id)[:2]) < self.target_radius:
                        gate_reward = 2.0
                    else:
                        gate_reward = 1.0
                    self.target_angular_velocities[self.gate_counter - 1] *= -1.0
                else:
                    gate_reward = 1.0
        self.score += gate_reward
        return {'gate_reward': gate_reward}

    def get_terminated(self, action):
        all_gates_passed = self.gate_counter >= self.num_gates
        time_limit_reached = self.steps >= self.max_steps
        return all_gates_passed or time_limit_reached

    def get_success(self):
        return self.gate_counter >= self.num_gates
\end{lstlisting}


==> env_codes/long_run/long_run_155.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Dynamic Target Pushing Challenge

    Description:
    - The environment is a 15 m x 15 m open area with a flat surface.
    - There are 3 dynamic targets (spheres with a 0.5 m diameter) that move along predefined linear paths. Each target moves back and forth along a 5 m path at a speed of 0.5 m/s.
    - The robot starts at the center of the area.
    - Three goal zones (1 m x 1 m squares) are located at the edges of the area: one at the north edge, one at the east edge, and one at the west edge.

    Task:
    The robot must push each moving target into its corresponding goal zone. The targets can be pushed in any order, but each target must come to rest fully within its goal zone to be considered successfully delivered.

    Initial Positions:
    - Robot: Center of the area at (0, 0, 0.5)
    - Target 1: Moving along the path from (-2.5, 5, 0.25) to (2.5, 5, 0.25)
    - Target 2: Moving along the path from (5, -2.5, 0.25) to (5, 2.5, 0.25)
    - Target 3: Moving along the path from (-5, -2.5, 0.25) to (-5, 2.5, 0.25)
    - Goal Zone 1: Centered at (0, 7, 0.05)
    - Goal Zone 2: Centered at (7, 0, 0.05)
    - Goal Zone 3: Centered at (-7, 0, 0.05)

    Success Conditions:
    The task is considered complete when all three targets come to rest fully within their respective goal zones.

    Time Limit:
    The robot has a time limit of 5 minutes to complete the task.

    Rewards:
    - Provide a small reward for moving closer to a target.
    - Provide a moderate reward for reaching a target.
    - Provide a large reward for pushing a target towards its goal zone.
    - Provide a significant reward for delivering a target to its goal zone.
    - Apply a small penalty for collisions with the targets or the boundaries of the area.

    Termination:
    The episode terminates if the robot flips over, if a target is pushed out of bounds, or if the time limit is exceeded. The episode should terminate with success if all targets are delivered to their goal zones.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [15.0, 15.0, 0.1]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.target_radius = 0.25
        self.target_speed = 0.5
        self.target_paths = [{'start': [-2.5, 5.0, self.target_radius], 'end': [2.5, 5.0, self.target_radius]}, {'start': [5.0, -2.5, self.target_radius], 'end': [5.0, 2.5, self.target_radius]}, {'start': [-5.0, -2.5, self.target_radius], 'end': [-5.0, 2.5, self.target_radius]}]
        self.target_ids = []
        for path in self.target_paths:
            target_id = self.create_sphere(mass=1.0, radius=self.target_radius, position=path['start'], color=[1.0, 0.0, 0.0, 1.0])
            self.target_ids.append(target_id)
        self.goal_size = [1.0, 1.0, 0.1]
        self.goal_positions = [[0.0, 7.0, self.goal_size[2] / 2], [7.0, 0.0, self.goal_size[2] / 2], [-7.0, 0.0, self.goal_size[2] / 2]]
        self.goal_ids = []
        for position in self.goal_positions:
            goal_id = self.create_box(mass=0.0, half_extents=[self.goal_size[0] / 2, self.goal_size[1] / 2, self.goal_size[2] / 2], position=position, color=[0.0, 1.0, 0.0, 1.0])
            self.goal_ids.append(goal_id)
        self.robot_position_init = [0.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.time_limit = 300.0

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        for i, path in enumerate(self.target_paths):
            self._p.resetBasePositionAndOrientation(self.target_ids[i], path['start'], [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_targets = [self.get_distance_to_object(target_id) for target_id in self.target_ids]
        observation, reward, terminated, truncated, info = super().step(action)
        for i, path in enumerate(self.target_paths):
            start = np.array(path['start'])
            end = np.array(path['end'])
            direction = (end - start) / np.linalg.norm(end - start)
            distance = self.target_speed * self.time
            new_position = start + direction * (distance % (2 * np.linalg.norm(end - start)))
            if distance // np.linalg.norm(end - start) % 2 == 1:
                new_position = end - (new_position - start)
            self._p.resetBasePositionAndOrientation(self.target_ids[i], new_position, [0.0, 0.0, 0.0, 1.0])
        self.time += self.dt
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distances_to_targets = [self.get_distance_to_object(target_id) for target_id in self.target_ids]
        rewards = {'move_closer_to_target': 0.0, 'reach_target': 0.0, 'push_to_goal': 0.0, 'deliver_to_goal': 0.0, 'collision_penalty': 0.0}
        for i, target_id in enumerate(self.target_ids):
            rewards['move_closer_to_target'] += (self.distance_to_targets[i] - new_distances_to_targets[i]) / self.dt
            if new_distances_to_targets[i] < self.target_radius:
                rewards['reach_target'] += 10.0
            distance_to_goal = self.get_distance_to_object(self.goal_ids[i])
            new_distance_to_goal = np.linalg.norm(self.get_object_position(target_id)[:2] - self.goal_positions[i][:2])
            rewards['push_to_goal'] += (distance_to_goal - new_distance_to_goal) / self.dt
            if new_distance_to_goal < self.goal_size[0] / 2:
                rewards['deliver_to_goal'] += 50.0
            if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=target_id)) > 0:
                rewards['collision_penalty'] -= 1.0
        return rewards

    def get_terminated(self, action):
        is_flipped = np.dot(np.asarray([0, 0, 1]), np.asarray(self._p.getMatrixFromQuaternion(self.robot.links['base'].orientation)).reshape(3, 3)[:, 2]) < 0.5
        is_time_up = self.time >= self.time_limit
        is_out_of_bounds = any((np.any(np.abs(self.get_object_position(target_id)[:2]) > np.array(self.ground_size[:2]) / 2) for target_id in self.target_ids))
        return is_flipped or is_time_up or is_out_of_bounds

    def get_success(self):
        return all((np.linalg.norm(self.get_object_position(target_id)[:2] - self.goal_positions[i][:2]) < self.goal_size[0] / 2 for i, target_id in enumerate(self.target_ids)))
\end{lstlisting}


==> env_codes/long_run/long_run_176.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Push two balls into separate goals while avoiding static obstacles.

    Description:
    - The environment consists of a large flat ground.
    - Two balls, one red and one blue, are placed at fixed initial positions on the ground. The red ball is positioned at [2.0, -2.0, 0.5] and the blue ball is positioned at [2.0, 2.0, 0.5].
    - Two goal areas are defined by pairs of posts. The red goal is defined by posts placed at [10.0, -2.0, 1.0] and [10.0, -1.0, 1.0]. The blue goal is defined by posts placed at [10.0, 1.0, 1.0] and [10.0, 2.0, 1.0].
    - Three cylindrical obstacles of 1 meter radius and 2 meters height are placed at fixed positions: [5.0, 0.0, 1.0], [7.0, -1.0, 1.0], and [7.0, 1.0, 1.0].
    - The robot is initialized at [0.0, 0.0, 0.5], facing the positive x-direction.
    - The task is for the robot to push the red ball into the red goal and the blue ball into the blue goal while avoiding the obstacles.

    Success:
    The task is completed successfully if the robot pushes both balls into their respective goals without colliding with any obstacles.

    Rewards:
    - The robot is rewarded for decreasing its distance to each ball.
    - The robot is rewarded for pushing each ball towards its respective goal.
    - The robot is penalized for colliding with obstacles.
    - The robot is greatly rewarded if a ball passes between the goal posts of its respective goal.

    Termination:
    The task is terminated if the robot collides with an obstacle, if a ball collides with an obstacle, or if a time limit of 60 seconds is reached.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [1000.0, 1000.0, 10.0]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.red_ball_position_init = [2.0, -2.0, self.ground_size[2] / 2 + self.ball_radius]
        self.blue_ball_position_init = [2.0, 2.0, self.ground_size[2] / 2 + self.ball_radius]
        self.red_ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=self.red_ball_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.blue_ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=self.blue_ball_position_init, color=[0.0, 0.0, 1.0, 1.0])
        self.goal_post_height = 2.0
        self.goal_post_radius = 0.1
        self.red_goal_position = [10.0, -1.5, self.ground_size[2] / 2 + self.goal_post_height / 2]
        self.blue_goal_position = [10.0, 1.5, self.ground_size[2] / 2 + self.goal_post_height / 2]
        self.red_goal_post_left_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.red_goal_position[0], self.red_goal_position[1] - 0.5, self.red_goal_position[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.red_goal_post_right_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.red_goal_position[0], self.red_goal_position[1] + 0.5, self.red_goal_position[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.blue_goal_post_left_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.blue_goal_position[0], self.blue_goal_position[1] - 0.5, self.blue_goal_position[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.blue_goal_post_right_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.blue_goal_position[0], self.blue_goal_position[1] + 0.5, self.blue_goal_position[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.obstacle_radius = 1.0
        self.obstacle_height = 2.0
        self.obstacle_positions = [[5.0, 0.0, self.ground_size[2] / 2 + self.obstacle_height / 2], [7.0, -1.0, self.ground_size[2] / 2 + self.obstacle_height / 2], [7.0, 1.0, self.ground_size[2] / 2 + self.obstacle_height / 2]]
        self.obstacle_ids = [self.create_cylinder(mass=0.0, radius=self.obstacle_radius, height=self.obstacle_height, position=pos, color=[0.0, 0.0, 0.0, 1.0]) for pos in self.obstacle_positions]
        self.robot_position_init = [0.0, 0.0, self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])
        self.time_limit = 60.0

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.red_ball_id, self.red_ball_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.blue_ball_id, self.blue_ball_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        return observation

    def step(self, action):
        self.distance_to_red_ball = self.get_distance_to_object(self.red_ball_id)
        self.distance_to_blue_ball = self.get_distance_to_object(self.blue_ball_id)
        self.red_ball_position = self.get_object_position(self.red_ball_id)
        self.blue_ball_position = self.get_object_position(self.blue_ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_red_ball = self.get_distance_to_object(self.red_ball_id)
        new_distance_to_blue_ball = self.get_distance_to_object(self.blue_ball_id)
        new_red_ball_position = self.get_object_position(self.red_ball_id)
        new_blue_ball_position = self.get_object_position(self.blue_ball_id)
        survival = 1.0
        reach_red_ball = (self.distance_to_red_ball - new_distance_to_red_ball) / self.dt
        reach_blue_ball = (self.distance_to_blue_ball - new_distance_to_blue_ball) / self.dt
        push_red_ball = (new_red_ball_position[0] - self.red_ball_position[0]) / self.dt
        push_blue_ball = (new_blue_ball_position[0] - self.blue_ball_position[0]) / self.dt
        collision_penalty = 0.0
        for obstacle_id in self.obstacle_ids:
            if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0:
                collision_penalty = -10.0
                break
        red_ball_in_goal = 0.0
        if self.red_goal_position[1] - 0.5 < new_red_ball_position[1] < self.red_goal_position[1] + 0.5 and new_red_ball_position[0] > self.red_goal_position[0]:
            red_ball_in_goal = 10.0
        blue_ball_in_goal = 0.0
        if self.blue_goal_position[1] - 0.5 < new_blue_ball_position[1] < self.blue_goal_position[1] + 0.5 and new_blue_ball_position[0] > self.blue_goal_position[0]:
            blue_ball_in_goal = 10.0
        return {'survival': survival, 'reach_red_ball': reach_red_ball, 'reach_blue_ball': reach_blue_ball, 'push_red_ball': push_red_ball, 'push_blue_ball': push_blue_ball, 'collision_penalty': collision_penalty, 'red_ball_in_goal': red_ball_in_goal, 'blue_ball_in_goal': blue_ball_in_goal}

    def get_terminated(self, action):
        for obstacle_id in self.obstacle_ids:
            if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0:
                return True
        for obstacle_id in self.obstacle_ids:
            if len(self._p.getContactPoints(bodyA=self.red_ball_id, bodyB=obstacle_id)) > 0 or len(self._p.getContactPoints(bodyA=self.blue_ball_id, bodyB=obstacle_id)) > 0:
                return True
        if self.time >= self.time_limit:
            return True
        return False

    def get_success(self):
        red_ball_position = self.get_object_position(self.red_ball_id)
        blue_ball_position = self.get_object_position(self.blue_ball_id)
        red_ball_in_goal = self.red_goal_position[1] - 0.5 < red_ball_position[1] < self.red_goal_position[1] + 0.5 and red_ball_position[0] > self.red_goal_position[0]
        blue_ball_in_goal = self.blue_goal_position[1] - 0.5 < blue_ball_position[1] < self.blue_goal_position[1] + 0.5 and blue_ball_position[0] > self.blue_goal_position[0]
        return red_ball_in_goal and blue_ball_in_goal
\end{lstlisting}


==> env_codes/long_run/long_run_178.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Coordinate with another moving ball to hit a target

    Description:
    - The environment consists of a large flat ground.
    - Two balls are placed 5 meters in front of the robot, spaced 2 meters apart laterally. Both balls begin rolling in parallel at 1 m/s after a short delay of 1 second.
    - A target area defined by a 2x2 meter flat vertical target is placed 10 meters from the balls' initial position. The target moves laterally back and forth at 0.5 m/s, covering 3 meters to each side before reversing direction.
    - The robot is initialized 3 meters behind the balls, facing the direction of the target.
    - The task is for the robot to coordinate its movements to kick both balls such that they hit the moving target simultaneously.

    Success:
    The task is completed successfully if both balls hit the front face of the moving target simultaneously.

    Rewards:
    - The robot is rewarded for decreasing the distance to each ball as they move.
    - The robot is rewarded for matching the velocity of each ball as it approaches.
    - The robot is rewarded for kicking each ball with a velocity that is likely to reach the target.
    - The robot is greatly rewarded if both balls hit the front face of the moving target simultaneously.

    Termination:
    The task is terminated if either ball stops moving, if the balls do not hit the target simultaneously, or if a time limit of 30 seconds is reached.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [100.0, 100.0, 0.1]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.ball_velocity_init = [1.0, 0.0, 0.0]
        self.ball1_position_init = [0.0, -1.0, self.ground_size[2] / 2 + self.ball_radius]
        self.ball2_position_init = [0.0, 1.0, self.ground_size[2] / 2 + self.ball_radius]
        self.ball1_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=self.ball1_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.ball2_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=self.ball2_position_init, color=[0.0, 0.0, 1.0, 1.0])
        self.target_size = [2.0, 0.1, 2.0]
        self.target_position_init = [10.0, 0.0, self.ground_size[2] / 2 + self.target_size[2] / 2]
        self.target_velocity = 0.5
        self.target_id = self.create_box(mass=0.0, half_extents=[self.target_size[0] / 2, self.target_size[1] / 2, self.target_size[2] / 2], position=self.target_position_init, color=[0.0, 1.0, 0.0, 1.0])
        self.robot_position_init = [self.ball1_position_init[0] - 3.0, 0.0, self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])
        self.ball_velocity_threshold = 0.1
        self.max_steps = 1000
        self.target_movement_range = 3.0

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_object_velocity(self, object_id):
        return np.asarray(self._p.getBaseVelocity(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.steps = 0
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.ball1_id, self.ball1_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBaseVelocity(self.ball1_id, [0.0, 0.0, 0.0], [0.0, 0.0, 0.0])
        self._p.resetBasePositionAndOrientation(self.ball2_id, self.ball2_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBaseVelocity(self.ball2_id, [0.0, 0.0, 0.0], [0.0, 0.0, 0.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        self._p.resetBasePositionAndOrientation(self.target_id, self.target_position_init, [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_ball1 = self.get_distance_to_object(self.ball1_id)
        self.distance_to_ball2 = self.get_distance_to_object(self.ball2_id)
        self.ball1_position = self.get_object_position(self.ball1_id)
        self.ball2_position = self.get_object_position(self.ball2_id)
        self.ball1_velocity = self.get_object_velocity(self.ball1_id)
        self.ball2_velocity = self.get_object_velocity(self.ball2_id)
        robot_base_link_state = self._p.getBaseVelocity(self.robot.robot_id)
        self.robot_velocity = robot_base_link_state[0]
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        self.steps += 1
        if self.time > 1.0:
            self._p.resetBaseVelocity(self.ball1_id, self.ball_velocity_init, [0.0, 0.0, 0.0])
            self._p.resetBaseVelocity(self.ball2_id, self.ball_velocity_init, [0.0, 0.0, 0.0])
        target_new_y = self.target_position_init[1] + self.target_movement_range * np.sin(self.target_velocity * self.time)
        self._p.resetBasePositionAndOrientation(self.target_id, [self.target_position_init[0], target_new_y, self.target_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_ball1 = self.get_distance_to_object(self.ball1_id)
        new_distance_to_ball2 = self.get_distance_to_object(self.ball2_id)
        new_ball1_position = self.get_object_position(self.ball1_id)
        new_ball2_position = self.get_object_position(self.ball2_id)
        new_ball1_velocity = self.get_object_velocity(self.ball1_id)
        new_ball2_velocity = self.get_object_velocity(self.ball2_id)
        robot_base_link_state = self._p.getBaseVelocity(self.robot.robot_id)
        new_robot_velocity = robot_base_link_state[0]
        reach_ball1 = (self.distance_to_ball1 - new_distance_to_ball1) / self.dt
        reach_ball2 = (self.distance_to_ball2 - new_distance_to_ball2) / self.dt
        velocity_match1 = 0.0
        if new_distance_to_ball1 < 1.0:
            velocity_match1 = -np.linalg.norm(new_ball1_velocity[:2] - new_robot_velocity[:2])
        velocity_match2 = 0.0
        if new_distance_to_ball2 < 1.0:
            velocity_match2 = -np.linalg.norm(new_ball2_velocity[:2] - new_robot_velocity[:2])
        kick_velocity1 = 0.0
        if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.ball1_id)) > 0:
            kick_velocity1 = np.linalg.norm(new_ball1_velocity)
        kick_velocity2 = 0.0
        if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.ball2_id)) > 0:
            kick_velocity2 = np.linalg.norm(new_ball2_velocity)
        ball1_in_target = 0.0
        ball2_in_target = 0.0
        if self.target_position_init[1] - self.target_movement_range / 2 < new_ball1_position[1] < self.target_position_init[1] + self.target_movement_range / 2 and new_ball1_position[0] > self.target_position_init[0]:
            ball1_in_target = 10.0
        if self.target_position_init[1] - self.target_movement_range / 2 < new_ball2_position[1] < self.target_position_init[1] + self.target_movement_range / 2 and new_ball2_position[0] > self.target_position_init[0]:
            ball2_in_target = 10.0
        simultaneous_hit = 0.0
        if ball1_in_target > 0 and ball2_in_target > 0 and (np.abs(new_ball1_position[0] - new_ball2_position[0]) < 0.1):
            simultaneous_hit = 20.0
        return {'reach_ball1': reach_ball1, 'reach_ball2': reach_ball2, 'velocity_match1': velocity_match1, 'velocity_match2': velocity_match2, 'kick_velocity1': kick_velocity1, 'kick_velocity2': kick_velocity2, 'ball1_in_target': ball1_in_target, 'ball2_in_target': ball2_in_target, 'simultaneous_hit': simultaneous_hit}

    def get_terminated(self, action):
        ball1_stopped = self.steps > 10 and np.linalg.norm(self.ball1_velocity) < self.ball_velocity_threshold
        ball2_stopped = self.steps > 10 and np.linalg.norm(self.ball2_velocity) < self.ball_velocity_threshold
        time_limit_reached = self.steps >= self.max_steps
        return ball1_stopped or ball2_stopped or time_limit_reached

    def get_success(self):
        ball1_position = self.get_object_position(self.ball1_id)
        ball2_position = self.get_object_position(self.ball2_id)
        ball1_in_target = self.target_position_init[1] - self.target_movement_range / 2 < ball1_position[1] < self.target_position_init[1] + self.target_movement_range / 2 and ball1_position[0] > self.target_position_init[0]
        ball2_in_target = self.target_position_init[1] - self.target_movement_range / 2 < ball2_position[1] < self.target_position_init[1] + self.target_movement_range / 2 and ball2_position[0] > self.target_position_init[0]
        simultaneous_hit = ball1_in_target and ball2_in_target and (np.abs(ball1_position[0] - ball2_position[0]) < 0.1)
        return simultaneous_hit
\end{lstlisting}


==> env_codes/long_run/long_run_196.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Dodgeball Arena

    Description:
    - The environment is a 15 m x 15 m walled arena with a flat ground surface.
    - There are 5 automatic ball launchers positioned around the perimeter of the arena. Each launcher can shoot a foam ball (0.2 m diameter) at varying speeds (up to 5 m/s) and angles.
    - The launchers are programmed to shoot balls at random intervals (between 1 to 3 seconds) and in random directions.
    - The robot starts in the center of the arena.

    Task:
    The robot must avoid being hit by the foam balls for as long as possible. The robot can move around the arena and jump to dodge the balls.

    Success Conditions:
    The task is considered successful if the robot can avoid being hit by any balls for a duration of 2 minutes.

    Rewards:
    - Provide a small reward for each second the robot avoids being hit.
    - Provide a large reward for successfully avoiding all balls for the entire duration.
    - Apply a small penalty for each ball that hits the robot.

    Termination:
    The episode ends if the robot is hit by a ball, or if the time limit of 2 minutes is exceeded.
    """

    def __init__(self):
        super().__init__()
        self.arena_size = [15.0, 15.0, 0.1]
        self.arena_position = [0.0, 0.0, 0.0]
        self.arena_id = self.create_box(mass=0.0, half_extents=[self.arena_size[0] / 2, self.arena_size[1] / 2, self.arena_size[2] / 2], position=self.arena_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.arena_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.wall_thickness = 0.1
        self.wall_height = 2.0
        self.create_walls()
        self.num_launchers = 5
        self.launcher_positions = [[self.arena_size[0] / 2 - self.wall_thickness, 0.0, self.wall_height / 2], [-self.arena_size[0] / 2 + self.wall_thickness, 0.0, self.wall_height / 2], [0.0, self.arena_size[1] / 2 - self.wall_thickness, self.wall_height / 2], [0.0, -self.arena_size[1] / 2 + self.wall_thickness, self.wall_height / 2], [self.arena_size[0] / 2 - self.wall_thickness, self.arena_size[1] / 2 - self.wall_thickness, self.wall_height / 2]]
        self.launcher_ids = [self.create_launcher(position) for position in self.launcher_positions]
        self.ball_radius = 0.1
        self.ball_speed_max = 5.0
        self.ball_interval_min = 1.0
        self.ball_interval_max = 3.0
        self.balls = []
        self.robot_position_init = [0.0, 0.0, self.robot.links['base'].position_init[2]]
        self.time_limit = 120.0

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_walls(self):
        wall_positions = [[self.arena_size[0] / 2 + self.wall_thickness / 2, 0.0, self.wall_height / 2], [-self.arena_size[0] / 2 - self.wall_thickness / 2, 0.0, self.wall_height / 2], [0.0, self.arena_size[1] / 2 + self.wall_thickness / 2, self.wall_height / 2], [0.0, -self.arena_size[1] / 2 - self.wall_thickness / 2, self.wall_height / 2]]
        wall_sizes = [[self.wall_thickness, self.arena_size[1], self.wall_height], [self.wall_thickness, self.arena_size[1], self.wall_height], [self.arena_size[0], self.wall_thickness, self.wall_height], [self.arena_size[0], self.wall_thickness, self.wall_height]]
        for position, size in zip(wall_positions, wall_sizes):
            self.create_box(mass=0.0, half_extents=[size[0] / 2, size[1] / 2, size[2] / 2], position=position, color=[0.2, 0.2, 0.2, 1.0])

    def create_launcher(self, position):
        launcher_size = [0.5, 0.5, 0.5]
        return self.create_box(mass=0.0, half_extents=[launcher_size[0] / 2, launcher_size[1] / 2, launcher_size[2] / 2], position=position, color=[1.0, 0.0, 0.0, 1.0])

    def launch_ball(self, launcher_id):
        launcher_position = self.get_object_position(launcher_id)
        angle = np.random.uniform(0, 2 * np.pi)
        speed = np.random.uniform(0, self.ball_speed_max)
        velocity = [speed * np.cos(angle), speed * np.sin(angle), 0.0]
        ball_position = [launcher_position[0], launcher_position[1], self.ball_radius]
        ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=ball_position, color=[1.0, 1.0, 0.0, 1.0])
        self._p.resetBaseVelocity(ball_id, linearVelocity=velocity)
        self.balls.append(ball_id)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self.balls = []
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        if np.random.uniform(0, 1) < self.dt / np.random.uniform(self.ball_interval_min, self.ball_interval_max):
            launcher_id = np.random.choice(self.launcher_ids)
            self.launch_ball(launcher_id)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        survival_reward = 1.0
        ball_collision_penalty = 0.0
        for ball_id in self.balls:
            if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=ball_id)) > 0:
                ball_collision_penalty = -10.0
                break
        success_reward = 0.0
        if self.time >= self.time_limit:
            success_reward = 100.0
        return {'survival': survival_reward, 'ball_collision': ball_collision_penalty, 'success': success_reward}

    def get_terminated(self, action):
        for ball_id in self.balls:
            if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=ball_id)) > 0:
                return True
        if self.time >= self.time_limit:
            return True
        return False

    def get_success(self):
        return self.time >= self.time_limit
\end{lstlisting}


==> env_codes/long_run/long_run_197.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Jumping Over Gaps

    Description:
    - The environment consists of a 10 m x 10 m platform with a series of gaps that the robot must jump over.
    - The platform is divided into three sections:
      1. The first section (3 m x 10 m) has three gaps, each 0.5 m wide, spaced 2 m apart.
      2. The second section (3 m x 10 m) has two gaps, each 1 m wide, spaced 3 m apart.
      3. The third section (4 m x 10 m) has one gap, 1.5 m wide, located 2 m from the end of the platform.

    - The robot begins at the start of the platform, facing the positive x-axis.

    Task:
    The robot must navigate through the three sections of the platform, jumping over the gaps to reach the end of the platform.

    Success Conditions:
    The task is considered complete when the robot reaches the end of the platform without falling into any gaps.

    Rewards:
    - Provide a small reward for each gap successfully jumped over.
    - Provide a large reward for reaching the end of the platform.
    - Apply a small penalty for each failed jump (falling into a gap).

    Termination:
    The episode ends if the robot falls into a gap, flips over, or reaches the end of the platform.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [10.0, 10.0, 0.1]
        self.platform_position = [0.0, 0.0, 0.0]
        self.platform_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.platform_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.gap_widths = [0.5, 0.5, 0.5, 1.0, 1.0, 1.5]
        self.gap_positions = [[1.5, 0.0, self.platform_position[2] + self.platform_size[2] / 2], [3.5, 0.0, self.platform_position[2] + self.platform_size[2] / 2], [5.5, 0.0, self.platform_position[2] + self.platform_size[2] / 2], [8.0, 0.0, self.platform_position[2] + self.platform_size[2] / 2], [11.0, 0.0, self.platform_position[2] + self.platform_size[2] / 2], [15.0, 0.0, self.platform_position[2] + self.platform_size[2] / 2]]
        self.gap_ids = []
        for i, gap_width in enumerate(self.gap_widths):
            gap_id = self.create_box(mass=0.0, half_extents=[gap_width / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.gap_positions[i], color=[0.0, 0.0, 0.0, 1.0])
            self.gap_ids.append(gap_id)
        self.robot_position_init = [self.platform_position[0] - self.platform_size[0] / 2 + 0.5, self.platform_position[1], self.platform_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.position = self.robot.links['base'].position
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_position = self.robot.links['base'].position
        survival = 1.0
        gap_reward = 0.0
        for i, gap_position in enumerate(self.gap_positions):
            if self.position[0] < gap_position[0] and new_position[0] >= gap_position[0]:
                gap_reward += 1.0
        end_reward = 10.0 if new_position[0] > self.platform_size[0] / 2 else 0.0
        return {'survival': survival, 'gap_reward': gap_reward, 'end_reward': end_reward}

    def get_terminated(self, action):
        if self.robot.links['base'].position[2] < self.platform_position[2]:
            return True
        if self.robot.links['base'].position[0] > self.platform_size[0] / 2:
            return True
        return False

    def get_success(self):
        return self.robot.links['base'].position[0] > self.platform_size[0] / 2
\end{lstlisting}


==> env_codes/long_run/long_run_23.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Search and Rescue in a Multi-Room Environment

    Description: 
    - The environment consists of a large, two-story building with multiple rooms connected by doors, hallways, and staircases. The layout is fixed but contains challenging features:
      - 8 rooms total (4 on each floor), connected by 2 hallways (one per floor)
      - Each room is 5 m x 5 m. Hallways are 20 m long and 2 m wide. Staircase is 5 m long.
      - Rooms contain various static and movable obstacles like furniture.
      - Doors are 1 m wide and initially closed. Robot must push them open.
    - A target object (a 0.5 m x 0.5 m x 1 m box) representing a person is located in one of the rooms on the second floor. Its location is fixed for now.
    - The robot starts at the entrance of the building on the first floor.
    - The robot must systematically explore the building, locate the target object, attach a virtual tether to it, and guide it back to the entrance while avoiding obstacles.

    Success Conditions:
    The task is considered complete when the robot brings the target object to rest within 2 m of the entrance location. 

    Time Limit:
    The robot has a time limit of 10 minutes to complete the task.

    Rewards:
    - Provide a small reward for exploring new areas of the environment.
    - Provide a moderate reward for locating the target object.
    - Provide a large reward for successfully bringing the target object to the goal location.
    - Provide a small penalty for collisions with obstacles to encourage careful navigation.

    Termination:
    The episode terminates if the robot flips over or if the time limit is exceeded.
    """

    def __init__(self):
        super().__init__()
        self.room_size = 5.0
        self.hallway_length = 20.0
        self.hallway_width = 2.0
        self.staircase_length = 5.0
        self.num_rooms_per_floor = 4
        self.num_floors = 2
        self.wall_thickness = 0.5
        self.wall_height = 2.0
        self.door_width = 1.0
        self.target_object_size = [0.5, 0.5, 1.0]
        self.entrance_position = [-self.hallway_length / 2, 0.0, 0.0]
        self.time_limit = 600.0
        self.wall_color = [0.5, 0.5, 0.5, 1.0]
        self.floor_color = [1.0, 1.0, 1.0, 1.0]
        self.target_object_color = [1.0, 0.0, 0.0, 1.0]
        self.maze = self.generate_maze()
        self.floor_ids = []
        for i in range(self.num_floors):
            floor_id = self.create_box(mass=0.0, half_extents=[self.hallway_length / 2, self.hallway_width / 2, 0.1], position=[0.0, 0.0, i * self.wall_height - 0.1], color=self.floor_color)
            self.floor_ids.append(floor_id)
        self.wall_ids = []
        for wall in self.maze:
            wall_id = self.create_box(mass=0.0, half_extents=[wall[1][0] / 2, wall[1][1] / 2, self.wall_height / 2], position=[wall[0][0], wall[0][1], wall[0][2] + self.wall_height / 2], color=self.wall_color)
            self.wall_ids.append(wall_id)
        self.target_object_id = self.create_box(mass=1.0, half_extents=[self.target_object_size[0] / 2, self.target_object_size[1] / 2, self.target_object_size[2] / 2], position=[self.room_size / 2, self.room_size / 2, self.wall_height + self.target_object_size[2] / 2], color=self.target_object_color)
        self.robot_position_init = [self.entrance_position[0] + self.robot.links['base'].position_init[0] + 1.0, self.entrance_position[1] + self.robot.links['base'].position_init[1], self.entrance_position[2] + self.robot.links['base'].position_init[2] + 0.5]

    def generate_maze(self):
        maze = []
        maze.append(([0.0, -self.hallway_width / 2, 0.0], [self.hallway_length, self.wall_thickness, self.wall_height]))
        maze.append(([0.0, self.hallway_width / 2, 0.0], [self.hallway_length, self.wall_thickness, self.wall_height]))
        maze.append(([-self.hallway_length / 2, 0.0, 0.0], [self.wall_thickness, self.hallway_width, self.wall_height]))
        maze.append(([self.hallway_length / 2, 0.0, 0.0], [self.wall_thickness, self.hallway_width, self.wall_height]))
        for i in range(self.num_rooms_per_floor):
            room_position = [-self.hallway_length / 2 + (i + 0.5) * self.room_size, self.hallway_width / 2 + self.room_size / 2, 0.0]
            maze.append((room_position, [self.room_size, self.wall_thickness, self.wall_height]))
            maze.append(([room_position[0], room_position[1] - self.room_size, 0.0], [self.room_size, self.wall_thickness, self.wall_height]))
            maze.append(([room_position[0] - self.room_size / 2, room_position[1] - self.room_size / 2, 0.0], [self.wall_thickness, self.room_size, self.wall_height]))
            maze.append(([room_position[0] + self.room_size / 2, room_position[1] - self.room_size / 2, 0.0], [self.wall_thickness, self.room_size - self.door_width, self.wall_height]))
        maze.append(([0.0, -self.hallway_width / 2, self.wall_height], [self.hallway_length, self.wall_thickness, self.wall_height]))
        maze.append(([0.0, self.hallway_width / 2, self.wall_height], [self.hallway_length, self.wall_thickness, self.wall_height]))
        maze.append(([-self.hallway_length / 2, 0.0, self.wall_height], [self.wall_thickness, self.hallway_width, self.wall_height]))
        maze.append(([self.hallway_length / 2, 0.0, self.wall_height], [self.wall_thickness, self.hallway_width, self.wall_height]))
        for i in range(self.num_rooms_per_floor):
            room_position = [-self.hallway_length / 2 + (i + 0.5) * self.room_size, -self.hallway_width / 2 - self.room_size / 2, self.wall_height]
            maze.append((room_position, [self.room_size, self.wall_thickness, self.wall_height]))
            maze.append(([room_position[0], room_position[1] + self.room_size, self.wall_height], [self.room_size, self.wall_thickness, self.wall_height]))
            maze.append(([room_position[0] - self.room_size / 2, room_position[1] + self.room_size / 2, self.wall_height], [self.wall_thickness, self.room_size - self.door_width, self.wall_height]))
            maze.append(([room_position[0] + self.room_size / 2, room_position[1] + self.room_size / 2, self.wall_height], [self.wall_thickness, self.room_size, self.wall_height]))
        maze.append(([-self.hallway_length / 2 + self.room_size, 0.0, 0.0], [self.staircase_length, self.hallway_width, self.wall_height]))
        maze.append(([-self.hallway_length / 2 + self.room_size, 0.0, self.wall_height], [self.staircase_length, self.hallway_width, self.wall_height]))
        return maze

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        self.time = 0.0
        self.explored_areas = set()
        self.found_target_object = False
        self.attached_target_object = False
        return observation

    def step(self, action):
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        if self.time >= self.time_limit:
            truncated = True
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        robot_position = self.robot.links['base'].position
        exploration_reward = 0.0
        current_area = (int(robot_position[0] // self.room_size), int(robot_position[1] // self.room_size), int(robot_position[2] // self.wall_height))
        if current_area not in self.explored_areas:
            exploration_reward = 1.0
            self.explored_areas.add(current_area)
        target_object_reward = 0.0
        if not self.found_target_object and self.is_robot_close_to_target_object():
            target_object_reward = 10.0
            self.found_target_object = True
        goal_reward = 0.0
        if self.attached_target_object and self.is_target_object_close_to_entrance():
            goal_reward = 100.0
        collision_penalty = 0.0
        if self.is_colliding_with_obstacles():
            collision_penalty = -1.0
        return {'exploration_reward': exploration_reward, 'target_object_reward': target_object_reward, 'goal_reward': goal_reward, 'collision_penalty': collision_penalty}

    def get_terminated(self, action):
        return self.is_robot_flipped() or (self.attached_target_object and self.is_target_object_close_to_entrance())

    def get_success(self):
        return self.attached_target_object and self.is_target_object_close_to_entrance()

    def is_robot_close_to_target_object(self):
        robot_position = self.robot.links['base'].position
        target_object_position = self._p.getBasePositionAndOrientation(self.target_object_id)[0]
        distance = np.linalg.norm(np.array(robot_position) - np.array(target_object_position))
        return distance < 1.0

    def is_target_object_close_to_entrance(self):
        target_object_position = self._p.getBasePositionAndOrientation(self.target_object_id)[0]
        distance = np.linalg.norm(np.array(target_object_position) - np.array(self.entrance_position))
        return distance < 2.0

    def is_colliding_with_obstacles(self):
        for obstacle_id in self.wall_ids:
            if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0:
                return True
        return False

    def is_robot_flipped(self):
        robot_orientation = self._p.getEulerFromQuaternion(self.robot.links['base'].orientation)
        return abs(robot_orientation[0]) > np.pi / 4 or abs(robot_orientation[1]) > np.pi / 4
\end{lstlisting}


==> env_codes/long_run/long_run_60.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Simplified 1-vs-1 robot soccer.

    Description:
    - The environment consists of a large flat ground representing a soccer field.
    - Two goals are placed on opposite ends of the field, each defined by two posts 2 meters high and 3 meters apart.  
    - The robot is placed on one side of the field, facing the opponent's goal.
    - A basic opponent robot is placed on the other side, initially stationary.
    - A soccer ball is placed in the center of the field.
    - The objective is for the robot to navigate to the ball, take possession of it, and kick it into the opponent's goal while defending its own goal.
    - In the first stage, the opponent robot remains stationary. In the second stage, the opponent robot also moves to chase after the ball and attempt to kick it into the robot's goal.

    Success:
    The task is completed successfully if the robot is able to kick the ball into the opponent's goal while preventing the opponent from scoring.

    Rewards:
    - The robot is rewarded for possessing the ball, defined as being within 1 meter of the ball while the opponent is not.
    - The robot is rewarded for bringing the ball closer to the opponent's goal.
    - The robot is rewarded for kicking the ball with a velocity toward the opponent's goal.
    - The robot is penalized if the opponent takes possession of the ball or if the ball goes out of bounds.
    - The robot is greatly rewarded for scoring a goal and penalized if the opponent scores.

    Termination:
    The task is terminated if a goal is scored by either side, if the ball goes out of bounds, or if a time limit is reached.
    """

    def __init__(self):
        super().__init__()
        self.field_size = [40.0, 20.0, 10.0]
        self.field_position = [0.0, 0.0, 0.0]
        self.field_id = self.create_box(mass=0.0, half_extents=[self.field_size[0] / 2, self.field_size[1] / 2, self.field_size[2] / 2], position=self.field_position, color=[0.0, 0.5, 0.0, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.field_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.ball_position_init = [0.0, 0.0, self.field_size[2] / 2 + self.ball_radius]
        self.ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=self.ball_position_init, color=[1.0, 1.0, 1.0, 1.0])
        self.goal_post_height = 2.0
        self.goal_post_radius = 0.1
        self.goal_width = 3.0
        self.goal_1_position = [self.field_size[0] / 2, 0.0, self.field_size[2] / 2 + self.goal_post_height / 2]
        self.goal_1_post_left_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_1_position[0], self.goal_1_position[1] - self.goal_width / 2, self.goal_1_position[2]], color=[1.0, 0.0, 0.0, 1.0])
        self.goal_1_post_right_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_1_position[0], self.goal_1_position[1] + self.goal_width / 2, self.goal_1_position[2]], color=[1.0, 0.0, 0.0, 1.0])
        self.goal_2_position = [-self.field_size[0] / 2, 0.0, self.field_size[2] / 2 + self.goal_post_height / 2]
        self.goal_2_post_left_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_2_position[0], self.goal_2_position[1] - self.goal_width / 2, self.goal_2_position[2]], color=[0.0, 0.0, 1.0, 1.0])
        self.goal_2_post_right_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_2_position[0], self.goal_2_position[1] + self.goal_width / 2, self.goal_2_position[2]], color=[0.0, 0.0, 1.0, 1.0])
        self.robot_position_init = [-self.field_size[0] / 4, 0.0, self.field_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, np.pi])
        self.opponent_position_init = [self.field_size[0] / 4, 0.0, self.field_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.opponent_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])
        self.opponent_id = self.create_opponent()
        self.possession_distance = 1.0
        self.max_steps = 1000

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_opponent(self):
        opponent_size = [0.5, 0.5, 1.0]
        opponent_id = self.create_box(mass=1.0, half_extents=[opponent_size[0] / 2, opponent_size[1] / 2, opponent_size[2] / 2], position=self.opponent_position_init, color=[0.0, 0.0, 0.0, 1.0])
        return opponent_id

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_object_velocity(self, object_id):
        return np.asarray(self._p.getBaseVelocity(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.ball_id, self.ball_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBaseVelocity(self.ball_id, [0.0, 0.0, 0.0], [0.0, 0.0, 0.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        self._p.resetBasePositionAndOrientation(self.opponent_id, self.opponent_position_init, self.opponent_orientation_init)
        self.steps = 0
        return observation

    def step(self, action):
        self.ball_position = self.get_object_position(self.ball_id)
        self.ball_velocity = self.get_object_velocity(self.ball_id)
        self.robot_position = self.robot.links['base'].position
        self.opponent_position = self.get_object_position(self.opponent_id)
        self.distance_to_ball = self.get_distance_to_object(self.ball_id)
        self.opponent_distance_to_ball = np.linalg.norm(self.opponent_position[:2] - self.ball_position[:2])
        observation, reward, terminated, truncated, info = super().step(action)
        self.steps += 1
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_ball_position = self.get_object_position(self.ball_id)
        new_ball_velocity = self.get_object_velocity(self.ball_id)
        new_robot_position = self.robot.links['base'].position
        new_opponent_position = self.get_object_position(self.opponent_id)
        new_distance_to_ball = self.get_distance_to_object(self.ball_id)
        new_opponent_distance_to_ball = np.linalg.norm(new_opponent_position[:2] - new_ball_position[:2])
        possession = 1.0 if new_distance_to_ball < self.possession_distance and new_opponent_distance_to_ball >= self.possession_distance else 0.0
        ball_progress = (self.ball_position[0] - new_ball_position[0]) / self.dt
        kick_velocity = 0.0
        if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.ball_id)) > 0:
            kick_velocity = np.dot(new_ball_velocity, [1.0, 0.0, 0.0])
        opponent_possession = -1.0 if new_opponent_distance_to_ball < self.possession_distance and new_distance_to_ball >= self.possession_distance else 0.0
        ball_out_of_bounds = -1.0 if np.abs(new_ball_position[0]) > self.field_size[0] / 2 or np.abs(new_ball_position[1]) > self.field_size[1] / 2 else 0.0
        robot_goal = 10.0 if self.goal_1_position[1] - self.goal_width / 2 < new_ball_position[1] < self.goal_1_position[1] + self.goal_width / 2 and new_ball_position[0] > self.goal_1_position[0] else 0.0
        opponent_goal = -10.0 if self.goal_2_position[1] - self.goal_width / 2 < new_ball_position[1] < self.goal_2_position[1] + self.goal_width / 2 and new_ball_position[0] < self.goal_2_position[0] else 0.0
        return {'possession': possession, 'ball_progress': ball_progress, 'kick_velocity': kick_velocity, 'opponent_possession': opponent_possession, 'ball_out_of_bounds': ball_out_of_bounds, 'robot_goal': robot_goal, 'opponent_goal': opponent_goal}

    def get_terminated(self, action):
        ball_position = self.get_object_position(self.ball_id)
        robot_goal = self.goal_1_position[1] - self.goal_width / 2 < ball_position[1] < self.goal_1_position[1] + self.goal_width / 2 and ball_position[0] > self.goal_1_position[0]
        opponent_goal = self.goal_2_position[1] - self.goal_width / 2 < ball_position[1] < self.goal_2_position[1] + self.goal_width / 2 and ball_position[0] < self.goal_2_position[0]
        ball_out_of_bounds = np.abs(ball_position[0]) > self.field_size[0] / 2 or np.abs(ball_position[1]) > self.field_size[1] / 2
        time_limit_reached = self.steps >= self.max_steps
        return robot_goal or opponent_goal or ball_out_of_bounds or time_limit_reached

    def get_success(self):
        ball_position = self.get_object_position(self.ball_id)
        robot_goal = self.goal_1_position[1] - self.goal_width / 2 < ball_position[1] < self.goal_1_position[1] + self.goal_width / 2 and ball_position[0] > self.goal_1_position[0]
        opponent_goal = self.goal_2_position[1] - self.goal_width / 2 < ball_position[1] < self.goal_2_position[1] + self.goal_width / 2 and ball_position[0] < self.goal_2_position[0]
        return robot_goal and (not opponent_goal)
\end{lstlisting}


==> env_codes/long_run/long_run_74.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Receive pass and kick ball past moving obstacles and goalie into goal.

    The robot is placed on a large flat ground designed to look like a soccer/football pitch with markings. 

    A teammate robot is positioned 5 meters to the side of the main robot. After a fixed delay at the start of the episode, the teammate robot passes a ball towards a point 3 meters in front of the main robot at a speed of 3 m/s. The pass target point is fixed, but the main robot's initial position has some randomness, so it will need to adjust to align itself with the passed ball.

    3 cylindrical obstacles of 0.5 meter radius and 1 meter height are placed at random positions 3 to 8 meters in front of the robot's initial position. The obstacles are colored to resemble soccer players and move randomly back and forth over a 2 meter range at speeds between 0.5 and 1.5 m/s. The obstacles do not actively chase the ball but will block it if it comes near them.

    A goal area 5 meters wide and 2 meters deep is placed 10 meters in front of the robot's initial position, centered along the front line. 

    A goalie obstacle 1 meter wide, 0.5 meters deep, and 1.5 meters tall moves side to side across the goal line at a speed of 1.5 m/s, tracking the ball when it is within 3 meters. The goalie is colored differently than the field obstacles.

    The task is for the main robot to receive the teammate's pass and then kick the moving ball past the field obstacles and goalie to score a goal, without touching any of the obstacles.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [100.0, 100.0, 0.1]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.ball_position_init = [0.0, 0.0, self.ground_size[2] / 2 + self.ball_radius]
        self.ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=self.ball_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.num_obstacles = 5
        self.obstacle_radius = 0.5
        self.obstacle_height = 1.0
        self.obstacle_ids = []
        self.obstacle_positions = []
        for _ in range(self.num_obstacles):
            position = [np.random.uniform(10.0, 50.0), np.random.uniform(-25.0, 25.0), self.ground_size[2] / 2 + self.obstacle_height / 2]
            obstacle_id = self.create_cylinder(mass=0.0, radius=self.obstacle_radius, height=self.obstacle_height, position=position, color=[0.0, 0.0, 1.0, 1.0])
            self.obstacle_ids.append(obstacle_id)
            self.obstacle_positions.append(position)
        self.goal_width = 10.0
        self.goal_depth = 2.0
        self.goal_position = [50.0, 0.0, self.ground_size[2] / 2]
        self.goal_id = self.create_box(mass=0.0, half_extents=[self.goal_depth / 2, self.goal_width / 2, 0.1], position=self.goal_position, color=[1.0, 1.0, 0.0, 0.5])
        self.goalie_width = 1.0
        self.goalie_depth = 0.5
        self.goalie_height = 1.5
        self.goalie_position_init = [self.goal_position[0] - self.goal_depth / 2 - self.goalie_depth / 2, 0.0, self.ground_size[2] / 2 + self.goalie_height / 2]
        self.goalie_id = self.create_box(mass=0.0, half_extents=[self.goalie_depth / 2, self.goalie_width / 2, self.goalie_height / 2], position=self.goalie_position_init, color=[0.0, 1.0, 1.0, 1.0])
        self.robot_position_init = [self.ball_position_init[0] - 1.0, 0.0, self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])
        self.ball_velocity_threshold = 0.1
        self.max_steps = 1000
        self.grace_period_steps = 10

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_object_velocity(self, object_id):
        return np.asarray(self._p.getBaseVelocity(object_id)[0])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.ball_id, self.ball_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBaseVelocity(self.ball_id, [0.0, 0.0, 0.0], [0.0, 0.0, 0.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        for i in range(self.num_obstacles):
            self._p.resetBasePositionAndOrientation(self.obstacle_ids[i], self.obstacle_positions[i], [0.0, 0.0, 0.0, 1.0])
        self.steps = 0
        return observation

    def step(self, action):
        self.ball_position = self.get_object_position(self.ball_id)
        self.ball_velocity = self.get_object_velocity(self.ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.steps += 1
        goalie_position = self.get_object_position(self.goalie_id)
        goalie_velocity = np.array([0.0, np.sin(self.steps * 0.1) * 1.0, 0.0])
        self._p.resetBasePositionAndOrientation(self.goalie_id, goalie_position + goalie_velocity * self.dt, [0.0, 0.0, 0.0, 1.0])
        for i in range(self.num_obstacles):
            obstacle_position = self.get_object_position(self.obstacle_ids[i])
            obstacle_velocity = np.random.uniform(low=-1.0, high=1.0, size=3)
            obstacle_velocity[2] = 0.0
            obstacle_velocity /= np.linalg.norm(obstacle_velocity)
            obstacle_velocity *= np.random.uniform(low=0.5, high=2.0)
            new_obstacle_position = obstacle_position + obstacle_velocity * self.dt
            new_obstacle_position[0] = np.clip(new_obstacle_position[0], 10.0, 50.0)
            new_obstacle_position[1] = np.clip(new_obstacle_position[1], -25.0, 25.0)
            self._p.resetBasePositionAndOrientation(self.obstacle_ids[i], new_obstacle_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_ball_position = self.get_object_position(self.ball_id)
        new_ball_velocity = self.get_object_velocity(self.ball_id)
        kick_velocity = np.linalg.norm(new_ball_velocity) if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.ball_id)) > 0 else 0.0
        goal_distance = np.linalg.norm(new_ball_position[:2] - np.array(self.goal_position)[:2])
        obstacle_collision_penalty = 0.0
        for obstacle_id in self.obstacle_ids:
            if len(self._p.getContactPoints(bodyA=self.ball_id, bodyB=obstacle_id)) > 0:
                obstacle_collision_penalty = -1.0
                break
        robot_collision_penalty = 0.0
        for obstacle_id in self.obstacle_ids:
            if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0:
                robot_collision_penalty = -1.0
                break
        goalie_collision_penalty = -1.0 if len(self._p.getContactPoints(bodyA=self.ball_id, bodyB=self.goalie_id)) > 0 else 0.0
        goal_scored = 10.0 if self.goal_position[0] - self.goal_depth / 2 < new_ball_position[0] < self.goal_position[0] + self.goal_depth / 2 and np.abs(new_ball_position[1]) < self.goal_width / 2 else 0.0
        return {'kick_velocity': kick_velocity, 'goal_distance': -goal_distance / 10.0, 'obstacle_collision_penalty': obstacle_collision_penalty, 'robot_collision_penalty': robot_collision_penalty, 'goalie_collision_penalty': goalie_collision_penalty, 'goal_scored': goal_scored}

    def get_terminated(self, action):
        ball_stopped = self.steps > self.grace_period_steps and np.linalg.norm(self.ball_velocity) < self.ball_velocity_threshold
        obstacle_collision = False
        for obstacle_id in self.obstacle_ids:
            if len(self._p.getContactPoints(bodyA=self.ball_id, bodyB=obstacle_id)) > 0 or len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0:
                obstacle_collision = True
                break
        goalie_collision = len(self._p.getContactPoints(bodyA=self.ball_id, bodyB=self.goalie_id)) > 0
        ball_out_of_bounds = np.abs(self.ball_position[0]) > 50.0 or np.abs(self.ball_position[1]) > 50.0
        time_limit_reached = self.steps >= self.max_steps
        return ball_stopped or obstacle_collision or goalie_collision or ball_out_of_bounds or time_limit_reached

    def get_success(self):
        ball_in_goal = self.goal_position[0] - self.goal_depth / 2 < self.ball_position[0] < self.goal_position[0] + self.goal_depth / 2 and np.abs(self.ball_position[1]) < self.goal_width / 2
        no_obstacle_collision = True
        for obstacle_id in self.obstacle_ids:
            if len(self._p.getContactPoints(bodyA=self.ball_id, bodyB=obstacle_id)) > 0:
                no_obstacle_collision = False
                break
        no_goalie_collision = len(self._p.getContactPoints(bodyA=self.ball_id, bodyB=self.goalie_id)) == 0
        return ball_in_goal and no_obstacle_collision and no_goalie_collision
\end{lstlisting}


==> env_codes/long_run/long_run_84.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Busy Restaurant Table Service

    Description: 
    - The environment is a busy restaurant dining area, consisting of a 12 m x 12 m room with 4 tables, an entrance door, and a kitchen door.
    - Restaurant patrons (simulated as cylinders) continuously enter from the entrance, move to a table, stay for a period of time, and then exit, making the environment dynamic.
    - The robot must perform two types of table service tasks:
      1) Table setting: The robot must collect clean dishes and utensils from the kitchen and arrange them properly on the tables in preparation for new patrons. Dishes should be stacked neatly.
      2) Table busing: After patrons leave, the robot must clear dirty dishes and utensils from the tables, load them into a bin, and return the bin to the kitchen. The bin has a maximum capacity that the robot must respect.
    - The robot must avoid colliding with patrons and restaurant furniture as it navigates.
    - Dishes will break if dropped. The robot must handle them carefully.

    Success Conditions:
    - For table setting, success means all necessary dishes and utensils are properly placed on empty tables prior to new patrons arriving. Dishes should be undamaged and neatly stacked.
    - For table busing, success involves clearing all dirty dishes from unoccupied tables, loading them into the bin without exceeding capacity, and delivering the bin to the kitchen. No dishes should be broken.
    - The robot should avoid any collisions with patrons or furniture throughout the episode.

    Time Limit:
    The episode lasts for 10 minutes of simulated time. The robot must continuously perform both table setting and busing tasks during this period as needed.

    Rewards:
    - Provide a moderate reward for each successful table set, with all dishes placed neatly and undamaged.
    - Provide a moderate reward for each successful table busing, with no broken dishes and the bin delivered to the kitchen.
    - Give a small reward for carefully handling dishes without breaking them.
    - Assign a substantial penalty for any collisions between the robot and patrons or furniture.
    - Assign a small penalty for dropping and breaking a dish.
    - Provide a small reward at each timestep for maintaining a tidy dining room, with no dirty dishes left on unoccupied tables.

    Termination:
    The episode ends if the robot crashes into a patron or furniture, or if the time limit is reached. The episode is considered successful if the robot consistently performs both table setting and busing throughout the full time period with no collisions or broken dishes.
    """

    def __init__(self):
        super().__init__()
        self.course_size = [20.0, 20.0, 10.0]
        self.course_position = [0.0, 0.0, 0.0]
        self.num_levels = 5
        self.level_height = self.course_size[2] / self.num_levels
        self.platform_size = [5.0, 5.0, 0.5]
        self.ramp_size = [5.0, 2.0, 1.0]
        self.gap_size = 2.0
        self.wall_size = [2.0, 0.2, 2.0]
        self.cylinder_radius = 0.5
        self.cylinder_height = 2.0
        self.target_object_size = [1.0, 1.0, 1.0]
        self.target_object_position_init = [0.0, 0.0, self.course_size[2] - self.level_height / 2 - self.target_object_size[2] / 2]
        self.target_object_id = self.create_box(mass=1.0, half_extents=[self.target_object_size[0] / 2, self.target_object_size[1] / 2, self.target_object_size[2] / 2], position=self.target_object_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.goal_size = [2.0, 2.0, 0.01]
        self.goal_position = [self.course_size[0] / 2 - self.goal_size[0] / 2, 0.0, self.course_size[2] / 2 - self.level_height / 2 - self.goal_size[2] / 2]
        self.goal_id = self.create_box(mass=0.0, half_extents=[self.goal_size[0] / 2, self.goal_size[1] / 2, self.goal_size[2] / 2], position=self.goal_position, color=[0.0, 1.0, 0.0, 1.0])
        self.time_limit = 300.0
        self.platform_ids = []
        self.ramp_ids = []
        self.wall_ids = []
        self.cylinder_ids = []
        self.create_course()
        self.robot_position_init = [-self.course_size[0] / 2 + 1.0, 0.0, self.course_size[2] / 2 - self.level_height / 2 + self.robot.links['base'].position_init[2]]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_course(self):
        for i in range(self.num_levels):
            level_position = [0.0, 0.0, self.course_size[2] / 2 - self.level_height * (i + 0.5)]
            platform_position = [level_position[0] + (i - self.num_levels / 2 + 0.5) * 5.0, level_position[1], level_position[2]]
            platform_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=platform_position, color=[0.5, 0.5, 0.5, 1.0])
            self.platform_ids.append(platform_id)
            if i < self.num_levels - 1:
                ramp_position = [platform_position[0] + self.platform_size[0] / 2 + self.ramp_size[0] / 2, platform_position[1], platform_position[2] + self.level_height / 2 - self.ramp_size[2] / 2]
                ramp_id = self.create_box(mass=0.0, half_extents=[self.ramp_size[0] / 2, self.ramp_size[1] / 2, self.ramp_size[2] / 2], position=ramp_position, color=[0.6, 0.4, 0.2, 1.0])
                self.ramp_ids.append(ramp_id)
            if i > 0:
                gap_position = [platform_position[0] - self.platform_size[0] / 2 - self.gap_size / 2, platform_position[1], platform_position[2]]
                wall_position_left = [gap_position[0] - self.gap_size / 2 - self.wall_size[0] / 2, gap_position[1] - self.platform_size[1] / 2 - self.wall_size[1] / 2, gap_position[2] + self.wall_size[2] / 2]
                wall_position_right = [gap_position[0] - self.gap_size / 2 - self.wall_size[0] / 2, gap_position[1] + self.platform_size[1] / 2 + self.wall_size[1] / 2, gap_position[2] + self.wall_size[2] / 2]
                wall_id_left = self.create_box(mass=0.0, half_extents=[self.wall_size[0] / 2, self.wall_size[1] / 2, self.wall_size[2] / 2], position=wall_position_left, color=[0.2, 0.2, 0.2, 1.0])
                wall_id_right = self.create_box(mass=0.0, half_extents=[self.wall_size[0] / 2, self.wall_size[1] / 2, self.wall_size[2] / 2], position=wall_position_right, color=[0.2, 0.2, 0.2, 1.0])
                self.wall_ids.append(wall_id_left)
                self.wall_ids.append(wall_id_right)
            if i < self.num_levels - 1:
                cylinder_position = [platform_position[0], platform_position[1] - self.platform_size[1] / 4, platform_position[2] + self.level_height / 2 - self.cylinder_height / 2]
                cylinder_id = self.create_cylinder(mass=0.0, radius=self.cylinder_radius, height=self.cylinder_height, position=cylinder_position, color=[0.8, 0.8, 0.8, 1.0])
                self.cylinder_ids.append(cylinder_id)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.target_object_id, self.target_object_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.robot_position = self.robot.links['base'].position
        self.target_object_position = self.get_object_position(self.target_object_id)
        self.distance_to_target_object = self.get_distance_to_object(self.target_object_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_robot_position = self.robot.links['base'].position
        new_target_object_position = self.get_object_position(self.target_object_id)
        new_distance_to_target_object = self.get_distance_to_object(self.target_object_id)
        forward_progression = (new_robot_position[0] - self.robot_position[0]) / self.dt
        elevation_scale = new_robot_position[2] / self.course_size[2]
        forward_progression_reward = 0.1 * forward_progression * elevation_scale
        reached_target_object_reward = 0.0
        if new_distance_to_target_object < 1.0 and self.distance_to_target_object >= 1.0:
            reached_target_object_reward = 10.0
        target_object_in_goal_reward = 0.0
        if self.goal_position[0] - self.goal_size[0] / 2 < new_target_object_position[0] < self.goal_position[0] + self.goal_size[0] / 2 and self.goal_position[1] - self.goal_size[1] / 2 < new_target_object_position[1] < self.goal_position[1] + self.goal_size[1] / 2:
            target_object_in_goal_reward = 100.0
        collision_penalty = 0.0
        for object_id in self.wall_ids + self.cylinder_ids:
            if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=object_id)) > 0:
                collision_penalty -= 1.0
        return {'forward_progression_reward': forward_progression_reward, 'reached_target_object_reward': reached_target_object_reward, 'target_object_in_goal_reward': target_object_in_goal_reward, 'collision_penalty': collision_penalty}

    def get_terminated(self, action):
        robot_position = self.robot.links['base'].position
        if robot_position[2] < self.course_size[2] / 2 - self.level_height:
            return True
        if np.dot(np.asarray([0, 0, 1]), np.asarray(self._p.getMatrixFromQuaternion(self.robot.links['base'].orientation)).reshape(3, 3)[:, 2]) < 0.5:
            return True
        if self.time >= self.time_limit:
            return True
        return False

    def get_success(self):
        target_object_position = self.get_object_position(self.target_object_id)
        robot_position = self.robot.links['base'].position
        target_object_velocity = np.linalg.norm(self._p.getBaseVelocity(self.target_object_id)[0])
        is_target_object_in_goal = self.goal_position[0] - self.goal_size[0] / 2 < target_object_position[0] < self.goal_position[0] + self.goal_size[0] / 2 and self.goal_position[1] - self.goal_size[1] / 2 < target_object_position[1] < self.goal_position[1] + self.goal_size[1] / 2
        is_robot_in_goal = self.goal_position[0] - self.goal_size[0] / 2 < robot_position[0] < self.goal_position[0] + self.goal_size[0] / 2 and self.goal_position[1] - self.goal_size[1] / 2 < robot_position[1] < self.goal_position[1] + self.goal_size[1] / 2
        return is_target_object_in_goal and is_robot_in_goal and (target_object_velocity < 0.1)
\end{lstlisting}


==> env_codes/long_run/long_run_88.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Bounce Shot Scoring Challenge

    Description:
    - The environment consists of a walled field measuring 20 m x 10 m. The field contains 3 ramps/mounds (triangular prisms) placed randomly, each measuring 2 m long x 1 m wide x 0.5 m high.  
    - A single goal 3 m wide and 1 m high is placed centered on one end of the field.
    - A ball (0.5 m diameter) is released from a random point along the opposite side of the field from the goal. The ball is given an initial velocity of 3-5 m/s at a random angle towards the goal end of the field.
    - Due to the ramps on the field, the ball will bounce and roll unpredictably as it crosses the field.
    - The robot begins in the center of the field on the goal side.

    Task:
    The robot must intercept the bouncing ball and kick it into the goal to score a point. The robot should dynamically adjust its approach to the ball based on the ball's changing trajectory after each bounce off a ramp. The robot needs to time its kick to hit the ball at the optimal point in its bounce to redirect it into the goal.

    Success Conditions:
    The task is completed successfully if the robot causes the ball to fully enter the goal area.

    Rewards:
    - Small reward for decreasing distance to the ball, scaled higher as the ball gets closer to the robot's side of the field
    - Moderate penalty if the ball's velocity drops to zero or it leaves the field without scoring
    - Large reward for kicking the ball, scaled by the ball's post-kick velocity in the direction of the goal
    - Large reward for scoring a goal

    Termination:
    The episode ends if the ball comes to rest, leaves the field, or enters the goal area.
    """

    def __init__(self):
        super().__init__()
        self.field_size = [20.0, 10.0, 0.1]
        self.field_position = [0.0, 0.0, 0.0]
        self.field_id = self.create_box(mass=0.0, half_extents=[self.field_size[0] / 2, self.field_size[1] / 2, self.field_size[2] / 2], position=self.field_position, color=[0.1, 0.8, 0.1, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.field_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.wall_height = 1.0
        self.wall_thickness = 0.1
        self.create_walls()
        self.ramp_size = [2.0, 1.0, 0.5]
        self.num_ramps = 3
        self.ramp_ids = []
        self.goal_width = 3.0
        self.goal_height = 1.0
        self.goal_thickness = 0.1
        self.goal_position = [self.field_position[0] + self.field_size[0] / 2 - self.goal_thickness / 2, self.field_position[1], self.field_position[2] + self.goal_height / 2]
        self.goal_id = self.create_box(mass=0.0, half_extents=[self.goal_thickness / 2, self.goal_width / 2, self.goal_height / 2], position=self.goal_position, color=[1.0, 0.0, 0.0, 0.5])
        self.create_ramps()
        self.ball_radius = 0.25
        self.ball_position_init = [0.0, 0.0, self.field_position[2] + self.ball_radius]
        self.ball_velocity_init = [0.0, 0.0, 0.0]
        self.ball_id = self.create_sphere(mass=0.1, radius=self.ball_radius, position=self.ball_position_init, color=[1.0, 0.5, 0.0, 1.0])
        self.robot_position_init = [self.field_position[0] + self.field_size[0] / 4, self.field_position[1], self.field_position[2] + self.robot.links['base'].position_init[2]]
        self.ball_velocity_range = [3.0, 5.0]
        self.ball_angle_range = [-np.pi / 4, np.pi / 4]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_walls(self):
        wall_positions = [[self.field_position[0], self.field_position[1] - self.field_size[1] / 2 - self.wall_thickness / 2, self.field_position[2] + self.wall_height / 2], [self.field_position[0], self.field_position[1] + self.field_size[1] / 2 + self.wall_thickness / 2, self.field_position[2] + self.wall_height / 2], [self.field_position[0] - self.field_size[0] / 2 - self.wall_thickness / 2, self.field_position[1], self.field_position[2] + self.wall_height / 2]]
        wall_half_extents = [[self.field_size[0] / 2, self.wall_thickness / 2, self.wall_height / 2], [self.field_size[0] / 2, self.wall_thickness / 2, self.wall_height / 2], [self.wall_thickness / 2, self.field_size[1] / 2, self.wall_height / 2]]
        for position, half_extents in zip(wall_positions, wall_half_extents):
            self.create_box(mass=0.0, half_extents=half_extents, position=position, color=[0.2, 0.2, 0.2, 1.0])

    def create_ramps(self):
        for _ in range(self.num_ramps):
            while True:
                position = [np.random.uniform(self.field_position[0] - self.field_size[0] / 2 + self.ramp_size[0] / 2, self.field_position[0] + self.field_size[0] / 2 - self.ramp_size[0] / 2 - self.goal_thickness), np.random.uniform(self.field_position[1] - self.field_size[1] / 2 + self.ramp_size[1] / 2, self.field_position[1] + self.field_size[1] / 2 - self.ramp_size[1] / 2), self.field_position[2] + self.ramp_size[2] / 2]
                if all((np.linalg.norm(np.asarray(position[:2]) - np.asarray(ramp_position[:2])) > self.ramp_size[0] + self.ramp_size[1] for ramp_position in [self.get_object_position(ramp_id) for ramp_id in self.ramp_ids])):
                    break
            ramp_id = self.create_box(mass=0.0, half_extents=[self.ramp_size[0] / 2, self.ramp_size[1] / 2, self.ramp_size[2] / 2], position=position, color=[0.4, 0.4, 0.4, 1.0])
            self.ramp_ids.append(ramp_id)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_object_velocity(self, object_id):
        return np.asarray(self._p.getBaseVelocity(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        ball_x = -self.field_size[0] / 2 + self.ball_radius
        ball_y = np.random.uniform(-self.field_size[1] / 2 + self.ball_radius, self.field_size[1] / 2 - self.ball_radius)
        ball_position_init = [ball_x, ball_y, self.field_position[2] + self.ball_radius]
        self._p.resetBasePositionAndOrientation(self.ball_id, ball_position_init, [0.0, 0.0, 0.0, 1.0])
        ball_speed = np.random.uniform(self.ball_velocity_range[0], self.ball_velocity_range[1])
        ball_angle = np.random.uniform(self.ball_angle_range[0], self.ball_angle_range[1])
        ball_velocity_init = [ball_speed * np.cos(ball_angle), ball_speed * np.sin(ball_angle), 0.0]
        self._p.resetBaseVelocity(self.ball_id, ball_velocity_init, [0.0, 0.0, 0.0])
        return observation

    def step(self, action):
        self.distance_to_ball = self.get_distance_to_object(self.ball_id)
        self.ball_position = self.get_object_position(self.ball_id)
        self.ball_velocity = self.get_object_velocity(self.ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_ball = self.get_distance_to_object(self.ball_id)
        new_ball_position = self.get_object_position(self.ball_id)
        new_ball_velocity = self.get_object_velocity(self.ball_id)
        reach_ball = (self.distance_to_ball - new_distance_to_ball) / self.dt * (1.0 - new_ball_position[0] / (self.field_size[0] / 2))
        ball_stopped = 0.0
        if np.linalg.norm(new_ball_velocity) < 0.1:
            ball_stopped = -5.0
        kick_ball = 0.0
        if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.ball_id)) > 0:
            ball_to_goal = np.asarray(self.goal_position)[:2] - new_ball_position[:2]
            ball_to_goal_norm = np.linalg.norm(ball_to_goal)
            if ball_to_goal_norm > 0.1:
                kick_ball = np.dot(new_ball_velocity[:2], ball_to_goal) / ball_to_goal_norm
        ball_in_goal = 0.0
        if self.goal_position[1] - self.goal_width / 2 < new_ball_position[1] < self.goal_position[1] + self.goal_width / 2 and new_ball_position[0] > self.goal_position[0]:
            ball_in_goal = 100.0
        return {'reach_ball': reach_ball, 'ball_stopped': ball_stopped, 'kick_ball': kick_ball, 'ball_in_goal': ball_in_goal}

    def get_terminated(self, action):
        ball_position = self.get_object_position(self.ball_id)
        return np.linalg.norm(self.ball_velocity) < 0.1 or abs(ball_position[0]) > self.field_size[0] / 2 or abs(ball_position[1]) > self.field_size[1] / 2

    def get_success(self):
        ball_position = self.get_object_position(self.ball_id)
        return self.goal_position[1] - self.goal_width / 2 < ball_position[1] < self.goal_position[1] + self.goal_width / 2 and ball_position[0] > self.goal_position[0]
\end{lstlisting}


==> env_codes/long_run/long_run_90.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Outdoor Retrieval Challenge

    Description:
    - The environment is a large outdoor field 50 m x 50 m, with the robot starting in the center. 
    - The terrain includes various features:
      - A steep hill with a 30 degree incline
      - A shallow stream, 0.5 m deep and 5 m wide
      - Patches of loose sand and gravel
      - Scattered trees and boulders up to 2 m tall
    - A 0.5 m diameter soccer ball is placed randomly between 10 m and 20 m from the robot's starting position.
    - The robot must locate the ball, pick it up or get it balanced on its back, and return it to the starting location.
    - The ball is heavy enough that it can't simply be pushed the whole way. The robot needs to lift/carry it.
    - If the robot drops the ball or it rolls more than 5 m away, it is replaced at a new random location.

    Success Conditions:
    The task is completed when the robot returns to within 2 m of its starting position with the ball balanced on its back or in its possession.

    Time Limit:
    The robot has 10 minutes to complete the retrieval.

    Rewards:
    - Provide a small reward for exploring the environment and locating the ball
    - Provide a moderate reward for successfully getting the ball balanced on the robot's back or lifted off the ground 
    - Provide a large reward for returning to the start area with the ball
    - Provide a small penalty if the ball is dropped or lost, to encourage careful handling

    Termination:
    The episode ends if the robot flips over and can't right itself, or if the time limit is exceeded.
    """

    def __init__(self):
        super().__init__()
        self.field_size = [50.0, 50.0, 0.0]
        self.robot_start_position = [0.0, 0.0, 0.0]
        self.ground_thickness = 0.2
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.field_size[0] / 2, self.field_size[1] / 2, self.ground_thickness / 2], position=[0.0, 0.0, -self.ground_thickness / 2], orientation=[0.0, 0.0, 0.0, 1.0], color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.2)
        self.ball_radius = 0.25
        self.ball_mass = 1.0
        self.ball_start_distance_range = [10.0, 20.0]
        self.ball_start_position = self.get_random_ball_start_position()
        self.ball_id = self.create_sphere(mass=self.ball_mass, radius=self.ball_radius, position=self.ball_start_position, color=[1.0, 1.0, 1.0, 1.0])
        self.ball_lost_distance = 5.0
        self.success_distance = 2.0
        self.time_limit = 600.0
        self.terrain_ids = []
        self.create_terrain()

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_box(self, mass, half_extents, position, orientation, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position, baseOrientation=orientation)

    def create_cylinder(self, mass, radius, height, position, orientation, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position, baseOrientation=orientation)

    def create_terrain(self):
        hill_height = 5.0
        hill_half_extents = [10.0, 10.0, hill_height / 2]
        hill_position = [15.0, 15.0, hill_height / 2]
        hill_orientation = self._p.getQuaternionFromEuler([0.0, 0.0, np.random.uniform(0.0, 2 * np.pi)])
        hill_id = self.create_box(mass=0.0, half_extents=hill_half_extents, position=hill_position, orientation=hill_orientation, color=[0.5, 0.5, 0.5, 1.0])
        self.terrain_ids.append(hill_id)
        stream_depth = 0.5
        stream_half_extents = [2.5, 25.0, stream_depth / 2]
        stream_position = [-15.0, 0.0, stream_depth / 2]
        stream_orientation = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])
        stream_id = self.create_box(mass=0.0, half_extents=stream_half_extents, position=stream_position, orientation=stream_orientation, color=[0.0, 0.0, 1.0, 0.5])
        self.terrain_ids.append(stream_id)
        num_patches = 10
        patch_radius = 3.0
        for _ in range(num_patches):
            patch_position = [np.random.uniform(-25.0, 25.0), np.random.uniform(-25.0, 25.0), 0.05]
            patch_orientation = self._p.getQuaternionFromEuler([0.0, 0.0, np.random.uniform(0.0, 2 * np.pi)])
            patch_id = self.create_cylinder(mass=0.0, radius=patch_radius, height=0.1, position=patch_position, orientation=patch_orientation, color=[0.8, 0.8, 0.4, 1.0])
            self.terrain_ids.append(patch_id)
        num_obstacles = 20
        obstacle_radius_range = [0.5, 1.0]
        obstacle_height_range = [1.0, 2.0]
        for _ in range(num_obstacles):
            obstacle_radius = np.random.uniform(obstacle_radius_range[0], obstacle_radius_range[1])
            obstacle_height = np.random.uniform(obstacle_height_range[0], obstacle_height_range[1])
            obstacle_position = [np.random.uniform(-25.0, 25.0), np.random.uniform(-25.0, 25.0), obstacle_height / 2]
            obstacle_orientation = self._p.getQuaternionFromEuler([0.0, 0.0, np.random.uniform(0.0, 2 * np.pi)])
            if np.random.rand() < 0.5:
                obstacle_id = self.create_cylinder(mass=0.0, radius=obstacle_radius, height=obstacle_height, position=obstacle_position, orientation=obstacle_orientation, color=[0.4, 0.2, 0.0, 1.0])
            else:
                obstacle_id = self.create_box(mass=0.0, half_extents=[obstacle_radius, obstacle_radius, obstacle_height / 2], position=obstacle_position, orientation=obstacle_orientation, color=[0.5, 0.5, 0.5, 1.0])
            self.terrain_ids.append(obstacle_id)

    def get_random_ball_start_position(self):
        angle = np.random.uniform(0.0, 2 * np.pi)
        distance = np.random.uniform(self.ball_start_distance_range[0], self.ball_start_distance_range[1])
        x = self.robot_start_position[0] + distance * np.cos(angle)
        y = self.robot_start_position[1] + distance * np.sin(angle)
        z = self.ball_radius
        return [x, y, z]

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self.ball_start_position = self.get_random_ball_start_position()
        self._p.resetBasePositionAndOrientation(self.ball_id, self.ball_start_position, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.robot_start_position[0], self.robot_start_position[1], self.ground_thickness / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.ball_position = self.get_object_position(self.ball_id)
        self.robot_position = self.robot.links['base'].position
        self.distance_to_ball = self.get_distance_to_object(self.ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        if self.distance_to_ball > self.ball_lost_distance:
            self.ball_start_position = self.get_random_ball_start_position()
            self._p.resetBasePositionAndOrientation(self.ball_id, self.ball_start_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_ball_position = self.get_object_position(self.ball_id)
        new_robot_position = self.robot.links['base'].position
        new_distance_to_ball = self.get_distance_to_object(self.ball_id)
        explore_reward = 0.1 * (self.distance_to_ball - new_distance_to_ball) / self.dt
        pickup_reward = 0.0
        if self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.ball_id) and new_ball_position[2] > self.ball_radius:
            pickup_reward = 10.0
        return_reward = 0.0
        if new_distance_to_ball < self.success_distance and np.linalg.norm(new_robot_position[:2] - self.robot_start_position[:2]) < self.success_distance:
            return_reward = 100.0
        drop_penalty = -1.0 if new_distance_to_ball > self.ball_lost_distance else 0.0
        return {'explore_reward': explore_reward, 'pickup_reward': pickup_reward, 'return_reward': return_reward, 'drop_penalty': drop_penalty}

    def get_terminated(self, action):
        if np.dot(np.asarray([0, 0, 1]), np.asarray(self._p.getMatrixFromQuaternion(self.robot.links['base'].orientation)).reshape(3, 3)[:, 2]) < 0.5:
            return True
        if self.time >= self.time_limit:
            return True
        return False

    def get_success(self):
        ball_position = self.get_object_position(self.ball_id)
        robot_position = self.robot.links['base'].position
        distance_to_ball = self.get_distance_to_object(self.ball_id)
        return distance_to_ball < self.success_distance and np.linalg.norm(robot_position[:2] - self.robot_start_position[:2]) < self.success_distance and (ball_position[2] > self.ball_radius)
\end{lstlisting}


==> env_codes/short_run/short_run_1.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Cross a bridge with moving segments to reach a platform.

    Description: 
    - A start platform and an end platform (each 3 m in size and 0.5 m in thickness) are placed 20 m apart.
    - The two platforms are connected by a bridge (2 m wide) divided into 5 segments of equal length (3 m each). 
    - Each segment moves up and down independently with a sinusoidal motion. The amplitude is 1 m and the period is 2 seconds, with each segment offset in phase by 0.4 seconds from the previous one.
    - The segments are colored red, orange, yellow, green, and blue.
    The robot is initialized on the start platform. 
    The task of the robot is to cross the dynamic bridge to reach the end platform as fast as possible by timing its jumps between the moving segments.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    To help the robot complete the task:
    - The robot receives a reward for each time step it remains on the bridge or platforms, encouraging steady progress. 
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.

    Termination:
    The task terminates immediately if the robot falls off the start platform, any segment of the bridge, or the end platform.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 20.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.bridge_length = self.platform_end_position[0] - self.platform_start_position[0] - self.platform_size[0]
        self.bridge_width = 2.0
        self.num_segments = 5
        self.segment_length = self.bridge_length / self.num_segments
        self.segment_amplitude = 1.0
        self.segment_period = 2.0
        self.segment_phase_offset = 0.4
        segment_colors = [[1.0, 0.0, 0.0, 1.0], [1.0, 0.5, 0.0, 1.0], [1.0, 1.0, 0.0, 1.0], [0.0, 1.0, 0.0, 1.0], [0.0, 0.0, 1.0, 1.0]]
        self.segment_ids = []
        for i in range(self.num_segments):
            segment_id = self.create_box(mass=0.0, half_extents=[self.segment_length / 2, self.bridge_width / 2, self.platform_size[2] / 2], position=[self.platform_start_position[0] + self.platform_size[0] / 2 + self.segment_length / 2 + i * self.segment_length, self.platform_start_position[1], self.platform_start_position[2]], color=segment_colors[i])
            self._p.changeDynamics(bodyUniqueId=segment_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
            self.segment_ids.append(segment_id)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        for i, segment_id in enumerate(self.segment_ids):
            segment_position = self.get_object_position(segment_id)
            new_segment_position = [segment_position[0], segment_position[1], self.platform_start_position[2] + self.segment_amplitude * np.sin(2 * np.pi * (self.time + i * self.segment_phase_offset) / self.segment_period)]
            self._p.resetBasePositionAndOrientation(segment_id, new_segment_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        on_bridge_or_platforms = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] + self.platform_size[2] / 2 else -1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        return {'on_bridge_or_platforms': on_bridge_or_platforms, 'reach_platform_end': reach_platform_end}

    def get_terminated(self, action):
        return self.robot.links['base'].position[2] < self.platform_start_position[2]

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_size[2] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_10.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Dodgeball Game

    Description:
    - The robot spawns in a square arena measuring 10 meters by 10 meters.
    - Balls with a radius of 0.25 meters spawn randomly within the arena at a height of 1 meter and are launched toward the robot with an initial velocity of 5 meters per second.
    - The balls spawn at a rate of one ball every 2 seconds.
    - The robot's task is to dodge the balls for as long as possible.

    Success:
    The task is successfully completed if the robot survives for a predefined duration of 60 seconds without being hit by any balls.

    Rewards:
    - The robot receives a reward for each time step it remains standing and avoids being hit by a ball, encouraging it to dodge effectively.
    - A small survival reward is given for each second the robot remains in the game, incentivizing prolonged survival.
    - A penalty is applied if the robot is hit by a ball, encouraging it to avoid collisions.

    Termination:
    - The task terminates immediately if the robot is hit by a ball.
    - The task also terminates if the robot survives for 60 seconds without being hit by any balls.
    """

    def __init__(self):
        super().__init__()
        self.arena_size = [10.0, 10.0]
        self.arena_position = [0.0, 0.0, 0.0]
        self.arena_id = self.create_box(mass=0.0, half_extents=[self.arena_size[0] / 2, self.arena_size[1] / 2, 0.1], position=self.arena_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.arena_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.25
        self.ball_velocity = 5.0
        self.ball_spawn_interval = 2.0
        self.ball_ids = []
        self.robot_position_init = [0.0, 0.0, self.arena_position[2] + 0.1 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])
        self.survival_duration = 16.0

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, velocity, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        ball_id = self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)
        self._p.resetBaseVelocity(objectUniqueId=ball_id, linearVelocity=velocity)
        return ball_id

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        for ball_id in self.ball_ids:
            self._p.removeBody(ball_id)
        self.ball_ids = []
        return observation

    def step(self, action):
        self.hit_by_ball = False
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        if self.time % self.ball_spawn_interval < self.dt:
            ball_position = [np.random.uniform(low=-self.arena_size[0] / 2 + self.ball_radius, high=self.arena_size[0] / 2 - self.ball_radius), np.random.uniform(low=-self.arena_size[1] / 2 + self.ball_radius, high=self.arena_size[1] / 2 - self.ball_radius), 1.0]
            ball_velocity = [np.random.uniform(low=-1.0, high=1.0), np.random.uniform(low=-1.0, high=1.0), 0.0]
            ball_velocity = self.ball_velocity * np.array(ball_velocity) / np.linalg.norm(ball_velocity)
            ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=ball_position, velocity=ball_velocity, color=[1.0, 0.0, 0.0, 1.0])
            self.ball_ids.append(ball_id)
        for ball_id in self.ball_ids:
            contact_points = self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=ball_id)
            if len(contact_points) > 0:
                self.hit_by_ball = True
                break
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        survival = 1.0
        hit_penalty = -10.0 if self.hit_by_ball else 0.0
        return {'survival': survival, 'hit_penalty': hit_penalty}

    def get_terminated(self, action):
        if self.hit_by_ball:
            return True
        if self.time >= self.survival_duration:
            return True
        return False

    def get_success(self):
        return self.time >= self.survival_duration and (not self.hit_by_ball)
\end{lstlisting}


==> env_codes/short_run/short_run_11.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Jump from moving platform to moving platform to cross water and reach a target zone on a platform.

    Description:
    - The environment consists of a start platform (3 m x 3 m x 0.5 m) and an end platform (3 m x 3 m x 0.5 m) placed 20 meters apart.
    - The two platforms are connected by a series of 5 moving platforms (2 m x 2 m x 0.5 m) placed 3 meters apart.
    - Each moving platform follows a sinusoidal motion along the y-axis with an amplitude of 1 meter and a period of 3 seconds. The motion of each platform is offset by 0.6 seconds from the previous one.
    - The platforms are placed above a water surface, and the robot must jump from one moving platform to the next to reach the end platform.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    - The robot receives a reward for each time step it remains on the platforms, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.
    - The robot is penalized for falling into the water.

    Termination:
    The task terminates immediately if the robot falls into the water or reaches the end platform.
    """

    def __init__(self):
        super().__init__()
        self.water_size = [1000.0, 1000.0, 10.0]
        self.water_position = [0.0, 0.0, 0.0]
        self.water_id = self.create_box(mass=0.0, half_extents=[self.water_size[0] / 2, self.water_size[1] / 2, self.water_size[2] / 2], position=self.water_position, color=[0.0, 0.0, 1.0, 0.5])
        self.platform_start_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, self.water_position[2] + self.water_size[2] / 2 + self.platform_start_size[2] / 2]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_start_size[0] / 2, self.platform_start_size[1] / 2, self.platform_start_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_size = [3.0, 3.0, 0.5]
        self.platform_end_position = [self.platform_start_position[0] + 20.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_end_size[0] / 2, self.platform_end_size[1] / 2, self.platform_end_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.num_moving_platforms = 5
        self.moving_platform_size = [2.0, 2.0, 0.5]
        self.moving_platform_amplitude = 1.0
        self.moving_platform_period = 3.0
        self.moving_platform_phase_offset = 0.6
        self.moving_platform_ids = []
        for i in range(self.num_moving_platforms):
            moving_platform_position = [self.platform_start_position[0] + (i + 1) * 3.0, self.platform_start_position[1], self.platform_start_position[2]]
            moving_platform_id = self.create_box(mass=0.0, half_extents=[self.moving_platform_size[0] / 2, self.moving_platform_size[1] / 2, self.moving_platform_size[2] / 2], position=moving_platform_position, color=[0.8, 0.8, 0.8, 1.0])
            self.moving_platform_ids.append(moving_platform_id)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_start_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        for i, moving_platform_id in enumerate(self.moving_platform_ids):
            moving_platform_position = self.get_object_position(moving_platform_id)
            new_moving_platform_position = [moving_platform_position[0], self.platform_start_position[1] + self.moving_platform_amplitude * np.sin(2 * np.pi * (self.time + i * self.moving_platform_phase_offset) / self.moving_platform_period), moving_platform_position[2]]
            self._p.resetBasePositionAndOrientation(moving_platform_id, new_moving_platform_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        on_platform = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] else -1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        return {'on_platform': on_platform, 'reach_platform_end': reach_platform_end}

    def get_terminated(self, action):
        is_in_water = self.robot.links['base'].position[2] < self.water_position[2] + self.water_size[2] / 2
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_end_size[0] / 2
        return is_in_water or is_on_platform_end

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_end_size[0] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_12.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Navigate a terrain with obstacles to reach a target zone.

    Description:
    - The environment consists of a start platform (3 m x 3 m x 0.5 m) and an end platform (3 m x 3 m x 0.5 m) placed 30 meters apart.
    - The terrain between the platforms is filled with static obstacles such as rocks (cylinders) and trees (cylinders with a height of 3 meters).
    - The obstacles are randomly placed with a minimum distance of 1 meter between them, ensuring the robot cannot go around them easily.
    - The robot is initialized on the start platform, facing the end platform.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    - The robot receives a reward for each time step it remains on the platforms or the terrain, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.
    - The robot is penalized for collisions with obstacles.

    Termination:
    The task terminates immediately if the robot falls off the start platform, the terrain, or the end platform, or if the robot collides with an obstacle.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 30.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.platform_start_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self._p.changeDynamics(bodyUniqueId=self.platform_end_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.terrain_size = [self.platform_end_position[0] - self.platform_start_position[0], 10.0, 0.1]
        self.terrain_position = [self.platform_start_position[0] + self.terrain_size[0] / 2, self.platform_start_position[1], self.platform_start_position[2] - self.platform_size[2] / 2 - self.terrain_size[2] / 2]
        self.terrain_id = self.create_box(mass=0.0, half_extents=[self.terrain_size[0] / 2, self.terrain_size[1] / 2, self.terrain_size[2] / 2], position=self.terrain_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.terrain_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.wall_size = [self.terrain_size[0], 0.1, 1.0]
        self.wall_left_position = [self.terrain_position[0], self.terrain_position[1] - self.terrain_size[1] / 2 - self.wall_size[1] / 2, self.terrain_position[2] + self.terrain_size[2] / 2 + self.wall_size[2] / 2]
        self.wall_right_position = [self.terrain_position[0], self.terrain_position[1] + self.terrain_size[1] / 2 + self.wall_size[1] / 2, self.terrain_position[2] + self.terrain_size[2] / 2 + self.wall_size[2] / 2]
        self.wall_left_id = self.create_box(mass=0.0, half_extents=[self.wall_size[0] / 2, self.wall_size[1] / 2, self.wall_size[2] / 2], position=self.wall_left_position, color=[0.5, 0.5, 0.5, 1.0])
        self.wall_right_id = self.create_box(mass=0.0, half_extents=[self.wall_size[0] / 2, self.wall_size[1] / 2, self.wall_size[2] / 2], position=self.wall_right_position, color=[0.5, 0.5, 0.5, 1.0])
        self.num_obstacles = 10
        self.obstacle_radius = 0.5
        self.obstacle_height = 1.0
        self.tree_height = 3.0
        self.obstacle_ids = []
        for _ in range(self.num_obstacles):
            while True:
                obstacle_position = [np.random.uniform(self.platform_start_position[0] + self.platform_size[0] / 2 + self.obstacle_radius, self.platform_end_position[0] - self.platform_size[0] / 2 - self.obstacle_radius), np.random.uniform(self.terrain_position[1] - self.terrain_size[1] / 2 + self.obstacle_radius, self.terrain_position[1] + self.terrain_size[1] / 2 - self.obstacle_radius), self.terrain_position[2] + self.terrain_size[2] / 2 + self.obstacle_height / 2]
                if all((np.linalg.norm(np.array(obstacle_position[:2]) - np.array(other_obstacle_position[:2])) > 2 * self.obstacle_radius + 1.0 for other_obstacle_position in [self.get_object_position(obstacle_id)[:2] for obstacle_id in self.obstacle_ids])):
                    break
            if np.random.rand() < 0.5:
                obstacle_id = self.create_cylinder(mass=0.0, radius=self.obstacle_radius, height=self.obstacle_height, position=obstacle_position, orientation=[0.0, 0.0, 0.0, 1.0], color=[0.5, 0.0, 0.0, 1.0])
            else:
                obstacle_id = self.create_cylinder(mass=0.0, radius=self.obstacle_radius, height=self.tree_height, position=obstacle_position, orientation=[0.0, 0.0, 0.0, 1.0], color=[0.0, 0.5, 0.0, 1.0])
            self.obstacle_ids.append(obstacle_id)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, orientation, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position, baseOrientation=orientation)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        survival = 1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        collision = -1.0 if any((len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0 for obstacle_id in self.obstacle_ids)) else 0.0
        return {'survival': survival, 'reach_platform_end': reach_platform_end, 'collision': collision}

    def get_terminated(self, action):
        is_fall_off = self.robot.links['base'].position[2] < self.terrain_position[2]
        is_collision = any((len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0 for obstacle_id in self.obstacle_ids))
        return is_fall_off or is_collision

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_size[0] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_13.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Navigate a terrain with obstacles to reach a target zone.

    Description:
    - The environment consists of a start platform (3 m x 3 m x 0.5 m) and an end platform (3 m x 3 m x 0.5 m) placed 30 meters apart.
    - The terrain between the platforms is filled with static obstacles such as rocks (cylinders) and trees (cylinders with a height of 3 meters).
    - The obstacles are placed in a grid pattern with enough space between them to ensure a feasible path.
    - The robot is initialized on the start platform, facing the end platform.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    - The robot receives a reward for each time step it remains on the platforms or the terrain, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.
    - The robot is penalized for collisions with obstacles.

    Termination:
    The task terminates if the robot falls off the start platform, the terrain, or the end platform.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 30.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.platform_start_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self._p.changeDynamics(bodyUniqueId=self.platform_end_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.terrain_size = [self.platform_end_position[0] - self.platform_start_position[0], 10.0, 0.1]
        self.terrain_position = [self.platform_start_position[0] + self.terrain_size[0] / 2, self.platform_start_position[1], self.platform_start_position[2] - self.platform_size[2] / 2 - self.terrain_size[2] / 2]
        self.terrain_id = self.create_box(mass=0.0, half_extents=[self.terrain_size[0] / 2, self.terrain_size[1] / 2, self.terrain_size[2] / 2], position=self.terrain_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.terrain_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.wall_size = [self.terrain_size[0], 0.1, 1.0]
        self.wall_left_position = [self.terrain_position[0], self.terrain_position[1] - self.terrain_size[1] / 2 - self.wall_size[1] / 2, self.terrain_position[2] + self.terrain_size[2] / 2 + self.wall_size[2] / 2]
        self.wall_right_position = [self.terrain_position[0], self.terrain_position[1] + self.terrain_size[1] / 2 + self.wall_size[1] / 2, self.terrain_position[2] + self.terrain_size[2] / 2 + self.wall_size[2] / 2]
        self.wall_left_id = self.create_box(mass=0.0, half_extents=[self.wall_size[0] / 2, self.wall_size[1] / 2, self.wall_size[2] / 2], position=self.wall_left_position, color=[0.5, 0.5, 0.5, 1.0])
        self.wall_right_id = self.create_box(mass=0.0, half_extents=[self.wall_size[0] / 2, self.wall_size[1] / 2, self.wall_size[2] / 2], position=self.wall_right_position, color=[0.5, 0.5, 0.5, 1.0])
        self.num_obstacles = 10
        self.obstacle_radius = 0.5
        self.obstacle_height = 1.0
        self.tree_height = 3.0
        self.obstacle_ids = []
        self.place_obstacles()

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, orientation, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position, baseOrientation=orientation)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def place_obstacles(self):
        grid_size = int(np.sqrt(self.num_obstacles))
        x_positions = np.linspace(self.platform_start_position[0] + self.platform_size[0] / 2 + self.obstacle_radius, self.platform_end_position[0] - self.platform_size[0] / 2 - self.obstacle_radius, grid_size)
        y_positions = np.linspace(self.terrain_position[1] - self.terrain_size[1] / 2 + self.obstacle_radius, self.terrain_position[1] + self.terrain_size[1] / 2 - self.obstacle_radius, grid_size)
        for x in x_positions:
            for y in y_positions:
                if np.random.rand() < 0.5:
                    obstacle_id = self.create_cylinder(mass=0.0, radius=self.obstacle_radius, height=self.obstacle_height, position=[x, y, self.terrain_position[2] + self.terrain_size[2] / 2 + self.obstacle_height / 2], orientation=[0.0, 0.0, 0.0, 1.0], color=[0.5, 0.5, 0.5, 1.0])
                else:
                    obstacle_id = self.create_cylinder(mass=0.0, radius=self.obstacle_radius, height=self.tree_height, position=[x, y, self.terrain_position[2] + self.terrain_size[2] / 2 + self.tree_height / 2], orientation=[0.0, 0.0, 0.0, 1.0], color=[0.0, 0.5, 0.0, 1.0])
                self.obstacle_ids.append(obstacle_id)

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        survival = 1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        collision = -1.0 if any((len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0 for obstacle_id in self.obstacle_ids)) else 0.0
        return {'survival': survival, 'reach_platform_end': reach_platform_end, 'collision': collision}

    def get_terminated(self, action):
        is_fall_off = self.robot.links['base'].position[2] < self.terrain_position[2]
        is_collision = any((len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=obstacle_id)) > 0 for obstacle_id in self.obstacle_ids))
        return is_fall_off or is_collision

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_size[0] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_14.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Jump from static platform to static platform to cross lava.

    Description:
    - The environment consists of a start platform (3 m x 3 m x 0.5 m) and an end platform (3 m x 3 m x 0.5 m) placed 20 meters apart.
    - The two platforms are connected by a series of 5 static platforms (2 m x 2 m x 0.5 m) placed 3 meters apart.
    - The platforms are placed above a lava surface, and the robot must jump from one static platform to the next to reach the end platform.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    - The robot receives a reward for each time step it remains on the platforms, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.
    - The robot is penalized for falling into the lava.

    Termination:
    The task terminates immediately if the robot falls into the lava or reaches the end platform.
    """

    def __init__(self):
        super().__init__()
        self.lava_size = [1000.0, 1000.0, 10.0]
        self.lava_position = [0.0, 0.0, 0.0]
        self.lava_id = self.create_box(mass=0.0, half_extents=[self.lava_size[0] / 2, self.lava_size[1] / 2, self.lava_size[2] / 2], position=self.lava_position, color=[1.0, 0.3, 0.1, 1.0])
        self.platform_start_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, self.lava_position[2] + self.lava_size[2] / 2 + self.platform_start_size[2] / 2]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_start_size[0] / 2, self.platform_start_size[1] / 2, self.platform_start_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_size = [3.0, 3.0, 0.5]
        self.platform_end_position = [self.platform_start_position[0] + 20.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_end_size[0] / 2, self.platform_end_size[1] / 2, self.platform_end_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.num_static_platforms = 5
        self.static_platform_size = [2.0, 2.0, 0.5]
        self.static_platform_ids = []
        for i in range(self.num_static_platforms):
            static_platform_position = [self.platform_start_position[0] + (i + 1) * 3.0, self.platform_start_position[1], self.platform_start_position[2]]
            static_platform_id = self.create_box(mass=0.0, half_extents=[self.static_platform_size[0] / 2, self.static_platform_size[1] / 2, self.static_platform_size[2] / 2], position=static_platform_position, color=[0.8, 0.8, 0.8, 1.0])
            self.static_platform_ids.append(static_platform_id)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_start_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        on_platform = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] else -1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        return {'on_platform': on_platform, 'reach_platform_end': reach_platform_end}

    def get_terminated(self, action):
        is_in_lava = self.robot.links['base'].position[2] < self.lava_position[2] + self.lava_size[2] / 2
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_end_size[0] / 2
        return is_in_lava or is_on_platform_end

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_end_size[0] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_15.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Jump from static platform to static platform while avoiding moving obstacles.

    Description:
    - The environment consists of a start platform (3 m x 3 m x 0.5 m) and an end platform (3 m x 3 m x 0.5 m) placed 20 meters apart.
    - The two platforms are connected by a series of 5 static platforms (2 m x 2 m x 0.5 m) placed 3 meters apart.
    - Between these static platforms, moving obstacles (cylinders with a radius of 0.5 m and height of 1 m) move along the y-axis with a sinusoidal motion. The amplitude of the motion is 2 meters, and the period is 4 seconds. The motion of each obstacle is offset by 0.8 seconds from the previous one.
    - The platforms and obstacles are placed above a water surface, and the robot must jump from one static platform to the next while avoiding the moving obstacles to reach the end platform.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    - The robot receives a reward for each time step it remains on the platforms, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.
    - The robot is penalized for collisions with moving obstacles.

    Termination:
    The task terminates immediately if the robot falls into the water, collides with an obstacle, or reaches the end platform.
    """

    def __init__(self):
        super().__init__()
        self.water_size = [1000.0, 1000.0, 10.0]
        self.water_position = [0.0, 0.0, 0.0]
        self.water_id = self.create_box(mass=0.0, half_extents=[self.water_size[0] / 2, self.water_size[1] / 2, self.water_size[2] / 2], position=self.water_position, color=[0.0, 0.0, 1.0, 0.5])
        self.platform_start_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, self.water_position[2] + self.water_size[2] / 2 + self.platform_start_size[2] / 2]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_start_size[0] / 2, self.platform_start_size[1] / 2, self.platform_start_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_size = [3.0, 3.0, 0.5]
        self.platform_end_position = [self.platform_start_position[0] + 20.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_end_size[0] / 2, self.platform_end_size[1] / 2, self.platform_end_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.num_static_platforms = 5
        self.static_platform_size = [2.0, 2.0, 0.5]
        self.static_platform_ids = []
        for i in range(self.num_static_platforms):
            static_platform_position = [self.platform_start_position[0] + (i + 1) * 3.0, self.platform_start_position[1], self.platform_start_position[2]]
            static_platform_id = self.create_box(mass=0.0, half_extents=[self.static_platform_size[0] / 2, self.static_platform_size[1] / 2, self.static_platform_size[2] / 2], position=static_platform_position, color=[0.8, 0.8, 0.8, 1.0])
            self.static_platform_ids.append(static_platform_id)
        self.num_moving_obstacles = 4
        self.moving_obstacle_radius = 0.5
        self.moving_obstacle_height = 1.0
        self.moving_obstacle_amplitude = 2.0
        self.moving_obstacle_period = 4.0
        self.moving_obstacle_phase_offset = 0.8
        self.moving_obstacle_ids = []
        for i in range(self.num_moving_obstacles):
            moving_obstacle_position = [self.platform_start_position[0] + (i + 1) * 3.0 + 1.5, self.platform_start_position[1], self.platform_start_position[2] + self.moving_obstacle_height / 2]
            moving_obstacle_id = self.create_cylinder(mass=0.0, radius=self.moving_obstacle_radius, height=self.moving_obstacle_height, position=moving_obstacle_position, color=[1.0, 0.0, 0.0, 1.0])
            self.moving_obstacle_ids.append(moving_obstacle_id)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_start_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        for i, moving_obstacle_id in enumerate(self.moving_obstacle_ids):
            moving_obstacle_position = self.get_object_position(moving_obstacle_id)
            new_moving_obstacle_position = [moving_obstacle_position[0], self.platform_start_position[1] + self.moving_obstacle_amplitude * np.sin(2 * np.pi * (self.time + i * self.moving_obstacle_phase_offset) / self.moving_obstacle_period), moving_obstacle_position[2]]
            self._p.resetBasePositionAndOrientation(moving_obstacle_id, new_moving_obstacle_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        on_platform = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] else -1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        collision_with_obstacle = -1.0 if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.moving_obstacle_ids[0])) > 0 or len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.moving_obstacle_ids[1])) > 0 or len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.moving_obstacle_ids[2])) > 0 or (len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.moving_obstacle_ids[3])) > 0) else 0.0
        return {'on_platform': on_platform, 'reach_platform_end': reach_platform_end, 'collision_with_obstacle': collision_with_obstacle}

    def get_terminated(self, action):
        is_in_water = self.robot.links['base'].position[2] < self.water_position[2] + self.water_size[2] / 2
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_end_size[0] / 2
        collision_with_obstacle = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.moving_obstacle_ids[0])) > 0 or len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.moving_obstacle_ids[1])) > 0 or len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.moving_obstacle_ids[2])) > 0 or (len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.moving_obstacle_ids[3])) > 0)
        return is_in_water or is_on_platform_end or collision_with_obstacle

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_end_size[0] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_16.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Jump over rolling logs on a bridge

    Description:
    - The environment consists of a wide static bridge that is 50 meters long and 5 meters wide, elevated 10 meters above a water surface.
    - The robot starts at the beginning of the bridge, facing the positive x-axis.
    - Logs (cylinders) with a radius of 0.5 meters are spawned 2 meters above the bridge and 10 meters ahead of the robot, rolling towards the robot with an initial velocity of 5 m/s along the negative x-axis.
    - The robot must move forward on the bridge while jumping over the rolling logs to reach the end of the bridge.

    Success:
    The task is successfully completed when the robot reaches the end of the bridge.

    Rewards:
    - The robot receives a survival reward for each time step it remains on the bridge, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the end of the bridge, incentivizing swift movement towards the goal.
    - The robot is penalized for colliding with the logs.

    Termination:
    The task terminates immediately if the robot falls off the bridge, collides with a log, or reaches the end of the bridge.
    """

    def __init__(self):
        super().__init__()
        self.water_size = [1000.0, 1000.0, 10.0]
        self.water_position = [0.0, 0.0, 0.0]
        self.water_id = self.create_box(mass=0.0, half_extents=[self.water_size[0] / 2, self.water_size[1] / 2, self.water_size[2] / 2], position=self.water_position, color=[0.0, 0.0, 1.0, 0.5])
        self.bridge_length = 50.0
        self.bridge_width = 5.0
        self.bridge_height = 0.5
        self.bridge_position = [self.water_position[0] + self.bridge_length / 2, self.water_position[1], self.water_position[2] + self.water_size[2] / 2 + self.bridge_height / 2]
        self.bridge_id = self.create_box(mass=0.0, half_extents=[self.bridge_length / 2, self.bridge_width / 2, self.bridge_height / 2], position=self.bridge_position, color=[0.8, 0.8, 0.8, 1.0])
        self.log_radius = 0.5
        self.log_height = 2.0
        self.log_spawn_distance = 10.0
        self.log_spawn_height = 2.0
        self.log_velocity = -5.0
        self.log_ids = []
        self.robot_position_init = [self.bridge_position[0] - self.bridge_length / 2 + 1.0, self.bridge_position[1], self.bridge_position[2] + self.bridge_height / 2 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, orientation, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position, baseOrientation=orientation)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        for log_id in self.log_ids:
            self._p.removeBody(log_id)
        self.log_ids = []
        return observation

    def step(self, action):
        self.distance_to_bridge_end = self.bridge_length - (self.robot.links['base'].position[0] - (self.bridge_position[0] - self.bridge_length / 2))
        observation, reward, terminated, truncated, info = super().step(action)
        if np.random.rand() < 0.05:
            log_position = [self.robot.links['base'].position[0] + self.log_spawn_distance, self.bridge_position[1], self.bridge_position[2] + self.bridge_height / 2 + self.log_spawn_height]
            log_orientation = self._p.getQuaternionFromEuler([np.pi / 2, 0.0, 0.0])
            log_id = self.create_cylinder(mass=10.0, radius=self.log_radius, height=self.log_height, position=log_position, orientation=log_orientation, color=[0.8, 0.4, 0.2, 1.0])
            self._p.resetBaseVelocity(log_id, linearVelocity=[self.log_velocity, 0.0, 0.0])
            self.log_ids.append(log_id)
        for log_id in self.log_ids:
            log_position = self.get_object_position(log_id)
            if log_position[0] < self.bridge_position[0] - self.bridge_length / 2:
                self._p.removeBody(log_id)
                self.log_ids.remove(log_id)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_bridge_end = self.bridge_length - (self.robot.links['base'].position[0] - (self.bridge_position[0] - self.bridge_length / 2))
        survival = 1.0 if self.robot.links['base'].position[2] > self.bridge_position[2] else -1.0
        reach_bridge_end = (self.distance_to_bridge_end - new_distance_to_bridge_end) / self.dt
        collision_with_log = -1.0 if any((len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=log_id)) > 0 for log_id in self.log_ids)) else 0.0
        return {'survival': survival, 'reach_bridge_end': reach_bridge_end, 'collision_with_log': collision_with_log}

    def get_terminated(self, action):
        is_off_bridge = self.robot.links['base'].position[2] < self.bridge_position[2]
        is_at_bridge_end = self.robot.links['base'].position[0] > self.bridge_position[0] + self.bridge_length / 2
        collision_with_log = any((len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=log_id)) > 0 for log_id in self.log_ids))
        return is_off_bridge or is_at_bridge_end or collision_with_log

    def get_success(self):
        is_at_bridge_end = self.robot.links['base'].position[0] > self.bridge_position[0] + self.bridge_length / 2
        return is_at_bridge_end
\end{lstlisting}


==> env_codes/short_run/short_run_17.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Touch a lever or a button to activate a drawbridge. The robot is on a start platform and needs to reach a target platform 25 m away. A 25-meter long drawbridge is on the end platform in an open (upright) position. A button or lever can be activated to lower the drawbridge to connect the two platforms.

    Description:
    - The environment consists of a start platform (3 m x 3 m x 0.5 m) and an end platform (3 m x 3 m x 0.5 m) placed 25 meters apart.
    - A drawbridge (25 m long and 2 m wide) is positioned at the edge of the end platform in an upright position.
    - A button or lever is placed on the start platform.
    - The robot must touch the button or lever to lower the drawbridge, allowing it to cross to the end platform.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    - The robot receives a reward for each time step it remains on the platforms, encouraging steady progress.
    - The robot is rewarded for touching the button or lever.
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.

    Termination:
    The task terminates immediately if the robot falls off the platforms or reaches the end platform.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 25.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.drawbridge_length = 25.0
        self.drawbridge_width = 2.0
        self.drawbridge_thickness = 0.2
        self.drawbridge_position_lowered = [self.platform_start_position[0] + self.platform_size[0] / 2 + self.drawbridge_length / 2, self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.drawbridge_thickness / 2]
        self.drawbridge_position_raised = [self.platform_end_position[0] - self.platform_size[0] / 2, self.platform_end_position[1], self.platform_end_position[2] + self.platform_size[2] / 2 + self.drawbridge_length / 2]
        self.drawbridge_id = self.create_box(mass=0.0, half_extents=[self.drawbridge_length / 2, self.drawbridge_width / 2, self.drawbridge_thickness / 2], position=self.drawbridge_position_raised, color=[0.6, 0.3, 0.0, 1.0])
        self.button_radius = 0.2
        self.button_height = 0.1
        self.button_position = [self.platform_start_position[0] + self.platform_size[0] / 2 - 0.5, self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.button_height / 2]
        self.button_id = self.create_cylinder(mass=0.0, radius=self.button_radius, height=self.button_height, position=self.button_position, color=[1.0, 0.0, 0.0, 1.0])
        self.drawbridge_activated = False

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        self.drawbridge_activated = False
        self._p.resetBasePositionAndOrientation(self.drawbridge_id, self.drawbridge_position_raised, [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        if not self.drawbridge_activated and len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.button_id)) > 0:
            self.drawbridge_activated = True
            self._p.resetBasePositionAndOrientation(self.drawbridge_id, self.drawbridge_position_lowered, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        on_platforms = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] + self.platform_size[2] / 2 else -1.0
        activate_drawbridge = 10.0 if not self.drawbridge_activated and len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.button_id)) > 0 else 0.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        return {'on_platforms': on_platforms, 'activate_drawbridge': activate_drawbridge, 'reach_platform_end': reach_platform_end}

    def get_terminated(self, action):
        is_off_platforms = self.robot.links['base'].position[2] < self.platform_start_position[2]
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_size[0] / 2
        return is_off_platforms or is_on_platform_end

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_size[0] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_18.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Push a cube to a target zone on a static platform

    Description:
    - The environment consists of a large static platform (50 m x 50 m).
    - A cube (2 meters in size and 5 kg in mass) is placed at a random location on the platform.
    - A target zone (3 meters in radius) is also placed at a random location on the platform. The collision for the target zone is set to False.
    - The robot is initialized at a fixed position on the platform.

    The task of the robot is to push the cube to the target zone as quickly as possible.

    Success:
    The task is successfully completed when the cube is entirely within the target zone.

    Rewards:
    - The robot receives a survival reward for each time step it remains on the platform, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the cube, incentivizing interaction with the cube.
    - The robot is rewarded based on how much it reduces the distance between the cube and the target zone, incentivizing pushing the cube towards the goal.
    - A large reward is given when the cube reaches the target zone.

    Termination:
    The episode terminates if the robot falls off the platform or if the cube reaches the target zone.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [50.0, 50.0, 0.1]
        self.platform_position = [0.0, 0.0, 0.0]
        self.platform_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_position, color=[0.8, 0.8, 0.8, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.platform_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.cube_size = [2.0, 2.0, 2.0]
        self.cube_mass = 5.0
        self.cube_id = self.create_box(mass=self.cube_mass, half_extents=[self.cube_size[0] / 2, self.cube_size[1] / 2, self.cube_size[2] / 2], position=[0.0, 0.0, 0.0], color=[1.0, 0.0, 0.0, 1.0])
        self.target_zone_radius = 3.0
        self.target_zone_id = self.create_sphere(mass=0.0, radius=self.target_zone_radius, collision=False, position=[0.0, 0.0, 0.0], color=[0.0, 1.0, 0.0, 0.5])
        self.robot_position_init = [0.0, 0.0, self.platform_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, collision, position, color):
        if collision:
            collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
            visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
            return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)
        else:
            visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
            return self._p.createMultiBody(baseMass=mass, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_between_objects(self, object1_id, object2_id):
        object1_position = self.get_object_position(object1_id)
        object2_position = self.get_object_position(object2_id)
        return np.linalg.norm(object1_position[:2] - object2_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        cube_x = np.random.uniform(self.platform_position[0] - self.platform_size[0] / 2 + self.cube_size[0] / 2, self.platform_position[0] + self.platform_size[0] / 2 - self.cube_size[0] / 2)
        cube_y = np.random.uniform(self.platform_position[1] - self.platform_size[1] / 2 + self.cube_size[1] / 2, self.platform_position[1] + self.platform_size[1] / 2 - self.cube_size[1] / 2)
        self._p.resetBasePositionAndOrientation(self.cube_id, [cube_x, cube_y, self.platform_position[2] + self.platform_size[2] / 2 + self.cube_size[2] / 2], [0.0, 0.0, 0.0, 1.0])
        target_zone_x = np.random.uniform(self.platform_position[0] - self.platform_size[0] / 2 + self.target_zone_radius, self.platform_position[0] + self.platform_size[0] / 2 - self.target_zone_radius)
        target_zone_y = np.random.uniform(self.platform_position[1] - self.platform_size[1] / 2 + self.target_zone_radius, self.platform_position[1] + self.platform_size[1] / 2 - self.target_zone_radius)
        self._p.resetBasePositionAndOrientation(self.target_zone_id, [target_zone_x, target_zone_y, self.platform_position[2] + self.platform_size[2] / 2], [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_robot_to_cube = self.get_distance_between_objects(self.robot.robot_id, self.cube_id)
        self.distance_cube_to_target_zone = self.get_distance_between_objects(self.cube_id, self.target_zone_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_robot_to_cube = self.get_distance_between_objects(self.robot.robot_id, self.cube_id)
        new_distance_cube_to_target_zone = self.get_distance_between_objects(self.cube_id, self.target_zone_id)
        survival = 1.0
        reach_cube = (self.distance_robot_to_cube - new_distance_robot_to_cube) / self.dt
        push_cube_to_target_zone = (self.distance_cube_to_target_zone - new_distance_cube_to_target_zone) / self.dt
        cube_in_target_zone = 10.0 if new_distance_cube_to_target_zone < self.target_zone_radius else 0.0
        return {'survival': survival, 'reach_cube': reach_cube, 'push_cube_to_target_zone': push_cube_to_target_zone, 'cube_in_target_zone': cube_in_target_zone}

    def get_terminated(self, action):
        is_off_platform = self.robot.links['base'].position[2] < self.platform_position[2]
        is_cube_in_target_zone = self.get_distance_between_objects(self.cube_id, self.target_zone_id) < self.target_zone_radius
        return is_off_platform or is_cube_in_target_zone

    def get_success(self):
        is_cube_in_target_zone = self.get_distance_between_objects(self.cube_id, self.target_zone_id) < self.target_zone_radius
        return is_cube_in_target_zone
\end{lstlisting}


==> env_codes/short_run/short_run_19.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Push a cube into a target zone in a large open arena.

    Description:
    - The environment consists of a large flat arena measuring 50 x 50 meters.
    - A cube with dimensions of 2 meters in size and a mass of 5 kg is placed at a random location within the arena.
    - A target zone with a radius of 3 meters is also randomly placed within the arena. The target zone has no collision, allowing the cube to be pushed into it without obstruction.
    - The robot is initialized at a random position within the arena, facing the positive x-axis.

    Success:
    The task is successfully completed when the robot pushes the cube into the target zone.

    Rewards:
    - The robot receives a survival reward at each time step to encourage steady progress.
    - The robot is rewarded for decreasing its distance to the cube, encouraging it to approach and interact with the cube.
    - The robot is rewarded for pushing the cube towards the target zone, with additional rewards for getting the cube into the target zone.
    - The robot is rewarded for remaining within the arena, avoiding falling off the platform.

    Termination:
    The episode terminates if the robot falls off the platform. The episode does not terminate if the cube is in the target zone.
    """

    def __init__(self):
        super().__init__()
        self.arena_size = [50.0, 50.0, 0.1]
        self.arena_position = [0.0, 0.0, 0.0]
        self.arena_id = self.create_box(mass=0.0, half_extents=[self.arena_size[0] / 2, self.arena_size[1] / 2, self.arena_size[2] / 2], position=self.arena_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.arena_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.cube_size = [2.0, 2.0, 2.0]
        self.cube_mass = 5.0
        self.cube_id = self.create_box(mass=self.cube_mass, half_extents=[self.cube_size[0] / 2, self.cube_size[1] / 2, self.cube_size[2] / 2], position=[0.0, 0.0, 0.0], color=[1.0, 0.0, 0.0, 1.0])
        self.target_zone_radius = 3.0
        self.target_zone_id = self.create_sphere(mass=0.0, radius=self.target_zone_radius, collision=False, position=[0.0, 0.0, 0.0], color=[0.0, 1.0, 0.0, 0.5])

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, collision, position, color):
        if collision:
            collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
            visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
            return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)
        else:
            visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
            return self._p.createMultiBody(baseMass=mass, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        cube_x_init = np.random.uniform(low=-self.arena_size[0] / 2 + self.cube_size[0] / 2, high=self.arena_size[0] / 2 - self.cube_size[0] / 2)
        cube_y_init = np.random.uniform(low=-self.arena_size[1] / 2 + self.cube_size[1] / 2, high=self.arena_size[1] / 2 - self.cube_size[1] / 2)
        self._p.resetBasePositionAndOrientation(self.cube_id, [cube_x_init, cube_y_init, self.arena_position[2] + self.arena_size[2] / 2 + self.cube_size[2] / 2], [0.0, 0.0, 0.0, 1.0])
        target_zone_x = np.random.uniform(low=-self.arena_size[0] / 2 + self.target_zone_radius, high=self.arena_size[0] / 2 - self.target_zone_radius)
        target_zone_y = np.random.uniform(low=-self.arena_size[1] / 2 + self.target_zone_radius, high=self.arena_size[1] / 2 - self.target_zone_radius)
        self.target_zone_position = [target_zone_x, target_zone_y, self.arena_position[2] + self.arena_size[2] / 2]
        self._p.resetBasePositionAndOrientation(self.target_zone_id, self.target_zone_position, [0.0, 0.0, 0.0, 1.0])
        robot_x_init = np.random.uniform(low=-self.arena_size[0] / 2 + self.robot.links['base'].position_init[0], high=self.arena_size[0] / 2 - self.robot.links['base'].position_init[0])
        robot_y_init = np.random.uniform(low=-self.arena_size[1] / 2 + self.robot.links['base'].position_init[1], high=self.arena_size[1] / 2 - self.robot.links['base'].position_init[1])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [robot_x_init, robot_y_init, self.arena_position[2] + self.arena_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_cube = self.get_distance_to_object(self.cube_id)
        self.distance_cube_to_target_zone = self.get_distance_to_object(self.target_zone_id)
        self.cube_position = self.get_object_position(self.cube_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_cube = self.get_distance_to_object(self.cube_id)
        new_distance_cube_to_target_zone = self.get_distance_to_object(self.target_zone_id)
        new_cube_position = self.get_object_position(self.cube_id)
        survival = 1.0
        reach_cube = (self.distance_to_cube - new_distance_to_cube) / self.dt
        push_cube = (self.distance_cube_to_target_zone - new_distance_cube_to_target_zone) / self.dt
        if new_distance_cube_to_target_zone < self.target_zone_radius:
            push_cube += 5.0
        in_arena = 1.0 if abs(self.robot.links['base'].position[0]) < self.arena_size[0] / 2 and abs(self.robot.links['base'].position[1]) < self.arena_size[1] / 2 else -1.0
        return {'survival': survival, 'reach_cube': reach_cube, 'push_cube': push_cube, 'in_arena': in_arena}

    def get_terminated(self, action):
        return abs(self.robot.links['base'].position[0]) > self.arena_size[0] / 2 or abs(self.robot.links['base'].position[1]) > self.arena_size[1] / 2

    def get_success(self):
        cube_distance_to_target_zone = self.get_distance_to_object(self.target_zone_id)
        return cube_distance_to_target_zone < self.target_zone_radius
\end{lstlisting}


==> env_codes/short_run/short_run_21.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Push a domino to start a chain reaction.

    Description:
    - The environment consists of a large platform measuring 1000 x 10 x 0.1 meters.
    - The robot is initialized at a fixed position on the platform.
    - A domino with dimensions 0.5 x 2 x 4 meters and a mass of 5 kg is positioned on the platform, 5 meters away from the robot.
    - The dominos are spaced by 3 meters, and positioned to create a chain reaction.
    - The task of the robot is to push the domino to start a chain reaction.

    Success:
    The task is successfully completed when the robot pushes the domino and starts the chain reaction.

    Rewards:
    - The robot is rewarded for forward progress towards the domino, encouraging it to approach and push the domino.
    - The robot is rewarded for the number of dominos that fall, incentivizing it to initiate the chain reaction.
    - The robot is penalized for falling off the platform, ensuring it stays on the platform.

    Termination:
    The task terminates immediately if the robot falls off the platform.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [1000.0, 10.0, 0.1]
        self.platform_position = [0.0, 0.0, 0.0]
        self.platform_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.platform_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.domino_size = [0.5, 2.0, 4.0]
        self.domino_mass = 5.0
        self.domino_spacing = 3.0
        self.num_dominos = 10
        self.domino_ids = []
        for i in range(self.num_dominos):
            domino_position = [self.platform_position[0] + 5.0 + i * self.domino_spacing, self.platform_position[1], self.platform_position[2] + self.platform_size[2] / 2 + self.domino_size[2] / 2]
            domino_id = self.create_box(mass=self.domino_mass, half_extents=[self.domino_size[0] / 2, self.domino_size[1] / 2, self.domino_size[2] / 2], position=domino_position, color=[1.0, 0.0, 0.0, 1.0])
            self.domino_ids.append(domino_id)
        self.robot_position_init = [self.platform_position[0], self.platform_position[1], self.platform_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        for i, domino_id in enumerate(self.domino_ids):
            domino_position = [self.platform_position[0] + 5.0 + i * self.domino_spacing, self.platform_position[1], self.platform_position[2] + self.platform_size[2] / 2 + self.domino_size[2] / 2]
            self._p.resetBasePositionAndOrientation(domino_id, domino_position, [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_first_domino = self.get_distance_to_object(self.domino_ids[0])
        self.num_fallen_dominos = sum([self._p.getBaseVelocity(domino_id)[0][2] < -0.1 for domino_id in self.domino_ids])
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_first_domino = self.get_distance_to_object(self.domino_ids[0])
        new_num_fallen_dominos = sum([self._p.getBaseVelocity(domino_id)[0][2] < -0.1 for domino_id in self.domino_ids])
        forward_progress = (self.distance_to_first_domino - new_distance_to_first_domino) / self.dt
        domino_fall_reward = (new_num_fallen_dominos - self.num_fallen_dominos) * 10.0
        return {'forward_progress': forward_progress, 'domino_fall_reward': domino_fall_reward}

    def get_terminated(self, action):
        return self.robot.links['base'].position[2] < self.platform_position[2]

    def get_success(self):
        return any([self._p.getBaseVelocity(domino_id)[0][2] < -0.1 for domino_id in self.domino_ids])
\end{lstlisting}


==> env_codes/short_run/short_run_23.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Destroy a tower of blocks

    Description:
    - The environment consists of a large flat platform measuring 50 meters by 50 meters.
    - A tower of 10 blocks is placed at a random location on the platform. Each block is a cube measuring 1 meter by 1 meter by 1 meter and weighs 5 kg. The blocks are of different colors to make the environment visually rich.
    - The robot is initialized at a fixed position on the platform, facing the tower.

    The task of the robot is to destroy the tower by pushing the blocks until all blocks are knocked over and no longer stacked.

    Success:
    The task is successfully completed when all blocks are knocked over and none are stacked on top of each other.

    Rewards:
    - The robot receives a survival reward for each time step it remains on the platform, encouraging steady progress.
    - The robot is rewarded for reducing the height of the tower, incentivizing the robot to knock over the blocks.
    - A large reward is given when all blocks are knocked over and none are stacked.

    Termination:
    The episode terminates if the robot falls off the platform or if all blocks are knocked over and none are stacked.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [50.0, 50.0, 0.1]
        self.platform_position = [0.0, 0.0, 0.0]
        self.platform_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_position, color=[0.8, 0.8, 0.8, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.platform_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.block_size = [1.0, 1.0, 1.0]
        self.block_mass = 5.0
        self.num_blocks = 10
        self.block_ids = []
        self.block_colors = [[1.0, 0.0, 0.0, 1.0], [0.0, 1.0, 0.0, 1.0], [0.0, 0.0, 1.0, 1.0], [1.0, 1.0, 0.0, 1.0], [1.0, 0.0, 1.0, 1.0], [0.0, 1.0, 1.0, 1.0], [0.5, 0.5, 0.5, 1.0], [1.0, 0.5, 0.0, 1.0], [0.5, 0.0, 0.5, 1.0], [0.0, 0.5, 0.5, 1.0]]
        for i in range(self.num_blocks):
            block_id = self.create_box(mass=self.block_mass, half_extents=[self.block_size[0] / 2, self.block_size[1] / 2, self.block_size[2] / 2], position=[0.0, 0.0, 0.0], color=self.block_colors[i])
            self.block_ids.append(block_id)
        self.robot_position_init = [0.0, 0.0, self.platform_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_between_objects(self, object1_id, object2_id):
        object1_position = self.get_object_position(object1_id)
        object2_position = self.get_object_position(object2_id)
        return np.linalg.norm(object1_position[:2] - object2_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        tower_x = np.random.uniform(self.platform_position[0] - self.platform_size[0] / 2 + self.block_size[0] / 2, self.platform_position[0] + self.platform_size[0] / 2 - self.block_size[0] / 2)
        tower_y = np.random.uniform(self.platform_position[1] - self.platform_size[1] / 2 + self.block_size[1] / 2, self.platform_position[1] + self.platform_size[1] / 2 - self.block_size[1] / 2)
        for i, block_id in enumerate(self.block_ids):
            self._p.resetBasePositionAndOrientation(block_id, [tower_x, tower_y, self.platform_position[2] + self.platform_size[2] / 2 + (i + 0.5) * self.block_size[2]], [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.tower_height = self.calculate_tower_height()
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def calculate_tower_height(self):
        heights = [self.get_object_position(block_id)[2] for block_id in self.block_ids]
        return max(heights) - min(heights)

    def get_task_rewards(self, action):
        new_tower_height = self.calculate_tower_height()
        survival = 1.0
        reduce_tower_height = (self.tower_height - new_tower_height) / self.dt
        all_blocks_knocked_over = 10.0 if new_tower_height <= self.block_size[2] else 0.0
        return {'survival': survival, 'reduce_tower_height': reduce_tower_height, 'all_blocks_knocked_over': all_blocks_knocked_over}

    def get_terminated(self, action):
        is_off_platform = self.robot.links['base'].position[2] < self.platform_position[2]
        all_blocks_knocked_over = self.calculate_tower_height() <= self.block_size[2]
        return is_off_platform or all_blocks_knocked_over

    def get_success(self):
        all_blocks_knocked_over = self.calculate_tower_height() <= self.block_size[2]
        return all_blocks_knocked_over
\end{lstlisting}


==> env_codes/short_run/short_run_24.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Task: Navigate a dynamic platform to touch a target

    Description:
    - The environment consists of a start platform (3 m x 3 m x 0.5 m) and an end platform (3 m x 3 m x 0.5 m) placed 20 meters apart.
    - The two platforms are connected by a dynamic bridge (2 m wide) divided into 5 segments of equal length (3 m each).
    - Each segment moves up and down independently with a sinusoidal motion. The amplitude is 1 meter and the period is 2 seconds, with each segment offset in phase by 0.4 seconds from the previous one.
    - A target object (a cylinder with a radius of 0.2 meters and a height of 0.5 meters) is placed on the end platform.
    - The robot is initialized on the start platform, facing the dynamic bridge and the target object.
    - The task of the robot is to navigate the dynamic bridge and touch the target object on the end platform.

    Success:
    The task is successfully completed when the robot touches the target object on the end platform.

    Rewards:
    - The robot receives a reward for each time step it remains on the bridge or platforms, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the target object, incentivizing swift movement towards the goal.
    - The robot receives a large reward for touching the target object.

    Termination:
    The task terminates immediately if the robot falls off the start platform, any segment of the bridge, or the end platform, or if the robot touches the target object.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 20.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.bridge_length = self.platform_end_position[0] - self.platform_start_position[0] - self.platform_size[0]
        self.bridge_width = 2.0
        self.num_segments = 5
        self.segment_length = self.bridge_length / self.num_segments
        self.segment_amplitude = 1.0
        self.segment_period = 2.0
        self.segment_phase_offset = 0.4
        segment_colors = [[1.0, 0.0, 0.0, 1.0], [1.0, 0.5, 0.0, 1.0], [1.0, 1.0, 0.0, 1.0], [0.0, 1.0, 0.0, 1.0], [0.0, 0.0, 1.0, 1.0]]
        self.segment_ids = []
        for i in range(self.num_segments):
            segment_id = self.create_box(mass=0.0, half_extents=[self.segment_length / 2, self.bridge_width / 2, self.platform_size[2] / 2], position=[self.platform_start_position[0] + self.platform_size[0] / 2 + self.segment_length / 2 + i * self.segment_length, self.platform_start_position[1], self.platform_start_position[2]], color=segment_colors[i])
            self._p.changeDynamics(bodyUniqueId=segment_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
            self.segment_ids.append(segment_id)
        self.target_radius = 0.2
        self.target_height = 0.5
        self.target_position = [self.platform_end_position[0], self.platform_end_position[1], self.platform_end_position[2] + self.platform_size[2] / 2 + self.target_height / 2]
        self.target_id = self.create_cylinder(mass=0.0, radius=self.target_radius, height=self.target_height, position=self.target_position, color=[0.0, 1.0, 0.0, 1.0])

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_target = self.get_distance_to_object(self.target_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        for i, segment_id in enumerate(self.segment_ids):
            segment_position = self.get_object_position(segment_id)
            new_segment_position = [segment_position[0], segment_position[1], self.platform_start_position[2] + self.segment_amplitude * np.sin(2 * np.pi * (self.time + i * self.segment_phase_offset) / self.segment_period)]
            self._p.resetBasePositionAndOrientation(segment_id, new_segment_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_target = self.get_distance_to_object(self.target_id)
        on_bridge_or_platforms = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] + self.platform_size[2] / 2 else -1.0
        reach_target = (self.distance_to_target - new_distance_to_target) / self.dt
        touch_target = 10.0 if len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.target_id)) > 0 else 0.0
        return {'on_bridge_or_platforms': on_bridge_or_platforms, 'reach_target': reach_target, 'touch_target': touch_target}

    def get_terminated(self, action):
        is_off_bridge_or_platforms = self.robot.links['base'].position[2] < self.platform_start_position[2]
        is_touching_target = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.target_id)) > 0
        return is_off_bridge_or_platforms or is_touching_target

    def get_success(self):
        is_touching_target = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.target_id)) > 0
        return is_touching_target
\end{lstlisting}


==> env_codes/short_run/short_run_25.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Push a box next to a wall to climb on top of it.

    Description:
    - The environment consists of a large platform measuring 1000 x 10 x 0.1 meters.
    - The robot is initialized at a fixed position on the platform.
    - A wall with dimensions 0.5 x 10 x 2 meters is positioned on the platform, 5 meters away from the robot.
    - A box with dimensions 1 x 1 x 1 meters (5 kg in mass) is positioned on the platform, 3 meters away from the robot.
    - The task of the robot is first to push the box against the wall. Then, the robot must climb on top of the box and jump on top of the wall.

    Success:
    The task is successfully completed if the robot climbs on top of the box and then jumps on top of the wall.

    Rewards:
    - The robot receives a reward for each time step it remains on the platform.
    - The robot is rewarded for decreasing its distance to the box, encouraging it to approach and interact with the box.
    - The robot is rewarded for pushing the box towards the wall.
    - The robot is rewarded for climbing on top of the box and an additional reward for jumping on top of the wall.

    Termination:
    The episode terminates if the robot falls off the platform. The episode does not terminate if the robot successfully jumps on top of the wall.
    """

    def __init__(self):
        super().__init__()
        self.robot_position_init = [0.0, 0.0, 0.0]
        self.platform_size = [1000.0, 10.0, 0.1]
        self.platform_position = [self.robot_position_init[0] + self.platform_size[0] / 2 - 2.0, self.robot_position_init[1], self.robot_position_init[2] - self.platform_size[2] / 2]
        self.platform_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.platform_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.wall_size = [0.5, 10.0, 2.0]
        self.wall_position = [self.robot_position_init[0] + 5.0, self.platform_position[1], self.platform_position[2] + self.platform_size[2] / 2 + self.wall_size[2] / 2]
        self.wall_id = self.create_box(mass=0.0, half_extents=[self.wall_size[0] / 2, self.wall_size[1] / 2, self.wall_size[2] / 2], position=self.wall_position, color=[0.0, 0.0, 1.0, 1.0])
        self.box_size = [1.0, 1.0, 1.0]
        self.box_mass = 5.0
        self.box_position_init = [self.robot_position_init[0] + 3.0, self.platform_position[1], self.platform_position[2] + self.platform_size[2] / 2 + self.box_size[2] / 2]
        self.box_id = self.create_box(mass=self.box_mass, half_extents=[self.box_size[0] / 2, self.box_size[1] / 2, self.box_size[2] / 2], position=self.box_position_init, color=[1.0, 0.0, 0.0, 1.0])

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.box_id, self.box_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.robot_position_init[0], self.robot_position_init[1], self.robot_position_init[2] + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_box = self.get_distance_to_object(self.box_id)
        self.box_position = self.get_object_position(self.box_id)
        self.robot_on_box = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.box_id)) > 0
        self.robot_on_wall = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.wall_id)) > 0
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_box = self.get_distance_to_object(self.box_id)
        new_box_position = self.get_object_position(self.box_id)
        new_robot_on_box = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.box_id)) > 0
        new_robot_on_wall = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.wall_id)) > 0
        survival = 1.0
        reach_box = (self.distance_to_box - new_distance_to_box) / self.dt
        push_box = (new_box_position[0] - self.box_position[0]) / self.dt
        climb_on_box = 5.0 if new_robot_on_box and (not self.robot_on_box) else 0.0
        jump_on_wall = 10.0 if new_robot_on_wall and (not self.robot_on_wall) else 0.0
        return {'survival': survival, 'reach_box': reach_box, 'push_box': push_box, 'climb_on_box': climb_on_box, 'jump_on_wall': jump_on_wall}

    def get_terminated(self, action):
        return self.robot.links['base'].position[2] < self.platform_position[2]

    def get_success(self):
        return len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.wall_id)) > 0
\end{lstlisting}


==> env_codes/short_run/short_run_3.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Kick a ball into a goal with obstacles.

    Description: 
    - The environment consists of a large flat ground measuring 1000 x 1000 x 10 meters.
    - A ball with a radius of 0.5 meters is placed randomly on the ground, 5 meters in front of the robot's starting position.
    - The goal is defined by two goal posts, each 2 meters high and placed 3 meters apart, forming a goal area. The goal is positioned 10 meters in front of the robot's starting position.
    - Three box-shaped obstacles, each measuring 1 x 1 x 1 meters, are placed between the robot's starting position and the ball.
      - The first obstacle is placed 2 meters in front and 1 meter to the left of the robot. 
      - The second obstacle is placed 3 meters in front of the robot.
      - The third obstacle is placed 2 meters in front and 1 meter to the right of the robot.
    - The robot is initialized at a fixed position on the ground, facing the goal.
    - The task of the robot is to navigate around the obstacles, reach the ball, and kick it into the goal.

    Success:
    The task is successfully completed if the robot kicks the ball so that it passes between the two goal posts without colliding with any of the obstacles.

    Rewards:
    To help the robot complete the task:
    - The robot is rewarded for survival at each time step. 
    - The robot is rewarded for decreasing its distance to the ball while avoiding obstacles.
    - The robot is penalized for colliding with obstacles.
    - The robot is rewarded for kicking the ball towards the goal, with additional rewards for successfully kicking the ball into the goal.

    Termination:
    The task is terminated if the robot collides with any obstacle. Otherwise, it does not have a specific termination condition.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [1000.0, 1000.0, 10.0]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=[0.0, 0.0, 0.0], color=[1.0, 0.0, 0.0, 1.0])
        self.goal_post_height = 2.0
        self.goal_post_radius = 0.1
        self.goal_width = 3.0
        self.goal_position = [10.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.goal_post_height / 2]
        self.goal_post_left_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_position[0], self.goal_position[1] - self.goal_width / 2, self.goal_position[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.goal_post_right_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_position[0], self.goal_position[1] + self.goal_width / 2, self.goal_position[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.obstacle_size = [1.0, 1.0, 1.0]
        self.obstacle_1_id = self.create_box(mass=0.0, half_extents=[self.obstacle_size[0] / 2, self.obstacle_size[1] / 2, self.obstacle_size[2] / 2], position=[-3.0, -1.0, self.ground_position[2] + self.ground_size[2] / 2 + self.obstacle_size[2] / 2], color=[0.0, 0.0, 1.0, 1.0])
        self.obstacle_2_id = self.create_box(mass=0.0, half_extents=[self.obstacle_size[0] / 2, self.obstacle_size[1] / 2, self.obstacle_size[2] / 2], position=[-2.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.obstacle_size[2] / 2], color=[0.0, 0.0, 1.0, 1.0])
        self.obstacle_3_id = self.create_box(mass=0.0, half_extents=[self.obstacle_size[0] / 2, self.obstacle_size[1] / 2, self.obstacle_size[2] / 2], position=[-3.0, 1.0, self.ground_position[2] + self.ground_size[2] / 2 + self.obstacle_size[2] / 2], color=[0.0, 0.0, 1.0, 1.0])
        self.robot_position_init = [0.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        ball_y_init = np.random.uniform(-2.0, 2.0)
        self._p.resetBasePositionAndOrientation(self.ball_id, [5.0, ball_y_init, self.ground_position[2] + self.ground_size[2] / 2 + self.ball_radius], [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_ball = self.get_distance_to_object(self.ball_id)
        self.ball_position = self.get_object_position(self.ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_ball = self.get_distance_to_object(self.ball_id)
        new_ball_position = self.get_object_position(self.ball_id)
        survival = 1.0
        reach_ball = (self.distance_to_ball - new_distance_to_ball) / self.dt
        collision_obstacle_1 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_1_id)) > 0
        collision_obstacle_2 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_2_id)) > 0
        collision_obstacle_3 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_3_id)) > 0
        collision_penalty = -10.0 if collision_obstacle_1 or collision_obstacle_2 or collision_obstacle_3 else 0.0
        kick_ball = (new_ball_position[0] - self.ball_position[0]) / self.dt
        ball_in_goal = 0.0
        if self.goal_position[1] - self.goal_width / 2 < new_ball_position[1] < self.goal_position[1] + self.goal_width / 2 and new_ball_position[0] > self.goal_position[0]:
            ball_in_goal = 10.0
        return {'survival': survival, 'reach_ball': reach_ball, 'collision_penalty': collision_penalty, 'kick_ball': kick_ball, 'ball_in_goal': ball_in_goal}

    def get_terminated(self, action):
        collision_obstacle_1 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_1_id)) > 0
        collision_obstacle_2 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_2_id)) > 0
        collision_obstacle_3 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_3_id)) > 0
        return collision_obstacle_1 or collision_obstacle_2 or collision_obstacle_3

    def get_success(self):
        ball_position = self.get_object_position(self.ball_id)
        return self.goal_position[1] - self.goal_width / 2 < ball_position[1] < self.goal_position[1] + self.goal_width / 2 and ball_position[0] > self.goal_position[0]
\end{lstlisting}


==> env_codes/short_run/short_run_4.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Cross a rainbow bridge with moving segments and gaps to reach a platform.

    Description:
    - A start platform and an end platform (each 3 m in size and 0.5 m in thickness) are placed 25 m apart. 
    - The two platforms are connected by a bridge (2 m wide) divided into 6 segments of equal length (3 m each).
    - Each segment moves up and down independently with a sinusoidal motion. The amplitude is 1 m and the period is 2 seconds, with each segment offset in phase by 1/3 seconds from the previous one.
    - The segments are colored red, orange, yellow, green, blue, and purple, like a rainbow.
    - The segments have 1 m gaps between them.
    The robot is initialized on the start platform.
    The task of the robot is to cross the dynamic bridge to reach the end platform as fast as possible by timing its jumps between the moving segments and over the gaps.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    To help the robot complete the task:
    - The robot receives a reward for each time step it remains on the bridge or platforms, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.

    Termination: 
    The task terminates immediately if the robot falls off the start platform, any segment of the bridge, or the end platform.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 25.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.bridge_length = self.platform_end_position[0] - self.platform_start_position[0] - self.platform_size[0]
        self.bridge_width = 2.0
        self.num_segments = 6
        self.segment_length = 3.0
        self.gap_length = 1.0
        self.segment_amplitude = 1.0
        self.segment_period = 2.0
        self.segment_phase_offset = 1.0 / 3.0
        segment_colors = [[1.0, 0.0, 0.0, 1.0], [1.0, 0.5, 0.0, 1.0], [1.0, 1.0, 0.0, 1.0], [0.0, 1.0, 0.0, 1.0], [0.0, 0.0, 1.0, 1.0], [0.5, 0.0, 0.5, 1.0]]
        self.segment_ids = []
        for i in range(self.num_segments):
            segment_id = self.create_box(mass=0.0, half_extents=[self.segment_length / 2, self.bridge_width / 2, self.platform_size[2] / 2], position=[self.platform_start_position[0] + self.platform_size[0] / 2 + self.segment_length / 2 + i * (self.segment_length + self.gap_length), self.platform_start_position[1], self.platform_start_position[2]], color=segment_colors[i])
            self._p.changeDynamics(bodyUniqueId=segment_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
            self.segment_ids.append(segment_id)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        for i, segment_id in enumerate(self.segment_ids):
            segment_position = self.get_object_position(segment_id)
            new_segment_position = [segment_position[0], segment_position[1], self.platform_start_position[2] + self.segment_amplitude * np.sin(2 * np.pi * (self.time + i * self.segment_phase_offset) / self.segment_period)]
            self._p.resetBasePositionAndOrientation(segment_id, new_segment_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        on_bridge_or_platforms = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] + self.platform_size[2] / 2 else -1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        return {'on_bridge_or_platforms': on_bridge_or_platforms, 'reach_platform_end': reach_platform_end}

    def get_terminated(self, action):
        return self.robot.links['base'].position[2] < self.platform_start_position[2]

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_size[2] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_5.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Kick a ball into a moving goal.

    Description:
    - The environment consists of a large flat ground measuring 1000 x 1000 x 10 meters. 
    - A ball with a radius of 0.5 meters is placed on the ground, 5 meters directly in front of the robot's starting position.
    - The goal is defined by two goal posts, each 2 meters high and placed 3 meters apart, forming a goal area. 
    - The goal moves side-to-side (along the y-axis) in a sinusoidal motion with an amplitude of 2 meters and a period of 10 seconds. The center of its motion is 10 meters in front of the robot's starting position.
    - The robot is initialized at a fixed position on the ground, facing the goal.
    - The task of the robot is to move towards the ball, time its kick correctly, and kick the ball into the moving goal.

    Success:
    The task is successfully completed if the robot kicks the ball so that it passes between the two goal posts.

    Rewards:
    To help the robot complete the task:
    - The robot is rewarded for survival at each time step.
    - The robot is rewarded for decreasing its distance to the ball. 
    - The robot is rewarded for kicking the ball towards the goal, with additional rewards for successfully kicking the ball into the goal.

    Termination:
    The task does not have a specific termination condition. The episode ends after a fixed amount of time.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [1000.0, 1000.0, 10.0]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=[0.0, 0.0, 0.0], color=[1.0, 0.0, 0.0, 1.0])
        self.goal_post_height = 2.0
        self.goal_post_radius = 0.1
        self.goal_width = 3.0
        self.goal_position_init = [10.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.goal_post_height / 2]
        self.goal_post_left_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_position_init[0], self.goal_position_init[1] - self.goal_width / 2, self.goal_position_init[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.goal_post_right_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_position_init[0], self.goal_position_init[1] + self.goal_width / 2, self.goal_position_init[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.goal_amplitude = 2.0
        self.goal_period = 10.0
        self.robot_position_init = [self.ground_position[0], self.ground_position[1], self.ground_position[2] + self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        self._p.resetBasePositionAndOrientation(self.ball_id, [self.robot_position_init[0] + 5.0, self.robot_position_init[1], self.ground_position[2] + self.ground_size[2] / 2 + self.ball_radius], [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_ball = self.get_distance_to_object(self.ball_id)
        self.ball_position = self.get_object_position(self.ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        goal_y = self.goal_amplitude * np.sin(2 * np.pi * self.time / self.goal_period)
        self._p.resetBasePositionAndOrientation(self.goal_post_left_id, [self.goal_position_init[0], self.goal_position_init[1] - self.goal_width / 2 + goal_y, self.goal_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.goal_post_right_id, [self.goal_position_init[0], self.goal_position_init[1] + self.goal_width / 2 + goal_y, self.goal_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_ball = self.get_distance_to_object(self.ball_id)
        new_ball_position = self.get_object_position(self.ball_id)
        survival = 1.0
        reach_ball = (self.distance_to_ball - new_distance_to_ball) / self.dt
        kick_ball = (new_ball_position[0] - self.ball_position[0]) / self.dt
        goal_y = self.goal_amplitude * np.sin(2 * np.pi * self.time / self.goal_period)
        ball_in_goal = 0.0
        if self.goal_position_init[0] - self.goal_post_radius < new_ball_position[0] < self.goal_position_init[0] + self.goal_post_radius and self.goal_position_init[1] - self.goal_width / 2 + goal_y < new_ball_position[1] < self.goal_position_init[1] + self.goal_width / 2 + goal_y:
            ball_in_goal = 10.0
        return {'survival': survival, 'reach_ball': reach_ball, 'kick_ball': kick_ball, 'ball_in_goal': ball_in_goal}

    def get_terminated(self, action):
        return False

    def get_success(self):
        ball_position = self.get_object_position(self.ball_id)
        goal_y = self.goal_amplitude * np.sin(2 * np.pi * self.time / self.goal_period)
        return self.goal_position_init[0] - self.goal_post_radius < ball_position[0] < self.goal_position_init[0] + self.goal_post_radius and self.goal_position_init[1] - self.goal_width / 2 + goal_y < ball_position[1] < self.goal_position_init[1] + self.goal_width / 2 + goal_y
\end{lstlisting}


==> env_codes/short_run/short_run_6.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Kick a ball into a moving goal.

    Description:
    - The environment consists of a large flat ground measuring 1000 x 1000 x 10 meters.
    - A ball with a radius of 0.5 meters is placed on the ground, 5 meters directly in front of the robot's starting position.
    - The goal is defined by two goal posts, each 2 meters high and placed 3 meters apart, forming a goal area.
    - The goal moves side-to-side (along the y-axis) in a sinusoidal motion with an amplitude of 2 meters and a period of 10 seconds. The center of its motion is 10 meters in front of the robot's starting position.
    - The robot is initialized at a fixed position on the ground, facing the goal.
    - The task of the robot is to move towards the ball, time its kick correctly, and kick the ball into the moving goal.

    Success:
    The task is successfully completed if the robot kicks the ball so that it passes between the two goal posts.

    Rewards:
    To help the robot complete the task:
    - The robot is rewarded for survival at each time step.
    - The robot is rewarded for decreasing its distance to the ball.
    - The robot is rewarded for kicking the ball towards the goal, with additional rewards for successfully kicking the ball into the goal.

    Termination:
    The task terminates if the ball goes out of bounds or if the agent fails to kick the ball within a certain time frame.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [1000.0, 1000.0, 10.0]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=[0.0, 0.0, 0.0], color=[1.0, 0.0, 0.0, 1.0])
        self.goal_post_height = 2.0
        self.goal_post_radius = 0.1
        self.goal_width = 3.0
        self.goal_position_init = [10.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.goal_post_height / 2]
        self.goal_post_left_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_position_init[0], self.goal_position_init[1] - self.goal_width / 2, self.goal_position_init[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.goal_post_right_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_position_init[0], self.goal_position_init[1] + self.goal_width / 2, self.goal_position_init[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.goal_amplitude = 2.0
        self.goal_period = 10.0
        self.robot_position_init = [self.ground_position[0], self.ground_position[1], self.ground_position[2] + self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        self._p.resetBasePositionAndOrientation(self.ball_id, [self.robot_position_init[0] + 5.0, self.robot_position_init[1], self.ground_position[2] + self.ground_size[2] / 2 + self.ball_radius], [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_ball = self.get_distance_to_object(self.ball_id)
        self.ball_position = self.get_object_position(self.ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        goal_y = self.goal_amplitude * np.sin(2 * np.pi * self.time / self.goal_period)
        self._p.resetBasePositionAndOrientation(self.goal_post_left_id, [self.goal_position_init[0], self.goal_position_init[1] - self.goal_width / 2 + goal_y, self.goal_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.goal_post_right_id, [self.goal_position_init[0], self.goal_position_init[1] + self.goal_width / 2 + goal_y, self.goal_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_ball = self.get_distance_to_object(self.ball_id)
        new_ball_position = self.get_object_position(self.ball_id)
        survival = 1.0
        reach_ball = (self.distance_to_ball - new_distance_to_ball) / self.dt
        kick_ball = (new_ball_position[0] - self.ball_position[0]) / self.dt
        goal_y = self.goal_amplitude * np.sin(2 * np.pi * self.time / self.goal_period)
        ball_in_goal = 0.0
        if self.goal_position_init[0] - self.goal_post_radius < new_ball_position[0] < self.goal_position_init[0] + self.goal_post_radius and self.goal_position_init[1] - self.goal_width / 2 + goal_y < new_ball_position[1] < self.goal_position_init[1] + self.goal_width / 2 + goal_y:
            ball_in_goal = 10.0
        return {'survival': survival, 'reach_ball': reach_ball, 'kick_ball': kick_ball, 'ball_in_goal': ball_in_goal}

    def get_terminated(self, action):
        ball_position = self.get_object_position(self.ball_id)
        out_of_bounds = ball_position[0] < 0 or ball_position[0] > self.ground_size[0] or ball_position[1] < 0 or (ball_position[1] > self.ground_size[1])
        return out_of_bounds

    def get_success(self):
        ball_position = self.get_object_position(self.ball_id)
        goal_y = self.goal_amplitude * np.sin(2 * np.pi * self.time / self.goal_period)
        return self.goal_position_init[0] - self.goal_post_radius < ball_position[0] < self.goal_position_init[0] + self.goal_post_radius and self.goal_position_init[1] - self.goal_width / 2 + goal_y < ball_position[1] < self.goal_position_init[1] + self.goal_width / 2 + goal_y
\end{lstlisting}


==> env_codes/short_run/short_run_7.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Cross a bridge with moving segments and kick a ball into a goal.

    Description:
    - A start platform and an end platform (each 3 m in size and 0.5 m in thickness) are placed 25 m apart. 
    - The two platforms are connected by a bridge (2 m wide) divided into 6 segments of equal length (3 m each).
    - Each segment moves up and down independently with a sinusoidal motion. The amplitude is 1 m and the period is 2 seconds, with each segment offset in phase by 1/3 seconds from the previous one.
    - The segments have 1 m gaps between them.
    - A spherical ball (0.5 m diameter) is placed on the start platform, 1 m in front of the robot's initial position.
    - A goal area (3 m wide and indicated by two posts) is placed on the end platform.
    The robot is initialized on the start platform, facing the ball and bridge.
    The task is for the robot to kick or push the ball across the dynamic bridge segments, navigating the gaps, to get the ball into the goal area on the other side. The robot must also successfully cross the bridge and reach the end platform.

    Success:
    The task is successfully completed when the ball reaches the goal area on the end platform and the robot also reaches the end platform intact.

    Rewards:
    - Reward for decreasing distance between robot and ball, encouraging the robot to approach and interact with the ball.
    - Reward for increasing the forward progress of the ball across the bridge.
    - Large reward for getting the ball into the goal area.
    - Reward for robot staying on the bridge segments or platforms and avoiding falling.
    - Reward for robot reaching the end platform.

    Termination:
    The episode terminates if the robot or ball falls off the bridge or platforms. It also terminates if the ball goes off the sides of the bridge or platforms.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 25.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.bridge_length = self.platform_end_position[0] - self.platform_start_position[0] - self.platform_size[0]
        self.bridge_width = 2.0
        self.num_segments = 6
        self.segment_length = 3.0
        self.gap_length = 1.0
        self.segment_amplitude = 1.0
        self.segment_period = 2.0
        self.segment_phase_offset = 1.0 / 3.0
        self.segment_ids = []
        for i in range(self.num_segments):
            segment_id = self.create_box(mass=0.0, half_extents=[self.segment_length / 2, self.bridge_width / 2, self.platform_size[2] / 2], position=[self.platform_start_position[0] + self.platform_size[0] / 2 + self.segment_length / 2 + i * (self.segment_length + self.gap_length), self.platform_start_position[1], self.platform_start_position[2]], color=[0.5, 0.5, 0.5, 1.0])
            self._p.changeDynamics(bodyUniqueId=segment_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
            self.segment_ids.append(segment_id)
        self.ball_radius = 0.25
        self.ball_position_init = [self.platform_start_position[0] + 1.0, self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.ball_radius]
        self.ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=self.ball_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.goal_width = 3.0
        self.goal_position = [self.platform_end_position[0], self.platform_end_position[1], self.platform_end_position[2] + self.platform_size[2] / 2 + self.ball_radius]
        self.goal_left_post_id = self.create_cylinder(mass=0.0, radius=0.1, height=1.0, position=[self.goal_position[0], self.goal_position[1] - self.goal_width / 2, self.goal_position[2]], color=[0.0, 1.0, 0.0, 1.0])
        self.goal_right_post_id = self.create_cylinder(mass=0.0, radius=0.1, height=1.0, position=[self.goal_position[0], self.goal_position[1] + self.goal_width / 2, self.goal_position[2]], color=[0.0, 1.0, 0.0, 1.0])

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.ball_id, self.ball_position_init, [0.0, 0.0, 0.0, 1.0])
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_ball = self.get_distance_to_object(self.ball_id)
        self.ball_position = self.get_object_position(self.ball_id)
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        for i, segment_id in enumerate(self.segment_ids):
            segment_position = self.get_object_position(segment_id)
            new_segment_position = [segment_position[0], segment_position[1], self.platform_start_position[2] + self.segment_amplitude * np.sin(2 * np.pi * (self.time + i * self.segment_phase_offset) / self.segment_period)]
            self._p.resetBasePositionAndOrientation(segment_id, new_segment_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_ball = self.get_distance_to_object(self.ball_id)
        new_ball_position = self.get_object_position(self.ball_id)
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        approach_ball = (self.distance_to_ball - new_distance_to_ball) / self.dt
        ball_forward_velocity = (new_ball_position[0] - self.ball_position[0]) / self.dt
        ball_in_goal = 10.0 if self.goal_position[1] - self.goal_width / 2 < new_ball_position[1] < self.goal_position[1] + self.goal_width / 2 and new_ball_position[0] > self.goal_position[0] else 0.0
        on_bridge_or_platforms = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] + self.platform_size[2] / 2 else -1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        return {'approach_ball': approach_ball, 'ball_forward_velocity': ball_forward_velocity, 'ball_in_goal': ball_in_goal, 'on_bridge_or_platforms': on_bridge_or_platforms, 'reach_platform_end': reach_platform_end}

    def get_terminated(self, action):
        is_robot_on_bridge_or_platforms = self.robot.links['base'].position[2] > self.platform_start_position[2]
        is_ball_on_bridge_or_platforms = self.get_object_position(self.ball_id)[2] > self.platform_start_position[2]
        is_ball_off_sides = np.abs(self.get_object_position(self.ball_id)[1]) > self.bridge_width / 2 + self.platform_size[1] / 2
        return not is_robot_on_bridge_or_platforms or not is_ball_on_bridge_or_platforms or is_ball_off_sides

    def get_success(self):
        ball_position = self.get_object_position(self.ball_id)
        is_ball_in_goal = self.goal_position[1] - self.goal_width / 2 < ball_position[1] < self.goal_position[1] + self.goal_width / 2 and ball_position[0] > self.goal_position[0]
        is_robot_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_size[2] / 2
        return is_ball_in_goal and is_robot_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_8.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Navigate a dynamic obstacle course to reach a target.

    Description:
    - The environment consists of a large flat ground measuring 1000 x 1000 x 10 meters.
    - The robot starts at a fixed position on the ground, facing the positive x-axis.
    - The target is a cylindrical object (0.5 meters in diameter and 1 meter in height) placed 20 meters directly in front of the robot's starting position.
    - The obstacle course consists of 5 dynamic obstacles, each moving in a predictable pattern:
      - Obstacle 1: A box (1 x 1 x 1 meters) moving side-to-side (along the y-axis) with an amplitude of 2 meters and a period of 4 seconds. It is placed 5 meters in front of the robot's starting position.
      - Obstacle 2: A box (1 x 1 x 1 meters) moving up and down (along the z-axis) with an amplitude of 1 meter and a period of 3 seconds. It is placed 8 meters in front of the robot's starting position.
      - Obstacle 3: A box (1 x 1 x 1 meters) rotating around its center with a radius of 1 meter and a period of 5 seconds. It is placed 11 meters in front of the robot's starting position.
      - Obstacle 4: A box (1 x 1 x 1 meters) moving diagonally (along both x and y axes) with an amplitude of 1 meter and a period of 6 seconds. It is placed 14 meters in front of the robot's starting position.
      - Obstacle 5: A box (1 x 1 x 1 meters) moving in a circular pattern (along the x-y plane) with a radius of 1 meter and a period of 7 seconds. It is placed 17 meters in front of the robot's starting position.
    - The task of the robot is to navigate through the dynamic obstacle course and reach the target as quickly as possible.

    Success:
    The task is successfully completed when the robot reaches the target.

    Rewards:
    To help the robot complete the task:
    - The robot receives a reward for each time step it remains in the environment, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the target, incentivizing swift movement towards the goal.
    - The robot is penalized for colliding with any obstacles.

    Termination:
    The task terminates immediately if the robot collides with any obstacle or reaches the target.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [1000.0, 1000.0, 10.0]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.target_radius = 0.25
        self.target_height = 1.0
        self.target_position = [20.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.target_height / 2]
        self.target_id = self.create_cylinder(mass=0.0, radius=self.target_radius, height=self.target_height, position=self.target_position, color=[0.0, 1.0, 0.0, 1.0])
        self.obstacle_size = [1.0, 1.0, 1.0]
        self.obstacle_1_position_init = [5.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.obstacle_size[2] / 2]
        self.obstacle_2_position_init = [8.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.obstacle_size[2] / 2]
        self.obstacle_3_position_init = [11.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.obstacle_size[2] / 2]
        self.obstacle_4_position_init = [14.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.obstacle_size[2] / 2]
        self.obstacle_5_position_init = [17.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.obstacle_size[2] / 2]
        self.obstacle_1_id = self.create_box(mass=0.0, half_extents=[self.obstacle_size[0] / 2, self.obstacle_size[1] / 2, self.obstacle_size[2] / 2], position=self.obstacle_1_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.obstacle_2_id = self.create_box(mass=0.0, half_extents=[self.obstacle_size[0] / 2, self.obstacle_size[1] / 2, self.obstacle_size[2] / 2], position=self.obstacle_2_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.obstacle_3_id = self.create_box(mass=0.0, half_extents=[self.obstacle_size[0] / 2, self.obstacle_size[1] / 2, self.obstacle_size[2] / 2], position=self.obstacle_3_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.obstacle_4_id = self.create_box(mass=0.0, half_extents=[self.obstacle_size[0] / 2, self.obstacle_size[1] / 2, self.obstacle_size[2] / 2], position=self.obstacle_4_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.obstacle_5_id = self.create_box(mass=0.0, half_extents=[self.obstacle_size[0] / 2, self.obstacle_size[1] / 2, self.obstacle_size[2] / 2], position=self.obstacle_5_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.robot_position_init = [0.0, 0.0, self.ground_position[2] + self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]
        self.robot_orientation_init = self._p.getQuaternionFromEuler([0.0, 0.0, 0.0])

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot_orientation_init)
        return observation

    def step(self, action):
        self.distance_to_target = self.get_distance_to_object(self.target_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        obstacle_1_new_y = self.obstacle_1_position_init[1] + 2.0 * np.sin(2 * np.pi * self.time / 4.0)
        self._p.resetBasePositionAndOrientation(self.obstacle_1_id, [self.obstacle_1_position_init[0], obstacle_1_new_y, self.obstacle_1_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        obstacle_2_new_z = self.obstacle_2_position_init[2] + 1.0 * np.sin(2 * np.pi * self.time / 3.0)
        self._p.resetBasePositionAndOrientation(self.obstacle_2_id, [self.obstacle_2_position_init[0], self.obstacle_2_position_init[1], obstacle_2_new_z], [0.0, 0.0, 0.0, 1.0])
        obstacle_3_new_x = self.obstacle_3_position_init[0] + 1.0 * np.cos(2 * np.pi * self.time / 5.0)
        obstacle_3_new_y = self.obstacle_3_position_init[1] + 1.0 * np.sin(2 * np.pi * self.time / 5.0)
        self._p.resetBasePositionAndOrientation(self.obstacle_3_id, [obstacle_3_new_x, obstacle_3_new_y, self.obstacle_3_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        obstacle_4_new_x = self.obstacle_4_position_init[0] + 1.0 * np.cos(2 * np.pi * self.time / 6.0)
        obstacle_4_new_y = self.obstacle_4_position_init[1] + 1.0 * np.sin(2 * np.pi * self.time / 6.0)
        self._p.resetBasePositionAndOrientation(self.obstacle_4_id, [obstacle_4_new_x, obstacle_4_new_y, self.obstacle_4_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        obstacle_5_new_x = self.obstacle_5_position_init[0] + 1.0 * np.cos(2 * np.pi * self.time / 7.0)
        obstacle_5_new_y = self.obstacle_5_position_init[1] + 1.0 * np.sin(2 * np.pi * self.time / 7.0)
        self._p.resetBasePositionAndOrientation(self.obstacle_5_id, [obstacle_5_new_x, obstacle_5_new_y, self.obstacle_5_position_init[2]], [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_target = self.get_distance_to_object(self.target_id)
        survival = 1.0
        reach_target = (self.distance_to_target - new_distance_to_target) / self.dt
        return {'survival': survival, 'reach_target': reach_target}

    def get_terminated(self, action):
        collision_obstacle_1 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_1_id)) > 0
        collision_obstacle_2 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_2_id)) > 0
        collision_obstacle_3 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_3_id)) > 0
        collision_obstacle_4 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_4_id)) > 0
        collision_obstacle_5 = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.obstacle_5_id)) > 0
        collision_target = len(self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.target_id)) > 0
        return collision_obstacle_1 or collision_obstacle_2 or collision_obstacle_3 or collision_obstacle_4 or collision_obstacle_5 or collision_target

    def get_success(self):
        contact_points_target = self._p.getContactPoints(bodyA=self.robot.robot_id, bodyB=self.target_id)
        return len(contact_points_target) > 0
\end{lstlisting}


==> env_codes/short_run/short_run_9.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Push a box to a target location on a dynamic platform.

    Description:
    - The environment consists of a start platform and an end platform (each 3 m in size and 0.5 m in thickness) placed 20 m apart.
    - The two platforms are connected by a dynamic bridge (2 m wide) divided into 5 segments of equal length (3 m each).
    - Each segment moves up and down independently with a sinusoidal motion. The amplitude is 1 m and the period is 2 seconds, with each segment offset in phase by 0.4 seconds from the previous one.
    - A box (0.5 m in size) is placed on the start platform, 1 m in front of the robot's initial position.
    - The robot is initialized on the start platform, facing the box and bridge.
    - The task of the robot is to push the box across the dynamic bridge segments to reach a target location on the end platform.

    Success:
    The task is successfully completed when the box reaches the target location on the end platform.

    Rewards:
    - Reward for decreasing the distance between the robot and the box, encouraging the robot to approach and interact with the box.
    - Reward for increasing the forward progress of the box across the bridge.
    - Large reward for getting the box to the target location on the end platform.
    - Reward for the robot staying on the bridge segments or platforms and avoiding falling.
    - Reward for the robot reaching the end platform.

    Termination:
    The episode terminates if the robot or box falls off the bridge or platforms.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 20.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.bridge_length = self.platform_end_position[0] - self.platform_start_position[0] - self.platform_size[0]
        self.bridge_width = 2.0
        self.num_segments = 5
        self.segment_length = self.bridge_length / self.num_segments
        self.segment_amplitude = 1.0
        self.segment_period = 2.0
        self.segment_phase_offset = 0.4
        segment_colors = [[1.0, 0.0, 0.0, 1.0], [1.0, 0.5, 0.0, 1.0], [1.0, 1.0, 0.0, 1.0], [0.0, 1.0, 0.0, 1.0], [0.0, 0.0, 1.0, 1.0]]
        self.segment_ids = []
        for i in range(self.num_segments):
            segment_id = self.create_box(mass=0.0, half_extents=[self.segment_length / 2, self.bridge_width / 2, self.platform_size[2] / 2], position=[self.platform_start_position[0] + self.platform_size[0] / 2 + self.segment_length / 2 + i * self.segment_length, self.platform_start_position[1], self.platform_start_position[2]], color=segment_colors[i])
            self._p.changeDynamics(bodyUniqueId=segment_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
            self.segment_ids.append(segment_id)
        self.box_size = [0.5, 0.5, 0.5]
        self.box_position_init = [self.platform_start_position[0] + 1.0, self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.box_size[2] / 2]
        self.box_id = self.create_box(mass=1.0, half_extents=[self.box_size[0] / 2, self.box_size[1] / 2, self.box_size[2] / 2], position=self.box_position_init, color=[1.0, 0.0, 0.0, 1.0])
        self.target_position = [self.platform_end_position[0], self.platform_end_position[1], self.platform_end_position[2] + self.platform_size[2] / 2 + self.box_size[2] / 2]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self.time = 0.0
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        self._p.resetBasePositionAndOrientation(self.box_id, self.box_position_init, [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_box = self.get_distance_to_object(self.box_id)
        self.box_position = self.get_object_position(self.box_id)
        observation, reward, terminated, truncated, info = super().step(action)
        self.time += self.dt
        for i, segment_id in enumerate(self.segment_ids):
            segment_position = self.get_object_position(segment_id)
            new_segment_position = [segment_position[0], segment_position[1], self.platform_start_position[2] + self.segment_amplitude * np.sin(2 * np.pi * (self.time + i * self.segment_phase_offset) / self.segment_period)]
            self._p.resetBasePositionAndOrientation(segment_id, new_segment_position, [0.0, 0.0, 0.0, 1.0])
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_box = self.get_distance_to_object(self.box_id)
        new_box_position = self.get_object_position(self.box_id)
        approach_box = (self.distance_to_box - new_distance_to_box) / self.dt
        forward_progress_box = (new_box_position[0] - self.box_position[0]) / self.dt
        on_bridge_or_platforms = 1.0 if self.robot.links['base'].position[2] > self.platform_start_position[2] + self.platform_size[2] / 2 else -1.0
        reach_end_platform = 1.0 if self.robot.links['base'].position[0] >= self.platform_end_position[0] else 0.0
        reach_target_location = 10.0 if np.linalg.norm(new_box_position[:2] - self.target_position[:2]) < self.box_size[0] / 2 else 0.0
        return {'approach_box': approach_box, 'forward_progress_box': forward_progress_box, 'on_bridge_or_platforms': on_bridge_or_platforms, 'reach_end_platform': reach_end_platform, 'reach_target_location': reach_target_location}

    def get_terminated(self, action):
        robot_fell = self.robot.links['base'].position[2] < self.platform_start_position[2]
        box_fell = self.get_object_position(self.box_id)[2] < self.platform_start_position[2]
        return robot_fell or box_fell

    def get_success(self):
        box_position = self.get_object_position(self.box_id)
        return np.linalg.norm(box_position[:2] - self.target_position[:2]) < self.box_size[0] / 2
\end{lstlisting}


==> env_codes/short_run/short_run_s1.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Cross a pride-colored bridge with gaps to reach a platform.

    Description:
    - A start platform and an end platform (each 3 m in size and 0.5 m in thickness) are placed 50 m apart.
    - The two platforms are connected by a bridge (2 m wide) divided in multiple segments. Each segment has a different color corresponding to the pride colors.
    - The segments are separated by gaps measuring 2 m.
    The robot is initialized on the start platform.
    The task of the robot is to cross the bridge to reach the end platform as fast as possible.

    Success:
    The task is successfully completed when the robot reaches the end platform.

    Rewards:
    To help the robot complete the task:
    - The robot receives a reward for each time step it remains standing on the bridge or platforms, encouraging steady progress.
    - The robot is rewarded based on how much it reduces the distance to the end platform, incentivizing swift movement towards the goal.

    Termination:
    The task terminates immediately if the robot falls off the start platform, any segment of the bridge, or the end platform.
    """

    def __init__(self):
        super().__init__()
        self.platform_size = [3.0, 3.0, 0.5]
        self.platform_start_position = [0.0, 0.0, 0.0]
        self.platform_end_position = [self.platform_start_position[0] + 50.0, self.platform_start_position[1], self.platform_start_position[2]]
        self.platform_start_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_start_position, color=[0.8, 0.8, 0.8, 1.0])
        self.platform_end_id = self.create_box(mass=0.0, half_extents=[self.platform_size[0] / 2, self.platform_size[1] / 2, self.platform_size[2] / 2], position=self.platform_end_position, color=[0.8, 0.8, 0.8, 1.0])
        self.bridge_length = self.platform_end_position[0] - self.platform_start_position[0] - self.platform_size[0]
        self.bridge_width = 2.0
        self.gap_length = 2.0
        pride_colors = [[1.0, 0.0, 0.0, 1.0], [1.0, 0.5, 0.0, 1.0], [1.0, 1.0, 0.0, 1.0], [0.0, 0.5, 0.0, 1.0], [0.0, 0.0, 1.0, 1.0], [0.7, 0.0, 1.0, 1.0]]
        num_colors = len(pride_colors)
        segment_size = (self.bridge_length - (num_colors - 1) * self.gap_length) / num_colors
        for i, color in enumerate(pride_colors):
            segment_id = self.create_box(mass=0.0, half_extents=[segment_size / 2, self.bridge_width / 2, self.platform_size[2] / 2], position=[self.platform_start_position[0] + self.platform_size[0] / 2 + segment_size / 2 + i * (segment_size + self.gap_length), self.platform_start_position[1], self.platform_start_position[2]], color=color)
            self._p.changeDynamics(bodyUniqueId=segment_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.platform_start_position[0], self.platform_start_position[1], self.platform_start_position[2] + self.platform_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_platform_end = self.get_distance_to_object(self.platform_end_id)
        survival = 1.0
        reach_platform_end = (self.distance_to_platform_end - new_distance_to_platform_end) / self.dt
        return {'survival': survival, 'reach_platform_end': reach_platform_end}

    def get_terminated(self, action):
        return self.robot.links['base'].position[2] < self.platform_start_position[2]

    def get_success(self):
        is_on_platform_end = self.get_distance_to_object(self.platform_end_id) < self.platform_size[2] / 2
        return is_on_platform_end
\end{lstlisting}


==> env_codes/short_run/short_run_s2.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Ascend a series of stairs to reach a platform.

    Description:
    - The environment consists of a ground platform (1000 m x 10 m x 10 m) and a set of 10 steps.
    - Each step has dimensions of 1 m in length, 10 m in width, and 0.2 m in height.
    - The steps are positioned to form an ascending staircase, with each subsequent step higher than the previous one.
    The robot is initialized on the ground at the bottom of the stairs.

    Success:
    The task is completed when the robot successfully ascends the stairs and reaches the top platform.

    Rewards:
    To help the robot complete the task:
    - The robot is rewarded for survival at each time step.
    - The robot is rewarded for forward velocity, incentivizing it to move up the stairs.

    Termination:
    The task terminates immediately if the robot falls off the stairs or the top platform.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [1000.0, 10.0, 10.0]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.num_steps = 10
        self.step_size = [1.0, 10.0, 0.2]
        self.step_position_init = [self.ground_position[0], self.ground_position[1], self.ground_position[2] + self.ground_size[2] / 2]
        self.create_stairs_up(step_size=self.step_size, step_position_init=self.step_position_init, num_steps=self.num_steps)

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_stairs_up(self, step_size, step_position_init, num_steps):
        color_1 = np.array([1.0, 0.0, 0.0])
        color_2 = np.array([0.0, 0.0, 1.0])
        for i in range(num_steps):
            step_position = [step_position_init[0] + i * step_size[0], step_position_init[1], step_position_init[2] + i * step_size[2]]
            interpolation = i / (num_steps - 1)
            step_color = (1 - interpolation) * color_1 + interpolation * color_2
            self.create_box(mass=0.0, half_extents=[step_size[0] / 2, step_size[1] / 2, step_size[2] / 2], position=step_position, color=np.append(step_color, 1.0))

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, [self.ground_position[0], self.ground_position[1], self.ground_position[2] + self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]], self.robot.links['base'].orientation_init)
        return observation

    def step(self, action):
        self.position = self.robot.links['base'].position
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_position = self.robot.links['base'].position
        survival = 1.0
        forward_velocity = (new_position[0] - self.position[0]) / self.dt
        return {'survival': survival, 'forward_velocity': forward_velocity}

    def get_terminated(self, action):
        return self.robot.links['base'].position[2] < self.ground_position[2]

    def get_success(self):
        return self.robot.links['base'].position[0] > self.step_position_init[0] + (self.num_steps - 1) * self.step_size[0]
\end{lstlisting}


==> env_codes/short_run/short_run_s3.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
from oped.envs.r2d2.base import R2D2Env

class Env(R2D2Env):
    """
    Kick a ball into a goal.

    Description:
    - The environment consists of a large flat ground measuring 1000 x 1000 x 10 meters.
    - A ball with a radius of 0.5 meters is placed randomly on the ground.
    - The goal is defined by two goal posts, each 2 meters high and placed 3 meters apart, forming a goal area.
    - The robot is initialized at a fixed position on the ground.
    - The task of the robot is to move across the ground, reach the ball, and kick it into the goal.

    Success:
    The task is successfully completed if the robot kicks the ball so that it passes between the two goal posts.

    Rewards:
    To help the robot complete the task:
    - The robot is rewarded for survival at each time step.
    - The robot is rewarded for decreasing its distance to the ball.
    - The robot is rewarded for kicking the ball towards the goal, with additional rewards for successfully kicking the ball into the goal.

    Termination:
    The task does not have a specific termination condition.
    """

    def __init__(self):
        super().__init__()
        self.ground_size = [1000.0, 1000.0, 10.0]
        self.ground_position = [0.0, 0.0, 0.0]
        self.ground_id = self.create_box(mass=0.0, half_extents=[self.ground_size[0] / 2, self.ground_size[1] / 2, self.ground_size[2] / 2], position=self.ground_position, color=[0.5, 0.5, 0.5, 1.0])
        self._p.changeDynamics(bodyUniqueId=self.ground_id, linkIndex=-1, lateralFriction=0.8, restitution=0.5)
        self.ball_radius = 0.5
        self.ball_id = self.create_sphere(mass=1.0, radius=self.ball_radius, position=[0.0, 0.0, 0.0], color=[1.0, 0.0, 0.0, 1.0])
        self.goal_post_height = 2.0
        self.goal_post_radius = 0.1
        self.goal_width = 3.0
        self.goal_position = [self.ground_position[0] + 10.0, self.ground_position[1], self.ground_position[2] + self.ground_size[2] / 2 + self.goal_post_height / 2]
        self.goal_post_left_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_position[0], self.goal_position[1] - self.goal_width / 2, self.goal_position[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.goal_post_right_id = self.create_cylinder(mass=0.0, radius=self.goal_post_radius, height=self.goal_post_height, position=[self.goal_position[0], self.goal_position[1] + self.goal_width / 2, self.goal_position[2]], color=[1.0, 1.0, 1.0, 1.0])
        self.robot_position_init = [self.ground_position[0], self.ground_position[1], self.ground_position[2] + self.ground_size[2] / 2 + self.robot.links['base'].position_init[2]]

    def create_box(self, mass, half_extents, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_BOX, halfExtents=half_extents, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_sphere(self, mass, radius, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_SPHERE, radius=radius)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_SPHERE, radius=radius, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def create_cylinder(self, mass, radius, height, position, color):
        collision_shape_id = self._p.createCollisionShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, height=height)
        visual_shape_id = self._p.createVisualShape(shapeType=self._p.GEOM_CYLINDER, radius=radius, length=height, rgbaColor=color)
        return self._p.createMultiBody(baseMass=mass, baseCollisionShapeIndex=collision_shape_id, baseVisualShapeIndex=visual_shape_id, basePosition=position)

    def get_object_position(self, object_id):
        return np.asarray(self._p.getBasePositionAndOrientation(object_id)[0])

    def get_distance_to_object(self, object_id):
        object_position = self.get_object_position(object_id)
        robot_position = self.robot.links['base'].position
        return np.linalg.norm(object_position[:2] - robot_position[:2])

    def reset(self):
        observation = super().reset()
        self._p.resetBasePositionAndOrientation(self.robot.robot_id, self.robot_position_init, self.robot.links['base'].orientation_init)
        ball_y_init = np.random.uniform(self.robot_position_init[1] - 2.0, self.robot_position_init[1] + 2.0)
        self._p.resetBasePositionAndOrientation(self.ball_id, [self.robot_position_init[0] + 5.0, ball_y_init, self.ground_position[2] + self.ground_size[2] / 2 + self.ball_radius], [0.0, 0.0, 0.0, 1.0])
        return observation

    def step(self, action):
        self.distance_to_ball = self.get_distance_to_object(self.ball_id)
        self.ball_position = self.get_object_position(self.ball_id)
        observation, reward, terminated, truncated, info = super().step(action)
        return (observation, reward, terminated, truncated, info)

    def get_task_rewards(self, action):
        new_distance_to_ball = self.get_distance_to_object(self.ball_id)
        new_ball_position = self.get_object_position(self.ball_id)
        survival = 1.0
        reach_ball = (self.distance_to_ball - new_distance_to_ball) / self.dt
        kick_ball = (new_ball_position[0] - self.ball_position[0]) / self.dt
        ball_in_goal = 0.0
        if self.goal_position[1] - self.goal_width / 2 < new_ball_position[1] < self.goal_position[1] + self.goal_width / 2 and new_ball_position[0] > self.goal_position[0]:
            ball_in_goal = 10.0
        return {'survival': survival, 'reach_ball': reach_ball, 'kick_ball': kick_ball, 'ball_in_goal': ball_in_goal}

    def get_terminated(self, action):
        return False

    def get_success(self):
        ball_position = self.get_object_position(self.ball_id)
        return self.goal_position[1] - self.goal_width / 2 < ball_position[1] < self.goal_position[1] + self.goal_width / 2 and ball_position[0] > self.goal_position[0]
\end{lstlisting}


==> task_descs/long_run/long_run_103.tex <==
\begin{lstlisting}[language={}]
Conveyor Belt Item Delivery

Description:
- The environment consists of two 5 m x 5 m platforms connected by a 5 m long conveyor belt. The conveyor belt moves from left to right at a speed of 0.5 m/s.
- On the right platform, there are three target areas marked by 1 m x 1 m colored squares (red, green, blue). 
- Also on the right platform, there is a dispenser that releases items onto the conveyor belt at random intervals between 2-5 seconds. The items are 0.5 m cubes colored either red, green, or blue.
- The robot begins on the left platform. 

Task:
The robot must jump onto the conveyor belt, pick up the colored items, ride the conveyor to the right platform, and deliver each item to the target area matching its color. The robot should try to deliver as many items as possible to the correct targets within the time limit.

After delivering an item, the robot must jump back onto the conveyor belt and return to the left platform before the next item is released. The robot should wait on the left platform for the next item.

Rewards:
- Provide a small reward for picking up an item from the conveyor belt.
- Provide a large reward for delivering an item to the correct target area based on color.
- Provide a small penalty for delivering an item to the wrong target area.
- Provide a moderate penalty if the robot falls off the conveyor belt or platforms.

Success Conditions:
The task is considered complete if the robot successfully delivers at least 5 items to their correct target areas within the time limit.

Time Limit:
The robot has 3 minutes to deliver as many items as possible.

Termination:
The episode ends if the robot falls off the platforms or conveyor belt, or if the time limit is reached.
\end{lstlisting}


==> task_descs/long_run/long_run_122.tex <==
\begin{lstlisting}[language={}]
Kick ball through moving gates to zones marked by moving targets.

The environment consists of a large flat ground. A ball is placed 5 meters directly in front of the robot. After a delay of 1-2 seconds (randomized), the ball begins rolling straight ahead at a constant velocity of 1-2 m/s (randomized).

Five vertical rectangular gates, each 3 meters tall and 1 meter wide, are placed at randomized positions between 5 to 25 meters in front of the ball's initial position, at randomized lateral offsets up to 5 meters on either side. The gates translate laterally with randomized constant velocities between 0.2-1 m/s, reversing direction each time they move 5 meters from their initial position. The gates' movement is triggered at the start of the episode.

Five target zones are marked on the ground at randomized positions between 10 to 30 meters in front of the ball's initial position, at randomized lateral offsets up to 10 meters on either side. Each target zone is a circle with radius 2 meters. At the center of each target zone is a flat cylindrical marker, 2 meters in radius and 0.1 meters tall. The markers rotate in place with randomized constant angular velocities between 0.1-0.5 rad/s, switching between clockwise and counterclockwise rotation each time the ball passes through a gate. The markers' rotation is triggered at the start of the episode.

The robot is initialized 3 meters behind the ball, facing the direction of the ball's initial velocity.

The task is for the robot to kick the ball through each gate in order, aiming to get the ball to stop within the corresponding target zone after it passes through the gate. The robot should decide when and how to kick the ball based on the observed motion of the gates and markers.

Passing through a gate awards 2 points if the ball subsequently stops in the correct target zone, and 1 point otherwise. The episode ends when the ball passes through all gates, or a maximum time limit is reached. The robot should aim to maximize its total score.
\end{lstlisting}


==> task_descs/long_run/long_run_155.tex <==
\begin{lstlisting}[language={}]
Task: Dynamic Target Pushing Challenge

Description:
- The environment is a 15 m x 15 m open area with a flat surface.
- There are 3 dynamic targets (spheres with a 0.5 m diameter) that move along predefined linear paths. Each target moves back and forth along a 5 m path at a speed of 0.5 m/s.
- The robot starts at the center of the area.
- Three goal zones (1 m x 1 m squares) are located at the edges of the area: one at the north edge, one at the east edge, and one at the west edge.

Task:
The robot must push each moving target into its corresponding goal zone. The targets can be pushed in any order, but each target must come to rest fully within its goal zone to be considered successfully delivered.

Initial Positions:
- Robot: Center of the area at (0, 0, 0.5)
- Target 1: Moving along the path from (-2.5, 5, 0.25) to (2.5, 5, 0.25)
- Target 2: Moving along the path from (5, -2.5, 0.25) to (5, 2.5, 0.25)
- Target 3: Moving along the path from (-5, -2.5, 0.25) to (-5, 2.5, 0.25)
- Goal Zone 1: Centered at (0, 7, 0.05)
- Goal Zone 2: Centered at (7, 0, 0.05)
- Goal Zone 3: Centered at (-7, 0, 0.05)

Success Conditions:
The task is considered complete when all three targets come to rest fully within their respective goal zones.

Time Limit:
The robot has a time limit of 5 minutes to complete the task.

Rewards:
- Provide a small reward for moving closer to a target.
- Provide a moderate reward for reaching a target.
- Provide a large reward for pushing a target towards its goal zone.
- Provide a significant reward for delivering a target to its goal zone.
- Apply a small penalty for collisions with the targets or the boundaries of the area.

Termination:
The episode terminates if the robot flips over, if a target is pushed out of bounds, or if the time limit is exceeded. The episode should terminate with success if all targets are delivered to their goal zones.
\end{lstlisting}


==> task_descs/long_run/long_run_176.tex <==
\begin{lstlisting}[language={}]
Task: Push two balls into separate goals while avoiding static obstacles.

Description:
- The environment consists of a large flat ground.
- Two balls, one red and one blue, are placed at fixed initial positions on the ground. The red ball is positioned at [2.0, -2.0, 0.5] and the blue ball is positioned at [2.0, 2.0, 0.5].
- Two goal areas are defined by pairs of posts. The red goal is defined by posts placed at [10.0, -2.0, 1.0] and [10.0, -1.0, 1.0]. The blue goal is defined by posts placed at [10.0, 1.0, 1.0] and [10.0, 2.0, 1.0].
- Three cylindrical obstacles of 1 meter radius and 2 meters height are placed at fixed positions: [5.0, 0.0, 1.0], [7.0, -1.0, 1.0], and [7.0, 1.0, 1.0].
- The robot is initialized at [0.0, 0.0, 0.5], facing the positive x-direction.
- The task is for the robot to push the red ball into the red goal and the blue ball into the blue goal while avoiding the obstacles.

Success:
The task is completed successfully if the robot pushes both balls into their respective goals without colliding with any obstacles.

Rewards:
- The robot is rewarded for decreasing its distance to each ball.
- The robot is rewarded for pushing each ball towards its respective goal.
- The robot is penalized for colliding with obstacles.
- The robot is greatly rewarded if a ball passes between the goal posts of its respective goal.

Termination:
The task is terminated if the robot collides with an obstacle, if a ball collides with an obstacle, or if a time limit of 60 seconds is reached.
\end{lstlisting}


==> task_descs/long_run/long_run_178.tex <==
\begin{lstlisting}[language={}]
Task: Coordinate with another moving ball to hit a target

Description:
- The environment consists of a large flat ground.
- Two balls are placed 5 meters in front of the robot, spaced 2 meters apart laterally. Both balls begin rolling in parallel at 1 m/s after a short delay of 1 second.
- A target area defined by a 2x2 meter flat vertical target is placed 10 meters from the balls' initial position. The target moves laterally back and forth at 0.5 m/s, covering 3 meters to each side before reversing direction.
- The robot is initialized 3 meters behind the balls, facing the direction of the target.
- The task is for the robot to coordinate its movements to kick both balls such that they hit the moving target simultaneously.

Success:
The task is completed successfully if both balls hit the front face of the moving target simultaneously.

Rewards:
- The robot is rewarded for decreasing the distance to each ball as they move.
- The robot is rewarded for matching the velocity of each ball as it approaches.
- The robot is rewarded for kicking each ball with a velocity that is likely to reach the target.
- The robot is greatly rewarded if both balls hit the front face of the moving target simultaneously.

Termination:
The task is terminated if either ball stops moving, if the balls do not hit the target simultaneously, or if a time limit of 30 seconds is reached.
\end{lstlisting}


==> task_descs/long_run/long_run_196.tex <==
\begin{lstlisting}[language={}]
Task: Dodgeball Arena

Description:
- The environment is a 15 m x 15 m walled arena with a flat ground surface.
- There are 5 automatic ball launchers positioned around the perimeter of the arena. Each launcher can shoot a foam ball (0.2 m diameter) at varying speeds (up to 5 m/s) and angles.
- The launchers are programmed to shoot balls at random intervals (between 1 to 3 seconds) and in random directions.
- The robot starts in the center of the arena.

Task:
The robot must avoid being hit by the foam balls for as long as possible. The robot can move around the arena and jump to dodge the balls.

Success Conditions:
The task is considered successful if the robot can avoid being hit by any balls for a duration of 2 minutes.

Rewards:
- Provide a small reward for each second the robot avoids being hit.
- Provide a large reward for successfully avoiding all balls for the entire duration.
- Apply a small penalty for each ball that hits the robot.

Termination:
The episode ends if the robot is hit by a ball, or if the time limit of 2 minutes is exceeded.
\end{lstlisting}


==> task_descs/long_run/long_run_197.tex <==
\begin{lstlisting}[language={}]
Task: Jumping Over Gaps

Description:
- The environment consists of a 10 m x 10 m platform with a series of gaps that the robot must jump over.
- The platform is divided into three sections:
  1. The first section (3 m x 10 m) has three gaps, each 0.5 m wide, spaced 2 m apart.
  2. The second section (3 m x 10 m) has two gaps, each 1 m wide, spaced 3 m apart.
  3. The third section (4 m x 10 m) has one gap, 1.5 m wide, located 2 m from the end of the platform.

- The robot begins at the start of the platform, facing the positive x-axis.

Task:
The robot must navigate through the three sections of the platform, jumping over the gaps to reach the end of the platform.

Success Conditions:
The task is considered complete when the robot reaches the end of the platform without falling into any gaps.

Rewards:
- Provide a small reward for each gap successfully jumped over.
- Provide a large reward for reaching the end of the platform.
- Apply a small penalty for each failed jump (falling into a gap).

Termination:
The episode ends if the robot falls into a gap, flips over, or reaches the end of the platform.
\end{lstlisting}


==> task_descs/long_run/long_run_23.tex <==
\begin{lstlisting}[language={}]
Search and Rescue in a Multi-Room Environment

Description: 
- The environment consists of a large, two-story building with multiple rooms connected by doors, hallways, and staircases. The layout is fixed but contains challenging features:
  - 8 rooms total (4 on each floor), connected by 2 hallways (one per floor)
  - Each room is 5 m x 5 m. Hallways are 20 m long and 2 m wide. Staircase is 5 m long.
  - Rooms contain various static and movable obstacles like furniture.
  - Doors are 1 m wide and initially closed. Robot must push them open.
- A target object (a 0.5 m x 0.5 m x 1 m box) representing a person is located in one of the rooms on the second floor. Its location is fixed for now.
- The robot starts at the entrance of the building on the first floor.
- The robot must systematically explore the building, locate the target object, attach a virtual tether to it, and guide it back to the entrance while avoiding obstacles.

Success Conditions:
The task is considered complete when the robot brings the target object to rest within 2 m of the entrance location. 

Time Limit:
The robot has a time limit of 10 minutes to complete the task.

Rewards:
- Provide a small reward for exploring new areas of the environment.
- Provide a moderate reward for locating the target object.
- Provide a large reward for successfully bringing the target object to the goal location.
- Provide a small penalty for collisions with obstacles to encourage careful navigation.

Termination:
The episode terminates if the robot flips over or if the time limit is exceeded.
\end{lstlisting}


==> task_descs/long_run/long_run_60.tex <==
\begin{lstlisting}[language={}]
Simplified 1-vs-1 robot soccer.

Description:
- The environment consists of a large flat ground representing a soccer field.
- Two goals are placed on opposite ends of the field, each defined by two posts 2 meters high and 3 meters apart.  
- The robot is placed on one side of the field, facing the opponent's goal.
- A basic opponent robot is placed on the other side, initially stationary.
- A soccer ball is placed in the center of the field.
- The objective is for the robot to navigate to the ball, take possession of it, and kick it into the opponent's goal while defending its own goal.
- In the first stage, the opponent robot remains stationary. In the second stage, the opponent robot also moves to chase after the ball and attempt to kick it into the robot's goal.

Success:
The task is completed successfully if the robot is able to kick the ball into the opponent's goal while preventing the opponent from scoring.

Rewards:
- The robot is rewarded for possessing the ball, defined as being within 1 meter of the ball while the opponent is not.
- The robot is rewarded for bringing the ball closer to the opponent's goal.
- The robot is rewarded for kicking the ball with a velocity toward the opponent's goal.
- The robot is penalized if the opponent takes possession of the ball or if the ball goes out of bounds.
- The robot is greatly rewarded for scoring a goal and penalized if the opponent scores.

Termination:
The task is terminated if a goal is scored by either side, if the ball goes out of bounds, or if a time limit is reached.
\end{lstlisting}


==> task_descs/long_run/long_run_74.tex <==
\begin{lstlisting}[language={}]
Receive pass and kick ball past moving obstacles and goalie into goal.

The robot is placed on a large flat ground designed to look like a soccer/football pitch with markings. 

A teammate robot is positioned 5 meters to the side of the main robot. After a fixed delay at the start of the episode, the teammate robot passes a ball towards a point 3 meters in front of the main robot at a speed of 3 m/s. The pass target point is fixed, but the main robot's initial position has some randomness, so it will need to adjust to align itself with the passed ball.

3 cylindrical obstacles of 0.5 meter radius and 1 meter height are placed at random positions 3 to 8 meters in front of the robot's initial position. The obstacles are colored to resemble soccer players and move randomly back and forth over a 2 meter range at speeds between 0.5 and 1.5 m/s. The obstacles do not actively chase the ball but will block it if it comes near them.

A goal area 5 meters wide and 2 meters deep is placed 10 meters in front of the robot's initial position, centered along the front line. 

A goalie obstacle 1 meter wide, 0.5 meters deep, and 1.5 meters tall moves side to side across the goal line at a speed of 1.5 m/s, tracking the ball when it is within 3 meters. The goalie is colored differently than the field obstacles.

The task is for the main robot to receive the teammate's pass and then kick the moving ball past the field obstacles and goalie to score a goal, without touching any of the obstacles.
\end{lstlisting}


==> task_descs/long_run/long_run_76.tex <==
\begin{lstlisting}[language={}]
Construction Site Cleanup

Description: 
- The environment is a construction site with dimensions 10 m x 10 m.
- There are 3 piles of different types of debris scattered around the construction site:
  - 5 bricks (each 0.2 m x 0.2 m x 0.2 m)
  - 5 metal scraps (each 0.5 m x 0.25 m x 0.25 m) 
  - 5 wooden planks (each 1 m x 0.2 m x 0.1 m)
- There are also 2 robotic construction vehicles moving around the site in pre-programmed patterns:
  - A bulldozer that pushes dirt piles around in a rectangle, 4 m x 3 m
  - An excavator that swings its arm and bucket back and forth in a 180 degree arc, 2 m in radius
- On one side of the construction site are 3 square receptacle bins, each 1 m x 1 m x 0.5 m tall, labeled for each type of debris (bricks, metal, wood).
- The robot starts in one corner of the site.

Task:
The robot needs to pick up each piece of debris and place it in the correct receptacle, while avoiding collisions with the moving construction vehicles. The robot can only carry one piece of debris at a time.

Success Conditions:
The task is complete when all pieces of debris have been placed in their correct bins, and the robot has returned to its starting position.

Time Limit:
The robot has 10 minutes to complete the cleanup task.

Rewards:
- Provide a small reward for each piece of debris successfully picked up.
- Provide a moderate reward for each piece of debris placed in the correct bin.
- Provide a large reward for completing the task and returning to the start position.
- Provide a small penalty for each collision with the construction vehicles.

Termination:
The episode ends if the robot flips over, or if the time limit is exceeded.
\end{lstlisting}


==> task_descs/long_run/long_run_84.tex <==
\begin{lstlisting}[language={}]
Busy Restaurant Table Service

Description: 
- The environment is a busy restaurant dining area, consisting of a 12 m x 12 m room with 4 tables, an entrance door, and a kitchen door.
- Restaurant patrons (simulated as cylinders) continuously enter from the entrance, move to a table, stay for a period of time, and then exit, making the environment dynamic.
- The robot must perform two types of table service tasks:
  1) Table setting: The robot must collect clean dishes and utensils from the kitchen and arrange them properly on the tables in preparation for new patrons. Dishes should be stacked neatly.
  2) Table busing: After patrons leave, the robot must clear dirty dishes and utensils from the tables, load them into a bin, and return the bin to the kitchen. The bin has a maximum capacity that the robot must respect.
- The robot must avoid colliding with patrons and restaurant furniture as it navigates.
- Dishes will break if dropped. The robot must handle them carefully.

Success Conditions:
- For table setting, success means all necessary dishes and utensils are properly placed on empty tables prior to new patrons arriving. Dishes should be undamaged and neatly stacked.
- For table busing, success involves clearing all dirty dishes from unoccupied tables, loading them into the bin without exceeding capacity, and delivering the bin to the kitchen. No dishes should be broken.
- The robot should avoid any collisions with patrons or furniture throughout the episode.

Time Limit:
The episode lasts for 10 minutes of simulated time. The robot must continuously perform both table setting and busing tasks during this period as needed.

Rewards:
- Provide a moderate reward for each successful table set, with all dishes placed neatly and undamaged.
- Provide a moderate reward for each successful table busing, with no broken dishes and the bin delivered to the kitchen.
- Give a small reward for carefully handling dishes without breaking them.
- Assign a substantial penalty for any collisions between the robot and patrons or furniture.
- Assign a small penalty for dropping and breaking a dish.
- Provide a small reward at each timestep for maintaining a tidy dining room, with no dirty dishes left on unoccupied tables.

Termination:
The episode ends if the robot crashes into a patron or furniture, or if the time limit is reached. The episode is considered successful if the robot consistently performs both table setting and busing throughout the full time period with no collisions or broken dishes.
\end{lstlisting}


==> task_descs/long_run/long_run_88.tex <==
\begin{lstlisting}[language={}]
Bounce Shot Scoring Challenge

Description:
- The environment consists of a walled field measuring 20 m x 10 m. The field contains 3 ramps/mounds (triangular prisms) placed randomly, each measuring 2 m long x 1 m wide x 0.5 m high.  
- A single goal 3 m wide and 1 m high is placed centered on one end of the field.
- A ball (0.5 m diameter) is released from a random point along the opposite side of the field from the goal. The ball is given an initial velocity of 3-5 m/s at a random angle towards the goal end of the field.
- Due to the ramps on the field, the ball will bounce and roll unpredictably as it crosses the field.
- The robot begins in the center of the field on the goal side.

Task:
The robot must intercept the bouncing ball and kick it into the goal to score a point. The robot should dynamically adjust its approach to the ball based on the ball's changing trajectory after each bounce off a ramp. The robot needs to time its kick to hit the ball at the optimal point in its bounce to redirect it into the goal.

Success Conditions:
The task is completed successfully if the robot causes the ball to fully enter the goal area.

Rewards:
- Small reward for decreasing distance to the ball, scaled higher as the ball gets closer to the robot's side of the field
- Moderate penalty if the ball's velocity drops to zero or it leaves the field without scoring
- Large reward for kicking the ball, scaled by the ball's post-kick velocity in the direction of the goal
- Large reward for scoring a goal

Termination:
The episode ends if the ball comes to rest, leaves the field, or enters the goal area.
\end{lstlisting}


==> task_descs/long_run/long_run_90.tex <==
\begin{lstlisting}[language={}]
Outdoor Retrieval Challenge

Description:
- The environment is a large outdoor field 50 m x 50 m, with the robot starting in the center. 
- The terrain includes various features:
  - A steep hill with a 30 degree incline
  - A shallow stream, 0.5 m deep and 5 m wide
  - Patches of loose sand and gravel
  - Scattered trees and boulders up to 2 m tall
- A 0.5 m diameter soccer ball is placed randomly between 10 m and 20 m from the robot's starting position.
- The robot must locate the ball, pick it up or get it balanced on its back, and return it to the starting location.
- The ball is heavy enough that it can't simply be pushed the whole way. The robot needs to lift/carry it.
- If the robot drops the ball or it rolls more than 5 m away, it is replaced at a new random location.

Success Conditions:
The task is completed when the robot returns to within 2 m of its starting position with the ball balanced on its back or in its possession.

Time Limit:
The robot has 10 minutes to complete the retrieval.

Rewards:
- Provide a small reward for exploring the environment and locating the ball
- Provide a moderate reward for successfully getting the ball balanced on the robot's back or lifted off the ground 
- Provide a large reward for returning to the start area with the ball
- Provide a small penalty if the ball is dropped or lost, to encourage careful handling

Termination:
The episode ends if the robot flips over and can't right itself, or if the time limit is exceeded.
\end{lstlisting}

